STACL: Simultaneous Translation with Implicit Anticipation and Controllable Latency using Prefix-to-Prefix Framework

Simultaneous translation, which translates sentences before they are finished, is useful in many scenarios but is notoriously difficult due to word-order differences. While the conventional seq-to-seq framework is only suitable for full-sentence translation, we propose a novel prefix-to-prefix framework for simultaneous translation that implicitly learns to anticipate in a single translation model. Within this framework, we present a very simple yet surprisingly effective wait-k policy trained to generate the target sentence concurrently with the source sentence, but always k words behind. Experiments show our strategy achieves low latency and reasonable quality (compared to full-sentence translation) on 4 directions: zh<->en and de<->en.

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs/*.tex)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<


%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi


long.bib:	all.bib
	./remove-short.pl all.bib > long.bib

submit:
	gs -q -sPAPERSIZE=a4 -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=paper.pdf -dFirstPage=1 -dLastPage=10 main.pdf
	gs -q -sPAPERSIZE=a4 -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=appendix.pdf -dFirstPage=11  main.pdf

######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile


==> appen.tex <==
% !TEX root = main.tex

\begin{figure*}
\begin{tabular}{cc}
\centering
  \includegraphics[width=7cm]{figs/for_acl/Fig_acl_de2en_RIBES-AP_test.pdf} & \centering
  \includegraphics[width=7cm]{figs/for_acl/Fig_acl_de2en_RIBES-CW_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{Translation quality RIBES against latency metrics (AP and CW) on German-to-English simultaneous translation,
  showing wait-$k$ models (for $k$=1, 3, 5, 7, 9), test-time wait-$k$ results,
  and full-sentence baselines.
  % full-sentence baselines, and our reimplementation of \namecite{gu+:2017}.
}
\label{fig:APCW_de2en_ribes}
\bigskip

\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2de_RIBES-AP_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2de_RIBES-CW_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{RIBES against latency metrics (AP and CW) on English-to-German simultaneous translation.
}
\label{fig:APCW_en2de_ribes}


\bigskip
\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_zh2en_RIBES-AP_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_zh2en_RIBES-CW_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{RIBES against latency metrics (AP and CW) on Chinese-to-English simultaneous translation.
}

\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2zh_RIBES-AP_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2zh_RIBES-CW_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{RIBES against latency metrics (AP and CW) on English-to-Chinese simultaneous translation.
}
\label{fig:APCW_en2zh_ribes}
\end{figure*}

==> simul-acl copy 2/Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs/*.tex)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<


%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi


long.bib:	all.bib
	./remove-short.pl all.bib > long.bib

submit:
	gs -q -sPAPERSIZE=a4 -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=paper.pdf -dFirstPage=1 -dLastPage=10 main.pdf
	gs -q -sPAPERSIZE=a4 -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=appendix.pdf -dFirstPage=11  main.pdf

######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile


==> simul-acl copy 2/al.tex <==
% !TEX root = main.tex
Beside translation quality, latency is another crucial aspect for evaluating simultaneous translation. % how much time
%is wasted waiting for the translation. 
%This section first introduce the existing metrics for latency measurements. 
We first review existing latency metrics, highlighting their limitations,
%and then show the problems of existing latency metrics.
aand then propose our new latency metric that address these limitations.

\subsection{Existing Metrics: CW and AP}
% AP and CW are the two most widely used metrics for measuring latencies, 
% and they are proposed in \cite{Cho+:16}.

Consecutive Wait (CW) \cite{gu+:2017} is the number of source words
waited between two target words. Using our notation,
for a policy $g(\cdot)$, the per-step CW at step $t$ is
\(
\CW_g(t) = g(t) - g(t-1).
\)
The CW of a sentence-pair $(\vecx, \vecy)$ is the average CW over all consecutive wait segments:
\[
\resizebox{.48\textwidth}{!}{
  $\CW_g(\vecx,\vecy) = \displaystyle\frac{\sum_{t=1}^{|\vecy|} \CW_g(t)}{\sum_{t=1}^{|\vecy|} \mathbbm{1}_{\CW_g(t) > 0}} = \frac{|\vecx|}{\sum_{t=1}^{|\vecy|} \mathbbm{1}_{\CW_g(t) > 0}}$
  }
\]
\vspace{-0.3cm}
%% defines the consecutive waits while 
%% translating each target word. It describes the length of silence 
%% between two translated adjacent words.
%% For each READ or WRITRE action, we have the CW definition as follows:

%% \begin{equation*}
%% c_t=\left\{\begin{matrix}
%%  c_{t-1} + 1& a_t \; \text{is READ}  & \\ 
%%  0& \;\;a_t \; \text{is WRITE}  & 
%% \end{matrix}\right.
%% \label{eq:CW}
%% \end{equation*}
%% where $a_t$ is the action at $t^{th}$ time step and $c_t$ is the number of 
%% waited words between two adjacent translated words.
In other words, CW measures the average source segment length (the best case is 1 for word-by-word translation or our wait-1 and the worst case is $|\vecx|$ for full-sentence MT).
The drawback of CW is 
that CW is local latency measurement which is 
insensitive to the actual lagging behind.
% as discussed in the previous Section;
% for example, catchup has no effect on CW.

Another latency measurement, Average Proportion (AP) \cite{Cho+:16} measures
%focuses on the global latency 
%which is defined as follows:
the proportion of the area above a policy path in Fig.~\ref{fig:idea}:
\vspace{-0.2cm}
\begin{equation}
\AP_g(\vecx,\vecy) = \frac{1}{|\vecx|\;|\vecy|} \textstyle\sum_{t=1}^{|\vecy|} g(t) 
\label{eq:AP}
\end{equation}

AP has two major flaws:
First, it is sensitive to input length. % is defined to show the global delays but there is an obvious flaw of it.
For example, consider our wait-1 policy.
When $|\vecx|=|\vecy|=1$, AP is 1,
and when $|\vecx|=|\vecy|=2$, AP is 0.75,
and eventually AP approaches 0.5 when  $|\vecx|=|\vecy|\goesto\infty$.
However, in all these cases, there is a one word delay,
so AP is not fair between long and short sentences.
Second, being a percentage,
it is not obvious to the user the actual delays in number of words.

\if
Consecutive Wait (CW)  \cite{gu+:2017} measures the average lengths of conseuctive wait segments
(the best case is 1 for our wait-1 and the worst case is $|\vecx|$ for full-sentence MT).
%%  (CW) \cite{gu+:2017} is the number of source words
%% waited between two target words. %Using our notation,
For a policy $g(\cdot)$, the per-step CW at step $t$ is
\(
\CW_g(t) = g(t) - g(t-1).
\)
The CW of a sentence-pair $(\vecx, \vecy)$ is the average CW over all consecutive wait segments:
\[
\resizebox{.48\textwidth}{!}{
  $\CW_g(\vecx,\vecy) = \displaystyle\frac{\sum_{t=1}^{|\vecy|} \CW_g(t)}{\sum_{t=1}^{|\vecy|} \mathbbm{1}_{\CW_g(t) > 0}} = \frac{|\vecx|}{\sum_{t=1}^{|\vecy|} \mathbbm{1}_{\CW_g(t) > 0}}$
  }
\]
\vspace{-0.3cm}


Another latency measurement, Average Proportion (AP) \cite{Cho+:16} measures
%focuses on the global latency 
%which is defined as follows:
the proportion of the area above a policy path in Fig.~\ref{fig:idea}:
\vspace{-0.2cm}
\begin{equation}
\AP_g(\vecx,\vecy) = \frac{1}{|\vecx|\;|\vecy|} \textstyle\sum_{t=1}^{|\vecy|} g(t) 
\label{eq:AP}
\end{equation}

The above 



Another latency measurement, Average Proportion (AP) \cite{Cho+:16} measures
%focuses on the global latency 
%which is defined as follows:
the proportion of the shaded area for a policy in Fig.~\ref{fig:catchup}:
\begin{equation}
\AP_g(\vecx,\vecy) = \frac{1}{|\vecx|\;|\vecy|} \textstyle\sum_{t=1}^{|\vecy|} g(t) 
\label{eq:AP}
\end{equation}

%% Same with Eq.~\ref{eq:policy}, $g(t)$ from above equation measures the number of source words been waited when decoding the 
%% $t^{th}$ on target side.

%% We observe from the above definitions that CW only defines the local latency 
%% and hard to define the global delays. 

AP has two major flaws:
First, it is sensitive to input length. % is defined to show the global delays but there is an obvious flaw of it.
For example, consider our wait-1 policy.
When $|\vecx|=|\vecy|=1$, AP is 1,
and when $|\vecx|=|\vecy|=2$, AP is 0.75,
and eventually AP approaches 0.5 when  $|\vecx|=|\vecy|\goesto\infty$.
However, in all these cases, there is a one word delay,
so AP is not fair between long and short sentences.
Second, being a percentage,
it is not obvious to the user the actual delays in number of words.
%% For example, we have an translation policy which decodes one target word once 
%% there is a new coming source word on the decoder side. 
%% More explicitly, the action sequence is ``R W R W R W R W...'' or ``(R W)$^+$'', where the number of R's
%% equals to the length of source words, and the number of W's equals to the length of target words.
%% Assume we have two source words and they can be translated into anther 
%% two words in target language.
%% Following Eq.~\ref{eq:AP}, we have a latency of $0.75$.
%% However, when we increase the length for both source and target side infinity,
%% % side (assume source and target sides have the same number of words for simplicity),a
%% % for example we set $|x|$ and $|y|$ to infinity.
%% we then will have a different latency for the same policy whose AP almost equals to $0.5$.
%% Furthermore, it is still not obvious to the user about the actual delays in number of words
%% when AP is defined in percentage.

%% Therefore, AP is very sensitive to the actual length on both side and it only
%% can make a fair comparison between two policies which are 
%% operated on the same source and target length.
%% In order to have a global latency definition which is not correlated with the source and 
%% target sides' length and more easy to understand by users,
%% we propose another latency measurements Average Lagging (AL).
\fi 

\subsection{New Metric: Average Lagging}

\begin{figure}%[t]
\centering
\includegraphics[width=7.8cm]{figs/al.pdf}
\captionof{figure}{Illustration of our proposed Average Lagging latency metric. The left figure shows a simple case 
  when $|\vecx|=|\vecy|$ while the right figure shows a more general case when $|\vecx| \neq |\vecy|$.
  The red policy is wait-4,  the yellow is  wait-1, and the thick black is % steps
  a policy whose AL is 0. % (wait-0 on the left).
}
\label{fig:al}
\end{figure}

Inspired by the idea of ``lagging behind the ideal policy'',
we propose a new metric called ``average lagging'' (AL),
shown in Fig.~\ref{fig:al}. % shows the basic idea of intuition of our proposed metric.
The goal of AL is to quantify the degree the user is out of sync with the speaker, in terms of the number of source words.
The left figure shows a special case when $|\vecx|=|\vecy|$ for simplicity reasons. %y demonstration.
The thick black line indicates the ``wait-0'' policy where the decoder is alway one word {\em ahead} of the encoder
and we define this policy to have an AL of 0.
The diagonal yellow policy is our ``wait-1'' which is always one word behind the wait-0 policy. %which starts translating every new words from the 
%first source word.
In this case, we define its AL to be 1.
%% which measures these averaged yellow areas 
%% which are below the thick black line across different steps.
% The yellow squares are on the diagonal which indicates the most ideal case when
% the decoder translates the new coming word without any delay. 
% In this case, our AL is $1$.
% The yellow indicates the ``wait-1'' policy which starts translating every new words from the 
% first source word.
% AL aims to measure these yellow areas which below the red line.
The red policy is our wait-4, and it is always 4 words behind the wait-0 policy, so its AL is 4.
Note that in both cases, we only count up to (but including) the cut-off point (indicated by the horizontal yellow/red arrows,
or 10 and 7, resp.) because the tail can be generated instantly without  further delay.
%% When we have ``wait-4'' policy which starts translating every new words from the 
%% third source word, we use all the red area and the first $7$ yellow square (start from left) to represents the lagging whose AL is $4$.
More formally, for the ideal case where $|\vecx=|\vecy|$, we can define:
\begin{equation}
\AL_g(\vecx,\vecy) = \frac{1}{\tau_g(|\vecx|)} \sum_{t = 1}^{\tau_g(|\vecx|)} g(t) - (t-1)
\label{eq:AL}
\end{equation}
We can infer that the AL for wait-$k$ is exactly $k$.


When we have more realistic cases like the right side of Fig.~\ref{fig:al} when $|\vecx|<|\vecy|$,
% as explained in Sec.~\ref{sec:catchup},
there are more and more delays accumulated when target sentence grows.% (see also Fig.~\ref{fig:catchup}).
For example, for the yellow wait-1 policy has a delay of more than 3 words at decoding its cut-off step 10,
and the red wait-4 policy has a delay of  almost 6 words at its cut-off step 7.
%while we only have $1$ word delay on the left case.
This difference is mainly caused by the tgt/src ratio.
For the right example, there are $1.3$ target words per source word.
%% Based on the above observation, we need to define a more general latency measurement that 
%% takes length ratio in to consideration.
More generally, we need to offset the ``wait-0'' policy and redefine: %have the AL definition as follows:
\begin{equation}
\AL_g(\vecx,\vecy) = \frac{1}{\tau_g(|\vecx|)} \sum_{t = 1}^{\tau_g(|\vecx|)} g(t) - \frac{t-1}{r}
\label{eq:AL2}
\end{equation}
%where we use $\tau = \argmin_{\tau}(g(\tau)=|x|)$ to find the earliest point 
%when encoder observes the full source sentence
where $\tau_g(|\vecx|)$ denotes the cut-off step,
and $r=|y|/|x|$ is the target-to-source length ratio.
%and the $1/r$ ratio is to offset the wait 
We observe that wait-$k$ with catchup has an AL  $\simeq k$.
%For the right example in Fig.~\ref{fig:al}, $\tau$ are $10$ and $7$ for the yellow policy and the red policy respectively.

%% Eq.~\ref{eq:AL} describes the average delayed words. Note that we sum the laggings up to
%% $\tau$ since when we can decode all the rest words without extra waiting 
%% after the entire source sentence are observed.
%% % The right side of Fig.~\ref{fig:al} shows that ``wait-1'' policy accumulates more delay
%% % when $\gamma>1$. 
%% ``wait-1'' policy's AL on right figure is greater than the one on the left side, which shows 
%% that our AL is more sensitive to the actual $\gamma$ ratio.




==> simul-acl copy 2/appen.tex <==
% !TEX root = main.tex

\begin{figure*}
\begin{tabular}{cc}
\centering
  \includegraphics[width=7cm]{figs/for_acl/Fig_acl_de2en_RIBES-AP_test.pdf} & \centering
  \includegraphics[width=7cm]{figs/for_acl/Fig_acl_de2en_RIBES-CW_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{Translation quality RIBES against latency metrics (AP and CW) on German-to-English simultaneous translation,
  showing wait-$k$ models (for $k$=1, 3, 5, 7, 9), test-time wait-$k$ results,
  and full-sentence baselines.
  % full-sentence baselines, and our reimplementation of \namecite{gu+:2017}.
}
\label{fig:APCW_de2en_ribes}
\bigskip

\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2de_RIBES-AP_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2de_RIBES-CW_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{RIBES against latency metrics (AP and CW) on English-to-German simultaneous translation.
}
\label{fig:APCW_en2de_ribes}


\bigskip
\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_zh2en_RIBES-AP_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_zh2en_RIBES-CW_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{RIBES against latency metrics (AP and CW) on Chinese-to-English simultaneous translation.
}

\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2zh_RIBES-AP_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2zh_RIBES-CW_test.pdf}
\end{tabular}\\[-0.3cm]
\captionof{figure}{RIBES against latency metrics (AP and CW) on English-to-Chinese simultaneous translation.
}
\label{fig:APCW_en2zh_ribes}
\end{figure*}

==> simul-acl copy 2/catchup.tex <==
% !TEX root = main.tex


% \newcolumntype{M}{>{\em}c}

% <<<<<<< HEAD
% % \begin{table*}[!ht]
% % \centering
% % % \setlength{\tabcolsep}{2pt}
% % \resizebox{16cm}{!}{%

% % \begin{tabular}{ | c |c |c|M |c|M |c |M |c |M |c|M|c|M|}
% % \hline
% % \color{red}\zhtoen test & \em{k} & \multicolumn{2}{c|}{1} &\multicolumn{2}{c|}{3} &\multicolumn{2}{c|}{5} &\multicolumn{2}{c|}{7} &\multicolumn{2}{c|}{9}& \multicolumn{2}{c|}{$\infty$} \\
% % \hline
% % \multirow{3}{*}{\shortstack{Transformer\\ wait-\em{k}}} & AP& 0.60 & \em{0.59} & 0.67 & \em{0.67} & 0.73 & \em{0.73} & 0.77 & \em{0.78} & 0.82 & \em{0.82} &  \multicolumn{2}{c|}{1}\\
% =======
% \begin{table*}[h]
% \centering
% % \setlength{\tabcolsep}{2pt}
% \resizebox{16cm}{!}{%

% \begin{tabular}{ | c |c |c|M |c|M |c |M |c |M |c|M|c|M|}
% \hline
% \color{red}\zhtoen test & \em{k} & \multicolumn{2}{c|}{1} &\multicolumn{2}{c|}{3} &\multicolumn{2}{c|}{5} &\multicolumn{2}{c|}{7} &\multicolumn{2}{c|}{9}& \multicolumn{2}{c|}{$\infty$} \\
% \hline
% \multirow{3}{*}{\shortstack{Transformer\\ wait-\em{k}}} & AP& 0.60 & \em{0.59} & 0.67 & \em{0.67} & 0.73 & \em{0.73} & 0.77 & \em{0.78} & 0.82 & \em{0.82} &  \multicolumn{2}{c|}{1}\\
% \cline{2-14}
% & AL & 2.9 & 2.7 & 5.0 & 5.0 & 6.8 & 6.9 & 8.3 & 8.5 & 10.3 & 10.5 &  \multicolumn{2}{c|}{28.7} \\
% \cline{2-14}
% & 4-ref BLEU & 25.79 & 26.02 & 28.94 & 29.45 & 31.14 & 31.62 & 31.74 & 32.55 & 33.46 & 34.39 & 36.29 & 38.34\\
% \hline
% \multirow{3}{*}{\shortstack{Transformer\\wait-\em{k}\\\color{blue} + \chn{decoder catchup}}} & AP&  0.53 & 0.52 & 0.61 & 0.6 & 0.67 & 0.66 & 0.73 & 0.72 & 0.79 & 0.78 &\multicolumn{2}{c|}{1}\\
% \cline{2-14}
% & AL & 0.54 & 0.29 & 2.6 & 2.3 & 4.1 & 3.8 & 6.3 & 5.9 & 8.7 & 8.2 &  \multicolumn{2}{c|}{28.7}\\
% \cline{2-14}
% % & 1-ref BLEU & 11.64 & 11.55 & 13.93 & 13.87 & 14.92 & 14.81 & 16.67 & 16.46 & 17.38 & 17.05 & 19.03 & 20.29\\
% >>>>>>> 6d37cd101f403427ab7c1ae43acbcbb9535f56b1
% \cline{2-14}
% & AL & 2.9 & 2.7 & 5.0 & 5.0 & 6.8 & 6.9 & 8.3 & 8.5 & 10.3 & 10.5 &  \multicolumn{2}{c|}{28.7} \\
% \cline{2-14}
% & 4-ref BLEU & 25.79 & 26.02 & 28.94 & 29.45 & 31.14 & 31.62 & 31.74 & 32.55 & 33.46 & 34.39 & 36.29 & 38.34\\
% \hline
% \multirow{3}{*}{\shortstack{Transformer\\wait-\em{k}\\\color{blue} + \chn{decoder catchup}}} & AP&  0.53 & 0.52 & 0.61 & 0.6 & 0.67 & 0.66 & 0.73 & 0.72 & 0.79 & 0.78 &\multicolumn{2}{c|}{1}\\
% \cline{2-14}
% & AL & 0.54 & 0.29 & 2.6 & 2.3 & 4.1 & 3.8 & 6.3 & 5.9 & 8.7 & 8.2 &  \multicolumn{2}{c|}{28.7}\\
% \cline{2-14}
% % & 1-ref BLEU & 11.64 & 11.55 & 13.93 & 13.87 & 14.92 & 14.81 & 16.67 & 16.46 & 17.38 & 17.05 & 19.03 & 20.29\\
% % \cline{2-14}
% & 4-ref BLEU & 19.95 & 20.32 & 24.52 & 24.85 & 27.53 & 27.66 & 30.56 & 30.51 & 31.19 & 31.29 & 36.29 & 38.34\\
% \hline
% \hline
% \color{red}\entozh test & \em{k} & \multicolumn{2}{c|}{1} &\multicolumn{2}{c|}{3} &\multicolumn{2}{c|}{5} &\multicolumn{2}{c|}{7} &\multicolumn{2}{c|}{9}& \multicolumn{2}{c|}{$\infty$} \\
% \hline
% \multirow{3}{*}{\shortstack{Transformer\\ wait-\em{k} \\ \color{blue}+ \chn{encoder catchup}}} & AP& 0.52 & 0.53 & 0.59 & 0.59 & 0.64 & 0.65 & 0.69 & 0.69 & 0.73 & 0.73 & \multicolumn{2}{c|}{1}\\
% \cline{2-14}
% & AL & 0.39 & 0.56 & 2.6 & 2.7 & 4.5 & 4.6 & 6.3 & 6.3 & 8.1 & 8.1 & \multicolumn{2}{c|}{38.3} \\
% \cline{2-14}
% & 1-ref BLEU & 9.37 & 9.41 & 12.62 & 12.61 & 14.4 & 14.56 & 15.67 & 16.39 & 16.22 & 16.99 & 18.65 & 19.56\\
% \hline
% \end{tabular} 
% }
% \caption{Performances of wait-$k$ with Transformer, its catchup version with various $k$ 
% % (the number of waited words) %(first row) 
% %and AP in
% %1-ref and 4-ref BLEU scores 
% on the \zhen test sets.
% For each $k$, the numbers on left side are from greedy decoding,
% and right, italic font numbers are from tail beam search.
% $\infty$ represents baseline with results from greedy and beam search.}
% \label{tb:waitktest}
% \end{table*}





%\subsection{Wait-$k$ with Catchup}
%In aforementioned section,
As mentioned in Sec.~\ref{sec:pred},
the wait-$k$ decoding % of proposed wait-$k$ process 
is always $k$ words behind the incoming source stream. 
In the ideal case where the input and output sentences have equal length,
the translation will finish $k$ steps after the source sentence finishes, i.e., the tail length is also $k$.
This is consistent with human interpreters who start and stop a few seconds after
the speaker starts and stops.



%% the last $k$ words on target side will be generated without waiting 
%% the encoder since there is no new word is expected 
%% on encoder side (for example, a period on source side indicates the source
%% sentence finishes).

However, %sentence pairs in parallel text
input and output sentences
generally have different lengths.
In some extreme directions such as Chinese to English,
the target side is significantly longer than the source side,
with an average gold tgt/src ratio,
\(r=\overline{|\vecy^\star|/|\vecx|}\),
of around 1.25 \cite{huang+:2017,yilin+:2018}.
In this case, if we still follow the vanilla wait-$k$ policy,
the tail length will be $0.25 |\vecx| + k$ which increases with input length.
For example, given a 20-word Chinese input sentence, the tail of wait-3 policy will be 8 word long, almost half of the source length.
This brings two negative effects:
(a) as decoding progresses, the user will be effectively lagging behind further and further (becomes each Chinese word in principle translates to 1.25 English words),
rendering the user more and more out of sync with the speaker;
and
(b) when a source sentence finishes, the rather long tail is displayed immediately, causing a cognitive burden on the user.\footnote{
It is true that the tail can in principle be displayed concurrently with the first $k$  words of the next input,
but the tail is now much longer than $k$.}
These problems become worse with longer input sentences (see Fig.~\ref{fig:catchup}). 
%% From the user perspective, all the previous words are decoded in a one-by-one 
%% fashion while the last $k$ words are shown at one time on 
%% the screen.
%% % (this phenomenon can be easily observed in our on-line demo).
%% This increases the user reading work load suddenly at the end of the sentence.
%% This kind of increases of work load might be fine when $k$ is small.
%% However, when target side are expected to be much longer than source side,
%% this phenomenon becomes displeasing for users when there are much more that
%% $k$ words are threw to users to digest at one time.

%% Based one the previous study of translation ratio from ~\namecite{huang+:2017,yilin+:2018}, it is well known that the target side could be much longer 
%% than source side between some certain translation pairs, e.g., Chinese-to-English.
%% In our Chinese-English development set
%% (NIST 06), 
%% %a widely used Chinese-to-English translation corpus, the NIST dataset, 
%% the target-side English sentence lengths
%% are on average $\sim1.27\times$ the Chinese
%% sentence lengths.


%% Fig.~\ref{fig:catchup} shows one example of translation from Chinese to English. 
%% Note that there are $13$ words on English side while there are only $10$ words on 
%% Chinese side. Left figure shows that in wait $2$ words policy, the translated 
%% English sentence is alway $2$ words behind Chinese inputs. 
%% After wait $2$ words gap, every English word corresponds to one Chinese input.
%% However, the last row indicates that there five English words have been translated
%% at one time during the last step. 
%% The sudden appearance of these five English words would increase the 
%% readers' work load. 
%% Therefore, we propose to ``amortize'' these sudden increased word loads to previous 
%% translation steps. 

To address this problem, we devise a ``wait-$k$+catchup'' policy %to reduce this lagging behind and making the user more in sync with the speaker.
so that the user is still $k$ word behind the input in terms of real information content,
i.e., always $k$ source words behind the ideal perfect synchronization policy denoted by the diagonal line in Fig.~\ref{fig:catchup}.
For example, assume the tgt/src ratio is $r=1.25$, % which can get from training corpus,
%we design another read and write action sequence pattern as $1-1-2$.
we will output 5 target words for every 4 source words;
i.e., the catchup frequency, denoted $c=r-1$, is 0.25.
%e.g., every 4th decoding step will output 2 words.
See Fig.~\ref{fig:catchup}.
%% This means that the decoder will decode $4$ words when there are $3$ new coming words.
%% And the extra one word will always be in the third decoding step for every $3$ 
%% translation time step.
%% In this way, we only expect to generate $3$ words instead of $5$ words. 
%% Note that when sentence gets longer, this different would be more significant.

More formally, with catchup frequency $c$, the new policy is: %we redefine:
\begin{equation}
\gcatchup(t) = \min\{k+t-1-\floor{ct},\; |\vecx|\}
\label{eq:policyc}
\end{equation}
and our decoding and training objectives change accordingly
(again, we {\em train} the model to catchup using this new policy). %become: % as follows:
% The formal definition is as follows:
% \begin{equation*}
% \vspace{-0.1cm}
% \score_{k}(\vecx,\vecy) = \textstyle\sum_{t=1}^{|\vecy|} \log p(y_t \mid \vecx_{\leq g_c(t)},\, \vecy_{<t-1})
% %\vspace{-0.1cm}
% \end{equation*}
%% \begin{eqnarray}
%% \vspace{-0.1cm}
%% p_{g_c}(\vecy \mid \vecx) = \textstyle\prod_{t=1}^{|\vecy|} p(y_t \mid \vecx_{\leq{g_c(t)}},\, \vecy_{<t})\\
%% \ell_{g_c}(D) = - \textstyle{\sum_{(\vecx,\vecy^\star)\in D}} \log p_{g_c} (\vecy^\star \mid \vecx) %\sum_{t=1}^{|\vecy^\star|}  \log p(y_t \mid \vecx_{\leq{g_c(t)}},\; \vecy^\star_{<t})
%% %}
%% \label{eq:catnewtrain}
%% \end{eqnarray}
%where we use $g_c(t)$ to describes the number of source words that have been processed by encoder in catchup mode:

%% where we use $ct$ to represent the index for extra decoding. For example, 
%% in Fig.~\ref{fig:catchup}, catchup index $ct$ is $3$.
%% The initialization value for $ct$ is $0$, and $ct$ increases by one 
%% when $t=3 \times ct$. 
%% In this way, during training time, for the example in Fig.~\ref{fig:catchup},
%% the second and third decoded words share the same context information 
%% from source side.
%% The desired $ct$ can be learned from training corpus.
%% For example, assume we have a length ratio of $1.3$, then we know
%% we should have one extra decoding at time step $3$ since $4/3\simeq 1.3$.

%% \subsection{Tail Beam Search}
On the other hand, when  translating from longer source sentences to shorter 
targets, e.g., from English to Chinese,
%the catchup frequency is negative
%(i.e., catchup on encoder rather than decoder). % is  also important. 
%Since the target side is shorter, % than source side sentence, 
it is very possible that the decoder finishes generation before
the encoder sees the entire source sentence,
ignoring the ``tail'' on the source side.
%% and 
%% ignores the unprocessed later information from source side.
% the decoder could generate \eos even before the entire source sentence are encoded.
% In this case, it is very possible that the generated target sentence 
% might miss the entire later information from source side. 
Therefore, we need ``reverse'' catchup, i.e., catching up on encoder instead of decoder. %  which has extra encoding step with certain frequency.
For example, in English-to-Chinese translation, 
we encode one extra word
every 4 steps, i.e., encoding 5 English words per 4 Chinese words.
In this case, the ``decoding'' catcup frequency $c=r-1=-0.2$ is negative but Eq.~\ref{eq:policyc} still holds.
Note that it works for any arbitrary $c$, such as 0.341, where the catchup pattern is not as easy as ``1 in every 4 steps'', but still maintains a rough frequency
of $c$ catchups per source word.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/catchup.pdf}
\captionof{figure}{Left (wait-2): it renders the user increasingly out of sync with the speaker (the diagonal line denotes the ideal perfect synchronization).
Right (+catchup): it shrinks the tail and is closer to the ideal diagonal, reducing the effective latency. %two words shorter.
Black and red arrows illustrate 2 and 4 words lagging behind the diagonal, resp.%  and the red arrow represents 4 word latency.
}
\label{fig:catchup}
\vspace{-0.5cm}
\end{figure}

Fig.~\ref{fig:bleuAL_dev1} shows the comparison between wait-$k$ 
model and catchup policy which enables one extra word decoding 
on every $4^{th}$ step. For example, for wait-$3$ policy with 
catchup, the policy is R R (R W R W R W R {\underline{W W}})$^+$ 
W$^+$. 


\begin{figure}[!h]
\centering
\includegraphics[width=7.3cm]{figs/for_TACL/Fig3a_zh2en_AL_dev.pdf} 
\captionof{figure}{
BLEU scores and AL comparisons with different wait-$k$ models on Chinese-to-English on dev set. 
% Note that we use 4-ref BLEU for Chinese-to-English.
\textcolor{colorC0}{\scriptsize$\square$} and \textcolor{colorC1}{$\circ$} are decoded with tail beam search. {$\bigstar$\ding{73}} and  \textcolor{colorC0}{$\bigstar$\ding{73}} are greedy decoding and beam-search baselines.}
\label{fig:bleuAL_dev1}
\end{figure}


% \begin{figure}[!h]
% \centering
% \includegraphics[width=7.3cm]{figs/for_TACL/Fig3b_en2zh_AL_dev.pdf}
% \captionof{figure}{
% BLEU scores and AL comparisons with different wait-$k$ models on Chinese-to-English (left) and English-to-Chinese (right)
% translations on dev set. Note that we use 4-ref BLEU for Chinese-to-English but 1-ref BLEU for English-to-Chinese since the multiple references are only available on English side.{$\bigstar$\ding{73}} and  \textcolor{colorC0}{$\bigstar$\ding{73}} are greedy decoding and beam-search baselines.}
% \label{fig:bleuAL_dev1}
% \end{figure}

%% at the 
%% second step for every five words and the encoding pattern becomes
%%  $1-2-1-1$ which encode $5$
%% words in 4 steps.
%% This frequency is determined by the training source-to-target sentence length ratio.

%\subsection{Tail Beam Search}
%>>>>>>> 1d89e9fb28070efa7608d99453452d94bb57d64e

%% \begin{figure}%[t]
%% \centering
%% \includegraphics[width=7.8cm]{figs/tailbeam.pdf}
%% \captionof{figure}{Tail beam search after encoder processes the entire source sentence.
%% }
%% \label{fig:tailbs}
%% \end{figure}

%% In conventional NMT framework, it has been demonstrated that beam search greatly 
%% improves translation quality by keeping $b$ candidates at each decoding step. 
%% Based over the entire trajectory score, later trajectory choice might 
%% change the previous decoded words.

%% However, the basic wait-$k$ model only decodes one word at a time and it 
%% does not allow the refinements on the decoded words. 
%% The model only have consecutive decoding steps until there is no new coming words 
%% on the encoder side.
%% We refer these consecutive decoding steps as tail and
%% we apply beam search to the tail of target sentence.
%% As shown in Fig.~\ref{fig:tailbs}, there are another 4 decoding steps (tail) after 
%% the encoder processed the entire source sentence.
%% The green box represents the beam search over tail words of target sentence.
%% There are longer tails for larger $k$ or larger source-to-target 
%% length ratio.

%% % The formal definition is as follows:
%% % \begin{equation*}
%% % \vspace{-0.1cm}
%% % \score_{k}(\vecx,\vecy) = \textstyle\sum_{t=1}^{|\vecy|} \log p(y_t \mid \vecx_{<{(t+k-ct)}},\, \vecy_{<t-1})
%% % %\vspace{-0.1cm}
%% % \end{equation*}
%% % where we use $ct$ to represent the index for extra decoding. For example, 
%% % in ~Fig.\ref{fig:catchup}, catchup index $ct$ is $3$.
%% % The initialization value for $ct$ is $0$, and $ct$ increases by one 
%% % when $t=3 \times ct$. 
%% % In this way, during training time, for the example in Fig.~\ref{fig:catchup},
%% % the second and third decoded words share the same context information 
%% % from source side.
%% % The desired $ct$ can be learned from training corpus.
%% % For example, assume we have a length ratio of $1.3$, then we know
%% % we should have one extra decoding at time step $3$ since $4/3$ is $1.3$.


% The formal definition is as follows:
% \begin{equation*}
% \vspace{-0.1cm}
% \score_{k}(\vecx,\vecy) = \textstyle\sum_{t=1}^{|\vecy|} \log p(y_t \mid \vecx_{<{(t+k-ct)}},\, \vecy_{<t-1})
% %\vspace{-0.1cm}
% \end{equation*}
% where we use $ct$ to represent the index for extra decoding. For example, 
% in ~Fig.\ref{fig:catchup}, catchup index $ct$ is $3$.
% The initialization value for $ct$ is $0$, and $ct$ increases by one 
% when $t=3 \times ct$. 
% In this way, during training time, for the example in Fig.~\ref{fig:catchup},
% the second and third decoded words share the same context information 
% from source side.
% The desired $ct$ can be learned from training corpus.
% For example, assume we have a length ratio of $1.3$, then we know
% we should have one extra decoding at time step $3$ since $4/3$ is $1.3$.




==> simul-acl copy 2/defs.tex <==
% !TEX root = main.tex

\newcommand{\tuple}[1]{\ensuremath{\langle {#1} \rangle}}
%\newcommand{\argmax}[2]{\ensuremath{\mbox{argmax}_{#1}\ {#2}}}

\newcommand{\featuresum}[1]{\ensuremath{\sum_i \lambda_i f_i({#1})}}

\newcommand{\fvec}[1]{\ensuremath{\vec{f} ({#1})}}

\newcommand{\fiof}[1]{\ensuremath{f_i ({#1})}}

\newcommand{\fofi}[0]{\ensuremath{f_i}}

\newcommand{\featureprod}[1]
{\ensuremath{\vec{\lambda} \cdot \fvec{#1} } }

\newcommand{\efprod}[1]{\ensuremath{e^{\featureprod{#1}}}}
\newcommand{\efsum} [1]{\ensuremath{e^{\featuresum {#1}}}}

\newcommand{\lami}{\ensuremath{\lambda_i}}

\newcommand{\empExp}[1]{\ensuremath{\mbox{\~{E}} [{#1}]}}
\newcommand{\expect}{\ensuremath{\mathbb{E}}}

\newcommand{\ks}{\ensuremath{k}}
\newcommand{\Ks}{\ensuremath{K}}
\newcommand{\kbest}{\ks-best\xspace}
\newcommand{\topk}{top-\ks\xspace}
\newcommand{\kBest}{\Ks-Best\xspace}

\newcommand{\notes}[1]{}%{\it {\small {#1}}}}

\newcommand{\acite}[1]{({--#1})}

\newcommand{\define}[1]{{\bf Definition.} {\em {#1}}}
\newcommand{\zerobar}{\ensuremath{\overline{0}}\xspace}
\newcommand{\onebar}{\ensuremath{\overline{1}}\xspace}

\newcommand{\Items}{\ensuremath{\mathcal{I}}\xspace}

\newcommand{\oplusk}{\ensuremath{\oplus_{\tiny k}}}
\newcommand{\otimesk}{\ensuremath{\otimes_{\tiny k}}}

\newcommand{\zerok}{\ensuremath{\overline{0}^k}\xspace}
\newcommand{\onek}{\ensuremath{\overline{1}^k}\xspace}

\newcommand{\scalar}{\ensuremath{\odot_k}}

\newcommand{\kdim}{\ks-dimensional\ }





% \newlistof{defin}{def}{List of Definitions}

% \newcommand{\defin}[1]{%
% \refstepcounter{defin}
% \par\noindent\textbf{Definition \thedefin. #1}
% \addcontentsline{ans}{defin}{\protect\numberline{\thedefin}#1}\par}

% for amsthm
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}[theorem]{Definition}

\newcommand{\gc}{\ensuremath{|G|}\xspace}
\newcommand{\ntsize}{\ensuremath{|N|}\xspace}
\newcommand{\nt}{\ensuremath{N}\xspace}
\newcommand{\rulepernt}{\ensuremath{R}\xspace}

\newcommand{\Ttimesk}{\ensuremath{T_{\otimesk}}\xspace}
\newcommand{\Tplusk}{\ensuremath{T_{\oplusk}}\xspace}
\newcommand{\maxk}{\ensuremath{\mbox{\bf max}_k}\xspace}

\newcommand{\tenexp}[1]{\ensuremath{10^{{-#1}}}\xspace}

\newcommand{\naive}{na\"{\i}ve\xspace}

\newcommand{\perc}[1]{\ensuremath{{#1}\%}\xspace}

\newcommand{\veca}{\ensuremath{\mathbf{a}}}
\newcommand{\vecb}{\ensuremath{\mathbf{b}}}
\newcommand{\vecp}{\ensuremath{\mathbf{p}}}
\newcommand{\klogk}{\ensuremath{k\log k}}
\newcommand{\vecz}{\ensuremath{\mathbf{z}}}
\newcommand{\vech}{\ensuremath{\mathbf{h}}}
\newcommand{\vecW}{\ensuremath{\mathbf{W}}}
\newcommand{\vecs}{\ensuremath{\mathbf{s}}\xspace}
\newcommand{\better}{\ensuremath{\preceq}}


\newcommand{\opt}{\ensuremath{\mbox{{\bf min}}_\better}}
\newcommand{\mergek}{\ensuremath{\mbox{{\bf merge}}_{\better k}}\xspace}
\newcommand{\multk}{\ensuremath{\mbox{{\bf mult}}_{\better k}}\xspace}

\newcommand{\kw}{\ensuremath{\mathbf{w}}}

\newcommand{\kwi}{\ensuremath{w_i}}
\newcommand{\wejv}[3]{\ensuremath{w^{#1}_{{#2}}({#3})}}

\newcommand{\vecj}{\ensuremath{\mathbf{j}}}
\newcommand{\vecD}{\ensuremath{\mathbf{D}}}
\newcommand{\vecu}{\ensuremath{\mathbf{u}}\xspace}
\newcommand{\vecU}{\ensuremath{\mathbf{U}}}
\newcommand{\vecjhat}{\ensuremath{\hat{\mathbf{j}}}}
\newcommand{\vecone}{\ensuremath{\mathbf{1}}}
\newcommand{\dbp}[2]{\ensuremath{\langle{#1}, {#2}\rangle}}

\newcommand{\reviewtimetoday}[3]{
    \AtBeginDocument{
    \special{
    !userdict begin
    /pagenum 0 def
    /bop-hook
    {
        /pagenum pagenum 1 add def
        pagenum #3 le
        {
        gsave
        430 750 translate
        0 rotate
        0.4 setgray
        /Times-Roman findfont
        10 scalefont setfont
        0 0   moveto
        (#1) show
        0 -10 moveto
        (#2) show
        grestore
        } if
    } def
    }  }}

% for submission
\iffalse
\renewcommand{\marginpar}[1]{}
\fi

%\newcommand{\comment}[1]{\marginpar{\raggedright{\em{\small #1}}}}

\newcommand{\ith}[1]{\ensuremath{i^{{th}}}}
\def\alglazy{Algorithm 3}

\newcommand{\JnM}{Jim\'enez and Marzal\xspace}

%\newcommand{\ind}[1]{\ensuremath{^{(#1)}}}
\newcommand{\srule}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\goesto}{\ensuremath{\rightarrow}\xspace}
\newcommand{\chn}[1]{\mbox{{\it {#1}}}}

\newcommand{\ngram}{\ensuremath{\text{$n$-gram}}\xspace}
\newcommand{\ngrams}{\ensuremath{\text{$n$-grams}}\xspace}

\newcommand{\ngramitem}[5]{
\ensuremath{
\left(
\begin{smallmatrix}
\mbox{\small {#4}} &\cdots & \mbox{\small {#5}} \\
&
%\!\!_{#2}
\mbox{#1}
%_{#3}
 &
\\ {#2} & & {#3}
\end{smallmatrix}
 \right)
}}

\newcommand{\specialngramitem}[7]{
\begin{math}
\left(
\begin{smallmatrix}
\mbox{\small {#2}}\ \cdots\ \mbox{\small{#3}}
& \cdots &
\mbox{\small {#4}}\ \cdots\ \mbox{\small {#5}} \\
& \mbox{{#1}} & \\
{#6} & & {#7}
\end{smallmatrix}
 \right)
\end{math}
}

\newcommand{\chartitem}[3]{
\ensuremath{(\mbox{#1},{#2},{#3})}
}

\newcommand{\vtnt}[1]{\ensuremath{V_{\mbox{\tiny #1}}}}
%%% \bigram{a}{b} means (a,b) is a bigram pair. P (b | a)!
\newcommand{\bigram}[2]{\ensuremath{\Pr(\mbox{\small #2} \mid \mbox{\small #1})}}

\newcount\permx
\newcount\permy
\def\permdot#1#2{
\permx=#1 \advance\permx by-1
\permy=#2 \advance\permy by-1
\psframe[fillcolor=black, fillstyle=solid]
(\permx,\permy)(#1, #2)
}

%%% note: realcalc.sty has a fatal bug : 23-0.5=23.5.
%%% so i have to do this... +1-0.5 thing
\newcommand{\minushalf}[1]{
    \Radd{\aaa}{#1}{-1}
    \Radd{\aaa}{\aaa}{0.5}
    \Rtrunc{\aaa}{1}{\aaa}
    \aaa
}


\newcommand{\permnt}[3]{
\rput({#1},{#2}){\huge\color{white} {#3}}
}


\newcommand\union{\cup}
\newcommand\intersect{\cap}

\newcommand\vecd[2]{\ensuremath{d_{#2}{(#1)}}}
\newcommand\veczero{\ensuremath{\mathbf{0}}}
\newcommand\vecq{\ensuremath{\mathbf{q}}}
\newcommand\vecn{\ensuremath{\mathbf{n}}}
%\newcommand\vecone{\ensuremath{\mathbf{1}}}
\newcommand{\argmax}{\operatornamewithlimits{\mathbf{argmax}}}
\newcommand{\argtop}{\operatornamewithlimits{\mathbf{argtop}}}
\newcommand{\toptop}{\operatornamewithlimits{\mathbf{top}}}
\newcommand{\argmin}{\operatornamewithlimits{\mathbf{argmin}}}

\newcommand{\deltahat}{\ensuremath{\hat{\delta}}\xspace}

\newcommand{\xrs}{{\bf xRs}\xspace}
\newcommand{\xrsln}{\mbox{1-{\bf xRLNs}}\xspace}
\newcommand{\RLN}{{\bf RLN}\xspace}

\newcommand{\x}[1]{\ensuremath{x_{#1}}\xspace}
\newcommand{\foot}[1]{\ensuremath{^{\tiny({#1})}_{\downarrow}}}


\newcommand{\chnprd}{{\tiny \ensuremath{_{\circ}}}}

%\newcommand{\ckyitem}[3]{\ensuremath{(_{#2}{\mbox{#1}}_{#3})}\xspace}
%\newcommand{\ckyitem}[3]{\ensuremath{({\mbox{#1}}_{#2, #3})}\xspace}
\newcommand{\ckyitem}[3]{\ensuremath{{\mbox{#1}}_{{{#2},\,{#3}}}}\xspace}
\newcommand{\treeitem}[2]{\ensuremath{{\mbox{#1}}_{#2}}\xspace}
\newcommand{\nodent}[3]{\ensuremath{\treeitem{#1}{#2}:{#3}}}

\newcommand{\coverage}[1]{\ensuremath{(\mbox{{#1}})}\xspace}
\newcommand{\lmcov}[2]{\ensuremath{(\mbox{#1}, ^{\mbox{\scriptsize #2}}\!)}\xspace}
\newcommand{\phritem}[3]{\ensuremath{\coverage{#1}:({#2}, \mbox{\footnotesize ``#3''})}\xspace}
\newcommand{\lmphritem}[4]{\ensuremath{\lmcov{#1}{#2}:({#3}, \mbox{\footnotesize ``#4''})}\xspace}
\newcommand{\phrpair}[2]{\ensuremath{\langle \mbox{\chn{#1}, {#2}}\rangle}\xspace}

\newcommand{\lmitem}[3]{\ensuremath{({{#1}}^{#2 \star #3})}\xspace}
%\newcommand{\lmckyitem}[5]{\resizebox{!}{.15in}{\ensuremath{(\mbox{\small #1}_{\mbox{\tiny\ {#2},{#3}}}^{\tiny\ \mbox{#4}\ \star\ \mbox{#5}})}}\xspace}
\newcommand{\lmckyitem}[5]{\ensuremath{(\mbox{#1}_{\mbox{\scriptsize\ ({#2},{#3})}}^{\scriptsize\ \mbox{#4}\ \star\ \mbox{#5}})}\xspace}

\def\wlm{$\mathord+\textrm{LM}$\xspace}
\def\wolm{$\mathord-\textrm{LM}$\xspace}

\newcommand{\sym}[1]{\textrm{#1}\xspace}
\newcommand{\VP}{\sym{VP}}
\newcommand{\PP}{\sym{PP}}

\newcommand{\startsym}{\mbox{\scriptsize \texttt{<s>}}\xspace}
\newcommand{\stopsym}{\mbox{\scriptsize \texttt{</s>}}\xspace}
\newcommand{\TOP}{\sym{TOP}}
%\newcommand{\plm}[2]{\ensuremath{P_{lm}(\mbox{\small #2}\mid\mbox{\small #1})}}
\newcommand{\plm}[2]{\ensuremath{P_{lm}(\mbox{#2}\mid\mbox{#1})}}

%\newcommand{\order}[1]{\ensuremath{\mathcal{O}(#1)}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}

\newcommand{\wocombo}{\ensuremath{h}\xspace}
\newcommand{\mincombo}{\ensuremath{h_{\mathit{combo}}}\xspace}

% \renewcommand{\min}{\ensuremath{\mbox{\bf min}}\xspace}
\newcommand{\hyp}[1]{\mbox{\tiny ``{#1}''}}
\newcommand{\hl}{\ensuremath{k}\xspace}


\newcommand{\cand}{\ensuremath{\mathit{cand}}\xspace}
\newcommand{\buf}{\ensuremath{\mathit{buf}}\xspace}
\newcommand{\bound}{\ensuremath{\mathit{bound}}\xspace}

\newcommand{\lazyjbest}{\ensuremath{\textproc{LazyJthBest}}\xspace}

\newcommand{\backwardstar}{\ensuremath{\mathit{IN}}\xspace}

\newtheorem{proposition}[theorem]{Proposition}

\newcommand{\ff}{\ensuremath{\mathbf{f}}\xspace}
\newcommand{\ee}{\ensuremath{\mathbf{e}}\xspace}
\newcommand{\al}{\ensuremath{\mathbf{a}}\xspace}

\newcommand{\pt}{\ensuremath{p_{\mbox{t}}}}
\newcommand{\pd}{\ensuremath{p_{\mbox{d}}}}


\newcommand{\current}{\color{blue}{\fbox{{\bf C}}}\xspace}
\newcommand{\future}{\color{red}{\fbox{{\bf F}}}\xspace}

\newcommand{\boxnum}[1]{{\setlength{\fboxsep}{1pt}\raisebox{1pt}{\hspace{1pt}\fbox{\tiny #1}\hspace{1pt}}}}
\newcommand{\ind}[1]{\ensuremath{_{\kern-0.5pt\boxnum{#1}}}}
\newcommand{\BS}{\ensuremath{\mathit{IN}}\xspace}
\newcommand{\NTX}{\text{X}}
\newcommand{\NTS}{\text{S}}

\def\FS{\mathit{FS}\xspace}
\def\BS{\mathit{BS}\xspace}
\def\bfR{\mathbf{R}\xspace}

\newcommand{\head}{\ensuremath{\mathit{head}}\xspace}
\newcommand{\tails}{\ensuremath{\mathit{tails}}\xspace}

\newcommand{\Deriv}{\ensuremath{\mathscr{D}}\xspace}
\newcommand{\hhat}{\ensuremath{\hat{h}}\xspace}

\newcommand{\opluseq}{\ensuremath{\ \oplus=}\xspace}

\newcommand{\lianheguo}{\chn{Li\'anh\'egu\'o}\xspace}
\newcommand{\jiandu}{\chn{ji\=and\=u}\xspace}


\newcommand{\chnBushi}{\chn{B\`ush\'i}\xspace}
\newcommand{\chnyu}{\chn{y\v{u}}\xspace}
\newcommand{\chnle}{\chn{le}\xspace}
\newcommand{\chnShalong}{\chn{Sh\=al\'ong}\xspace}
\newcommand{\chnBaoweier}{\chn{B\`aow\=eier}\xspace}
\newcommand{\chnjuxing}{\chn{j\v{u}x\'ing}\xspace}
\newcommand{\chnhuitan}{\chn{hu\`it\'an}\xspace}

\newcommand{\mybullet}{\ensuremath{\bullet\hspace{-0.05mm}}}
\newcommand{\myunderscore}{\ensuremath{\mbox{\Large\_}}}

\newcommand{\nocov}{$_0$\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}
\newcommand{\onecov}{\mybullet$_1$\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}
\newcommand{\halfcov}{\mybullet\myunderscore\myunderscore\mybullet\mybullet\mybullet$_{6}$}
\newcommand{\fullcov}{\mybullet\mybullet\mybullet$_{3}$\mybullet\mybullet\mybullet}

%% \newcommand{\nocov}{\ensuremath{_0\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}\xspace}
%% \newcommand{\onecov}{\ensuremath{\mybullet_1\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}\xspace}
%% \newcommand{\halfcov}{\ensuremath{\mybullet\myunderscore\myunderscore\mybullet\mybullet\mybullet_6}\xspace}
%% \newcommand{\fullcov}{\ensuremath{\mybullet\mybullet\mybullet_3\mybullet\mybullet\mybullet}\xspace}
\newcommand{\fullncov}{\mybullet\mybullet\ldots\mybullet}


\long\def\signature#1{%
% \begin{flushleft}
\begin{center}
% \begin{minipage}{6in}
\parindent=0pt
\shortstack{\vrule width 3in height 0.4pt\\ #1}
% \end{minipage}
\end{center}
% \end{flushleft}
}

% forest rerank acl 2008
\newcommand{\feat}[1]{{\bf {#1}}}
\newcommand{\Gen}[1]{\ensuremath{\mathit{cand}({#1})}\xspace}
\newcommand{\yhat}{\ensuremath{\hat{y}}\xspace}
\newcommand{\ystar}{\ensuremath{y^*}\xspace}
\newcommand{\yplus}{\ensuremath{y^+}\xspace}
\newcommand{\cost}{\ensuremath{\mathit{c}}\xspace}
\newcommand{\oracle}{\ensuremath{\mathit{oracle}}\xspace}
\newcommand{\ora}{\ensuremath{\mathit{ora}}\xspace}
\newcommand{\cnj}{charniak+johnson:2005}
\newcommand{\coll}{collins:2000}
\newcommand{\dom}{\ensuremath{\mathit{dom}}\xspace}
\newcommand{\gold}{\ensuremath{\mathit{gold}}\xspace}

\newcommand{\myoval}[1]{\ovalnode[linestyle=none,fillstyle=solid,fillcolor=lightgray]{foo}{#1}}
\newcommand{\mybox}[1]{\psframebox[linestyle=none,linewidth=0pt,fillstyle=solid,fillcolor=lightgray]{#1}}

\newcommand{\vecx}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\vecy}{\ensuremath{\mathbf{y}}\xspace}
\newcommand{\vecw}{\ensuremath{\mathbf{w}}\xspace}
\newcommand{\vecc}{\ensuremath{\mathbf{c}}\xspace}
\newcommand{\vecR}{\ensuremath{\mathbb{R}}\xspace}

\newcommand{\vecv}{\ensuremath{\mathbf{v}}\xspace}
\newcommand{\vecf}{\ensuremath{\mathbf{f}}\xspace}
\newcommand{\vecfl}{\ensuremath{\mathbf{f}_L}\xspace}
%\newcommand{\veczero}{\ensuremath{\mathbf{j}}}

\newcommand{\heap}{\ensuremath{\mathit{heap}}\xspace}

\newcommand{\feature}[1]{$\langle$ {#1} $\rangle$\xspace}

\newcommand{\defineq}{\ensuremath{\; \triangleq\; }\xspace}
\newcommand{\extradgt}{\color{white}{0}\xspace}

\newcommand{\funit}{\ensuremath{\mathring{f}}\xspace}
\newcommand{\vecfunit}{\ensuremath{\mathring{\vecf}}\xspace}
\newcommand{\Done}[1]{\ensuremath{D_1(#1)}}

% kbest paper 2005
\let\algsize\normalsize
\newcommand{\algline}[2]{%
\begin{center}
\algsize$\text{#1:}\hspace{1em}#2$
\end{center}}

\def\Dhat{\hat{D}}
\def\vecDhat{\mathbf{\hat{D}}}

%%%%%%%%%%%%%%% pinyins

\newcommand{\Baoweier}{\chn{B\`aow\=eier}\xspace}
\newcommand{\Bushi}{\chn{B\`ush\'i}\xspace}
\newcommand{\bushi}{\Bushi}
\newcommand{\Shalong}{\chn{Sh\=al\'ong}\xspace}
\newcommand{\yu}{\chn{y\v{u}}\xspace}
\newcommand{\hai}{\chn{h\'ai}\xspace}
\newcommand{\jiang}{\chn{ji\=ang}\xspace}
\newcommand{\huiwu}{\chn{hu\`iw\`u}\xspace}
\newcommand{\jinyibu}{\chn{j\`iny\={\i}b\`u}\xspace}
\newcommand{\juxing}{\chn{j\v{u}x\'ing}\xspace}
\newcommand{\huitan}{\chn{hu\`it\'an}\xspace}
\newcommand{\dangtian}{\chn{d\=angti\=an}\xspace}
\newcommand{\jiu}{\chn{ji\`u}\xspace}
\newcommand{\zhongdong}{\chn{zh\=ongd\=ong}\xspace}
\newcommand{\weiji}{\chn{w\=eij\=\i}\xspace}
\newcommand{\fuze}{\chn{f\`uz\'e}\xspace}

\newcommand{\zongtong}{\chn{z\v{o}ngt\v{o}ng}\xspace}
\newcommand{\zai}{\chn{z\`ai}\xspace}
\newcommand{\mosike}{\chn{M\`os\-{i}k\={e}}\xspace}
\newcommand{\pujing}{\chn{P\v{u}j\={\i}ng}\xspace}
\newcommand{\eluosi}{\chn{\'Elu\'os\=\i}\xspace}
\newcommand{\meiguo}{\chn{M\v{e}igu\'o}\xspace}
%\dangju & \dui & \shate & \jiezhe & \shizong & \yi & \an &\gandao &  \danyou \\
\newcommand{\dangju}{\chn{d\=angj\'u}\xspace}
\newcommand{\dui}{\chn{du\`\i}\xspace}
\newcommand{\shate}{\chn{Sh\=at\`e}\xspace}
\newcommand{\jiezhe}{\chn{j\`{\i}zh\v{e}}\xspace}
\newcommand{\shizong}{\chn{sh\={\i}z\=ong}\xspace}
\newcommand{\danyou}{\chn{d\=any\=ou}\xspace}
\newcommand{\gandao}{\chn{g\v{a}nd\`ao}\xspace}
\newcommand{\an}{\chn{\`an}\xspace}
\newcommand{\yi}{\chn{y\=\i}\xspace}
\newcommand{\buman}{\chn{b\`um\v{a}n}\xspace}

\newcommand{\Prob}{\ensuremath{\mathrm{P}}\xspace}

\newcommand{\lhs}{\ensuremath{\mathit{lhs}}\xspace}
\newcommand{\rhs}{\ensuremath{\mathit{rhs}}\xspace}

\newcommand{\NULL}{\ensuremath{\mathit{null}}\xspace}

\newcommand{\gap}{\ensuremath{\sqcup}\xspace}
\newcommand{\spanof}{\ensuremath{\mathit{span}}\xspace}
\newcommand{\yield}{\ensuremath{\mathit{yield}}\xspace}
\newcommand{\fs}{\ensuremath{\mathit{admset}}\xspace}

\newcommand{\closed}{\ensuremath{\mathit{closed}}\xspace}
\newcommand{\open}{\ensuremath{\mathit{open}}\xspace}
\newcommand{\hs}{\frag} %\ensuremath{\mathit{frag}}\xspace}
\newcommand{\vs}{\ensuremath{\mathit{vs}}\xspace}
\newcommand{\frag}{\ensuremath{\mathit{frag}}\xspace}
\renewcommand{\root}{\ensuremath{\mathit{root}}\xspace}
\newcommand{\leaves}{\yield} %\ensuremath{\mathit{leaves}}\xspace}
\newcommand{\exps}{\ensuremath{\mathit{front}}\xspace} % frontier
\newcommand{\newexps}{\ensuremath{\mathit{\exps'}}\xspace}


\newcommand{\PLM}{\ensuremath{\Prob_{\mathrm{lm}}}\xspace}
\newcommand{\PT}{\ensuremath{\Prob}\xspace}
\newcommand{\PLex}{\ensuremath{\Prob_{\mathrm{lex}}}\xspace}

\newcommand{\GHKM}[3]{\ensuremath{{\mbox{#1}}_{{#2}}^{{#3}}}\xspace}
%\newcommand{\newGHKM}[2]{\ensuremath{{\mbox{#1}}\\{\mbox{\scriptsize #2}}}\xspace}
\newcommand{\tspan}[1]{\scriptsize {#1}\xspace}
\newcommand{\wnode}[1]{\rnode[t]{#1}{#1}\xspace}  %% target words

\newcommand{\vtitem}[2]{\ensuremath{({\vtnt{#1}}_{#2})}\xspace}
%\newcommand{\gap}{\ensuremath{\sqcup}}
%\newcommand{\treeitem}[2]{\ensuremath{({\mbox{#1}}_{#2})}\xspace}

\newcommand{\ruleset}{\ensuremath{\mathcal{R}}\xspace}

% pattern-match
\newcommand{\match}{\ensuremath{\mathit{match}}\xspace}
\newcommand{\vars}{\ensuremath{\mathit{vars}}\xspace}
\newcommand{\mlist}{\ensuremath{\mathit{mlist}}\xspace}
%\newcommand{\Prob}{\ensuremath{\mathrm{P}}\xspace}
\newcommand{\eP}{\ensuremath{e_{\mathit{p}}}\xspace}
%\newcommand{\PLM}{\ensuremath{\Prob_{\mathrm{lm}}}\xspace}
% \newcommand{\PT}{\ensuremath{\Prob}\xspace}
% \newcommand{\PLex}{\ensuremath{\Prob_{\mathrm{lex}}}\xspace}

%NOW MOVED HERE
\newcommand{\npshift}{\hspace{1.6cm}}
\newcommand{\styleb}{linestyle=dashed}

\newcommand{\et}{\ensuremath{e^{\mathrm{t}}}}
\newcommand{\Ht}{\ensuremath{H^{\mathrm{t}}}}
%\newcommand{\ep}{\ensuremath{e^{\mathrm{p}}}}
\newcommand{\ep}{\ensuremath{e}\xspace}  % just for EMNLP
\newcommand{\Hp}{\ensuremath{H^{\mathrm{p}}}}
\newcommand{\Vp}{\ensuremath{V^{\mathrm{p}}}}

%\newcommand\newcite{\citet}
\def\namecite{\newcite}
%\def\namecite{\cite}

\def\Fone{F$_1$\xspace}
\def\Foneperc{F$_1\%$}
\newcommand{\goto}{\ensuremath{\triangleright}\xspace}

\newcommand{\TODO}[1]{\textbf{TODO:} \textit{#1}\xspace}

\newcommand{\smallnt}[1]{\ensuremath{_{\mbox{\tiny PP}}}\xspace}

\newcommand{\shift}{\ensuremath{\mathsf{sh}}\xspace}
\newcommand{\reduce}{\ensuremath{\mathsf{re}}\xspace}
\newcommand{\lreduce}{\ensuremath{\mathsf{re_{\small \curvearrowleft}}}\xspace}
\newcommand{\rreduce}{\ensuremath{\mathsf{re_{\small \curvearrowright}}}\xspace}


\newcommand{\sep}{\ensuremath{ \circ }\xspace}

\newcommand{\sttop}{\ensuremath{s_0}\xspace}
\newcommand{\stnext}{\ensuremath{s_1}\xspace}
\newcommand{\stthird}{\ensuremath{s_2}\xspace}
\newcommand{\qhead}{\ensuremath{q_0}\xspace}
\newcommand{\qnext}{\ensuremath{q_1}\xspace}
\newcommand{\qthird}{\ensuremath{q_2}\xspace}
\newcommand{\Tag}[1]{\ensuremath{{#1}.\mathsf{t}}\xspace}
\newcommand{\Wrd}[1]{\ensuremath{{#1}.\mathsf{w}}\xspace}
\newcommand{\LC}[1]{\ensuremath{{#1}.\mathsf{lc}}\xspace}
\newcommand{\RC}[1]{\ensuremath{{#1}.\mathsf{rc}}\xspace}

% Algorithm 3 -> Pseudocode 3
\newcommand{\pseudocode}{Algorithm}
\floatname{algorithm}{\pseudocode}

\newcommand{\cont}[2]{\ensuremath{\mathit{c}({#1}, {#2})}\xspace}
\newcommand{\contR}[2]{\ensuremath{\mathit{c}_{\mbox{\tiny \sc R}}({#1}, {#2})}\xspace}
\newcommand{\contsttops}{\ensuremath{\cont{\stnext}{\sttop}}\xspace}
\newcommand{\contsttopqhead}{\ensuremath{\contR{\sttop}{\qhead}}\xspace}

\newcommand{\sspan}{\ensuremath{\mathit{sp}}\xspace}
\renewcommand{\tspan}{\ensuremath{\mathit{tp}}\xspace}
\newcommand{\aspan}{\ensuremath{\mathit{ap}}\xspace}

% vanilla non-dp shift-reduce item: (l, S, Q)
\newcommand{\olditem}[3]{\ensuremath{{#1}: \tuple{{#2}, \ {#3}}}\xspace}
\newcommand{\newitem}[4]{\ensuremath{{#1}: \tuple{{#2}, \ {#3}, \ {#4}}}\xspace}

\newcommand{\arcs}{\ensuremath{\mathbf{a}}\xspace}
\newcommand{\arcleft}[2]{\ensuremath{{#1}^\curvearrowleft{#2}}\xspace}
\newcommand{\arcright}[2]{\ensuremath{{#1}^\curvearrowright{#2}}\xspace}

% kernel feature function
\newcommand{\vecfker}{\ensuremath{\widetilde{\mathbf{f}}}\xspace}
\newcommand{\fker}[1]{\ensuremath{\vecfker({#1})}\xspace}
\newcommand{\earleyitem}[3]{\ensuremath{\tuple{{#1}, {#2}, \ {#3}}}\xspace}
\newcommand{\nodpearleyitem}[2]{\ensuremath{\tuple{{#1}, \ {#2}}}\xspace}

\iffalse
\newcommand{\eisneritem}[4]{\newitem{#1}{#2}{#3}{\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#4}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\xspace}
\newcommand{\specialeisneritem}[4]{\newitem{#1}{#2}{#3}{#4}\xspace}
\else
\newcommand{\eisneritem}[4]{\tuple{{#1}, {\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#4}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\!\!\!}\xspace}
\newcommand{\specialeisneritem}[4]{\ensuremath{{#1}: \tuple{{#4}}}\xspace}
\newcommand{\gpeisneritem}[5]{\ensuremath{{#1}:\tuple{{#4}, {\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#5}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\!\!\!}}\xspace}
\fi

\newcommand{\decode}{\ensuremath{\mathit{decode}}\xspace}
\newcommand{\GEN}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\GENbar}{\ensuremath{\overline{\GEN}}\xspace}

\newcommand{\spb}[1]{\ensuremath{^{{#1}}}\xspace}
\newcommand{\spbkp}{\ensuremath{\spb{k+1}}\xspace}
\newcommand{\vecwk}{\ensuremath{\vecw\spb{k}}\xspace}
\newcommand{\vecwkp}{\ensuremath{\vecw\spb{k+1}}\xspace}
\newcommand{\vecwt}{\ensuremath{\vecw\spb{t}}\xspace}
\newcommand{\vecwtp}{\ensuremath{\vecw\spb{t+1}}\xspace}
\newcommand{\tth}{\ensuremath{t^{\mathrm{th}}}\xspace}


\newcommand{\err}{\ensuremath{\mathit{err}}\xspace}
\newcommand{\bPhi}{\ensuremath{\mathbf{\Phi}}\xspace}
\newcommand{\dPhi}{\ensuremath{\Delta\bPhi}\xspace}
\newcommand{\labels}{\ensuremath{\mathit{labels}}\xspace}
\newcommand{\onestep}{\ensuremath{\mathit{onestep}}\xspace}
\newcommand{\seqx}{\ensuremath{\overline{x}}\xspace}
\newcommand{\seqy}{\ensuremath{\overline{y}}\xspace}
\newcommand{\seqz}{\ensuremath{\overline{z}}\xspace}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\card}[1]{\lvert#1\rvert}  % cardinality |x|
\newcommand{\normtwo}[1]{\norm{#1}^2}

\newcommand{\seqzt}{\ensuremath{\overline{z}^{(t)}}\xspace}
\newcommand{\seqxt}{\ensuremath{\overline{x}^{(t)}}\xspace}
\newcommand{\seqyt}{\ensuremath{\overline{y}^{(t)}}\xspace}

\newcommand{\defeq}{\ensuremath{\stackrel{\Delta}{=}}\xspace}
\newcommand{\InlineIf}[2]{{\bf if} {#1} {\bf then} {#2}}
\newcommand{\dsep}{\ensuremath{\mathcal{D}(\vecu,\delta)}\xspace}
\newcommand{\dgsep}{\ensuremath{\mathcal{D}_g(\vecu,\delta)}\xspace}

\newcommand{\hinge}{\ensuremath{h_{\delta}}\xspace}

\newcommand{\Beam}{\ensuremath{\mathcal{B}}\xspace}

% equivalence class under ~: [[x]]_~
\newcommand{\eqvcls}[1]{\ensuremath{\llbracket {#1} \rrbracket_{\equiv}}\xspace}

\newcommand{\Cs}{\ensuremath{C_{\mathrm{s}}}}
\newcommand{\Cg}{\ensuremath{C_{\mathrm{g}}}}
\newcommand{\Cb}{\ensuremath{C_{\mathrm{b}}}}

\newcommand{\state}{\ensuremath{\mathit{state}}\xspace}
\newcommand{\action}{\ensuremath{\mathit{action}}\xspace}


\newcommand{\fkerdp}[1]{\ensuremath{\vecfker_{{\mathrm{DP}}}({#1})}\xspace}
\newcommand{\fkernodp}[1]{\ensuremath{\vecfker_{\mathrm{noDP}}({#1})}\xspace}

\newcommand{\score}{\ensuremath{\mathit{S}}\xspace}
\newcommand{\scoring}[2]{\ensuremath{\score_{#1}({#2})}\xspace}
\newcommand{\scoresh}[1]{\ensuremath{\scoring{\shift}{#1}}\xspace}
\newcommand{\scoreleft}[1]{\ensuremath{\scoring{\lreduce}{#1}}\xspace}
\newcommand{\scoreright}[1]{\ensuremath{\scoring{\rreduce}{#1}}\xspace}

\newcommand{\leftptrs}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\rightptrs}{\ensuremath{\mathcal{R}}\xspace}

\newcommand{\chart}{\ensuremath{\mathit{C}}\xspace}
\newcommand{\pq}{\ensuremath{\mathit{Q}}\xspace}

\newcommand{\bleu}{{\sc Bleu}\xspace}
\newcommand{\bleuplusone}{\ensuremath{\mathrm{Bleu}^{+1}}\xspace}
\newcommand{\mert}{{\sc Mert}\xspace}
\newcommand{\ce}{{\sc Ch-En}\xspace}
\newcommand{\se}{{\sc Sp-En}\xspace}
\newcommand{\pro}{{\sc Pro}\xspace}
\newcommand{\mira}{{\sc Mira}\xspace}
\newcommand{\hols}{{\sc Hols}\xspace}
\newcommand{\ramp}{{\sc Ramp}\xspace}
\newcommand{\hiero}{{\sc Hiero}\xspace}
\newcommand{\cdec}{{\tt cdec}\xspace}

\newcommand{\MaxForce}{{\sc MaxForce}\xspace}

\newcommand{\myinfer}[3]{\ensuremath{\infer[\mbox{\footnotesize ${#1}$}]{#2}{#3}}\xspace}
\newcommand{\pre}{\ensuremath{\mathit{pre}}\xspace}
\newcommand{\good}{\ensuremath{\mathit{good}}\xspace}
\newcommand{\bad}{\ensuremath{\mathit{bad}}\xspace}
\newcommand{\ygood}{\ensuremath{\mbox{$y$-good}}\xspace}
\newcommand{\ybad}{\ensuremath{\mbox{$y$-bad}}\xspace}

\newcommand{\cn}{\ensuremath{{\sf cn}}\xspace}
\newcommand{\en}{\ensuremath{{\sf en}}\xspace}

\newcommand{\kNN}{\ensuremath{\mbox{$k$-NN}}\xspace}

\newcommand{\Yahoo}{{\sc Yahoo}\xspace}
\newcommand{\TREC}{{\sc TREC}\xspace}
\newcommand{\DMV}{{\sc DMV}\xspace}
\newcommand{\Insurance}{{\sc Insurance}\xspace}


\def\lr{\mbox{\begin{picture}(7,10)
\put(1,0){\line(1,0){5}}
\put(1,0){\line(1,2){5}}
\put(6,0){\line(0,1){10}}
\end{picture}
}}

\def\ll{\mbox{\begin{picture}(7,10)
\put(1,0){\line(1,0){5}}
\put(6,0){\line(-1,2){5}}
\put(1,0){\line(0,1){10}}
\end{picture}
}}

\def\llbig{\mbox{\begin{picture}(25,10)
\put(1,0){\line(1,0){30}}
\put(31,0){\line(-3,1){30}}
\put(1,0){\line(0,1){10}}
\end{picture}
}}

\def\lrbig{\mbox{\begin{picture}(25,10)
\put(1,0){\line(1,0){30}}
\put(1,0){\line(3,1){30}}
\put(31,0){\line(0,1){10}}
\end{picture}
}}
\newcommand{\doubleitem}[2]{\ensuremath{\stackrel{\!\!\!\!\!{#1}}{\ll} \stackrel{\ {#2}}{\lr}}\xspace}

\newcommand{\doubleitemleft}[2]{\ensuremath{\stackrel{\hspace{-0.9cm}{#1}}{\llbig} \quad \stackrel{\ {#2}}{\lr}}\xspace}


\newcommand{\doubleitemright}[2]{\ensuremath{\stackrel{\!\!\!\!\!{#1}}{\ll} \; \stackrel{\hspace{1.1cm} {#2}}{\lrbig}}\xspace}

\newcommand{\pytorch}{PyTorch\xspace}
\newcommand{\rnnsearch}{RNNsearch\xspace}

\newcommand{\best}{\ensuremath{\mathit{best}}\xspace}
\newcommand{\bestuptoi}{\ensuremath{\mathit{best}_{\leq i}}\xspace}
\newcommand{\completed}{\ensuremath{\mathit{comp}}\xspace}
\newcommand{\eos}{\mbox{\scriptsize \texttt{<eos>}}\xspace}
\newcommand{\bp}{\ensuremath{\mathit{bp}}\xspace}
\newcommand{\BLEU}{\ensuremath{\mathrm{BLEU}}\xspace}
\newcommand{\PWR}{\ensuremath{\mathrm{PWR}}\xspace}
\newcommand{\AdaR}{\ensuremath{\mathrm{AdaR}}\xspace}
\newcommand{\gnmt}{\ensuremath{\mathrm{GNMT}}\xspace}
\newcommand{\lengthnorm}{\ensuremath{\mathrm{length\_norm}}\xspace}
\newcommand{\word}{\ensuremath{\mathrm{word}}\xspace}
\newcommand{\len}{\ensuremath{\mathit{len}}\xspace}
\newcommand{\gratio}{\ensuremath{\mathit{gr}}\xspace}
\newcommand{\lratio}{\ensuremath{\mathit{lr}}\xspace}
\newcommand{\pred}{\ensuremath{\mathit{pred}}\xspace}

\newcommand{\spinyin}[1]{{\small\em {#1}}}
\newcommand{\bajisitan}{B\=aj\={\i}s\={\i}t\v{a}n}
\newcommand{\yindu}{Y\`{\i}nd\`u}

\newcommand{\deen}{{{de}$\leftrightarrow${en}}\xspace}
\newcommand{\zhen}{{{zh}$\leftrightarrow${en}}\xspace}
\newcommand{\detoen}{{{de}$\goesto${en}}\xspace}
\newcommand{\entode}{{{en}$\goesto${de}}\xspace}
\newcommand{\zhtoen}{{{zh}$\goesto${en}}\xspace}
\newcommand{\entozh}{{{en}$\goesto${zh}}\xspace}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\gwaitk}{\ensuremath{{g_\text{wait-$k$}}}\xspace}
\newcommand{\gcatchup}{\ensuremath{{g_\text{wait-$k$, $c$}}}\xspace}

\newcommand{\CW}{\ensuremath{\mathrm{CW}}\xspace}
\newcommand{\AP}{\ensuremath{\mathrm{AP}}\xspace}
\newcommand{\AL}{\ensuremath{\mathrm{AL}}\xspace}


==> simul-acl copy 2/detail.tex <==
% !TEX root = main.tex
%\subsection{Wait-$k$ with RNNs}
%% We first introduce our uni-directional RNN-based approach as one baseline to set up a fair comparison 
%% with other methods.
% For simplicity, we only use uni-directional RNN.

While RNN-based implementation of our wait-$k$ model is straightforward
and our initial experiments showed equally strong results,
due to space constraints we will only present Transformer-based results.
Here we describe the implementation details for training a prefix-to-prefix Transformer,
which is a bit more involved than RNN.

\iffalse
\subsection{Background: Full-Sentence RNN}
%For the basic RNN-based framework, on the encoder side, the RNN %recursively
The (unidirectional) RNN encoder maps a sequence  $\vecx$ into a sequence of hidden states: % as follows:
\begin{equation*}
\overrightarrow{h}_i = \text{RNN}(x_i, \overrightarrow{h}_{(i-1)};\theta_e),
\label{eq:rnnencoder}
\end{equation*}
Then list of hidden states $\vech$ now represent the %context from
source side.
%% Since we are using uni-directional RNN,
%% we could easily append the new coming word with constant time to the encoder.
%On the other side,
The decoder takes another RNN to generate the target side hidden 
representations at decoding step $t$:% as follows:
\begin{equation}
\overrightarrow{s_t} = \text{RNN}(\overrightarrow{s}_{(t-1)},\vech;\theta_d)
\label{eq:rnndecoder}
\end{equation}
%The encoder and decoder are parameterized by $\theta_{e}$ and $\theta_{d}$, respectively. 
%% Note that the decoder takes the entire source context $\vech$ as input during generation 
%% for each step.

\subsection{Training Simultaneous RNN}
Different from full-sentence translation, in simultaneous translation, 
the source words are fed into the encoder %system
one by one. %after $k$ words delay.
%% As mentioned above, during encoding, we could just simply append the new coming words to the 
%% end of the existing encoder.
For decoding, we need to change Eq.~\ref{eq:rnndecoder} %into following definition:
to predict using source prefix:
\begin{equation*}
\overrightarrow{s_t} = \text{RNN}(\overrightarrow{s}_{(t-1)},\vech_{\leq g(t)};\theta_d)
\label{eq:rnndecoder2}
\end{equation*}
%% where $\vech_{\leq g(t)}$ indicates that the decoder only can observe the first $g(t)$ 
%% hidden states from encoder.
%% Decoder waits for $k$ words on source side, then starts generating a new word 
%% once there is another words are feed  into the encoder side.

%% Beside RNN-based, in order to improve our system's performance even further,
%% we also design a Transformer-based framework. 

%\subsection{Wait-$k$ with Transformer}
% For the sake of the remarkable performance, we also re-design our simultaneous 
% Neural Machine Translation frameworks based on Transformer.
%% Due to the remarkable performance of the Transformer \cite{vaswani+:2017}, we renovate the 
%% Transformer framework into an simultaneous machine 
%% translation framework with arbitrary latency constraints.

\fi

\subsection{Background: Full-Sentence Transformer}

We first briefly review the Transformer architecture step by step %with stepwise point of view
to highlight the difference between the conventional and simultaneous Transformer.
The encoder of Transformer works in a self-attention fashion and takes an input 
sequence $\vecx$,
and produces a new sequence of hidden states $\vecz = (z_1,...,z_n)$ 
where $z_i \in \mathbb{R}^{d_z}$ is as follows:
\begin{equation}
z_i = \textstyle\sum_{j=1}^n \alpha_{ij} \;  P_{W_\text{V}}(x_j)
\label{eq:weightedcontext}
\end{equation}
Here $P_{W_\text{V}}(\cdot)$ is a projection function from the input space to the value space, % with parameter $W_\text{V}$,
and $\alpha_{ij}$ denotes the attention weights: % which are computed with a softmax function:
\begin{equation}
  \alpha_{ij}\!=\!\frac{\exp e_{ij}}{\sum_{l=1}^n \exp e_{il}},
  \; e_{ij}\!=\!\frac{P_{W_\text{Q}}(x_i) P_{W_\text{V}}(x_j)^T} {\sqrt{d_x}}
\label{eq:simisoft}
\end{equation}
where $e_{ij}$ measures similarity between inputs. %two elements:
%% \begin{equation}
%% e_{ij} = \frac{P_{W_\text{Q}}(x_i) \; P_{W_\text{V}}(x_j)^T} {\sqrt{d_x}}
%% \label{eq:simieq}
%% \end{equation}
Here $P_{W_\text{Q}}(x_i)$ and $P_{W_\text{K}}(x_j)$ project $x_i$ and $x_j$ to query and key spaces, resp.
%with parameters  $W_\text{Q}$ and ${W_\text{K}}$.
%% When more self-attention layers are needed, these projection parameters 
%% are unique for each layer and attention head.
We use 6 layers of self-attention %in our model 
and use $\vech$ to denote the top layer output sequence (i.e., the source context).

On the decoder side, during training time, the  gold output sequence 
$\vecy^* = (y_1^*,...,y_m^*)$ goes 
through the same  self-attention to generate hidden self-attended 
state sequence $\vecc = (c_1,...,c_m)$. 
Note that because decoding is incremental, we let $\alpha_{ij} = 0$ if $j>i$ in Eq.~\ref{eq:simisoft}
to restrict  self-attention to previously generated words.
% for the $i^{th}$ given word.

In each layer, after we gather all the hidden representations for each target word 
through self-attention,
we perform target-to-source attention: % as follows:
% similar to Eq.~\ref{eq:weightedcontext} to 
% Eq.~\ref{eq:simieq} as 
\begin{equation*}
c'_i = \textstyle\sum_{j=1}^n \beta_{ij} \;  P_{W_{\text{V}'}}(h_j)
\end{equation*}
similar to self-attention, $\beta_{ij}$ measures the similarity between $h_j$ and $c_i$ 
as in Eq.~\ref{eq:simisoft}. %--\ref{eq:simieq}.  
%% After stacking several layers 
%% of above operations, we use $\vecs$ to denote the top layer's output.


\subsection{Training Simultaneous  Transformer}

% As mentioned above, 
% simultaneous translation needs to start generating translations before the input
% sentence finishes.
Simultaneous translation requires feeding the source 
words incrementally to the encoder,
but a naive implementation of such
incremental encoder/decoder is inefficient.
Below we describe a faster implementation.
%% and the decoder also needs to predict a new target word once 
%% the encoder gets a new source word. 
%% Obviously, training the incremental encoder and decoder is inefficient.
%% In order to train our framework with above requirements efficiently, we need to 
%% make several modifications on both encoder and decoder sides.

For the encoder, during training time, 
we still feed the entire sentence at once %at one time 
to the encoder. 
But different from the self-attention layer % which is 
in conventional Transformer (Eq.~\ref{eq:simisoft}),
we constrain each source word to 
attend to its predecessors only (similar to decoder-side self-attention),
effectively simulating an incremental encoder: % to the prefix of sentence as follows:
\begin{equation*}
  \alpha^{(t)}_{ij} = \left\{\begin{matrix}  
  \frac{\exp e^{(t)}_{ij}}{\sum_{l=1}^{g(t)} \exp e^{(t)}_{il}}  & \text{if} \;\; {i,j}  \leq g(t)  \\[0.05cm]
  0 &\text{otherwise}
  \end{matrix}\right.
\label{eq:simulsoft}
\end{equation*}
\begin{equation*}
e^{(t)}_{ij} =  \left\{\begin{matrix} 
\frac{P_{W_\text{Q}}(x_i) \; P_{W_\text{K}}(x_j)^T} {\sqrt{d_x}} & \text{if} \;\; {i,j}  \leq g(t)  \\[0.05cm]
-\infty  & \text{otherwise}
\end{matrix}\right. 
\label{eq:simulweights}
\end{equation*}
%% when both $i$ and $j$ are bounded by $g(t)$, 
%% % where $k \in [1,n]$ is latency constraint, 
%% % e.g., wait $3$ words, 
%% and set $\alpha^{(t)}_{ij}$ to $0$ otherwise (just like the decoder-side self-attention). 
%% The translation time step is represented by $t$. 
%% For example, when we are at the $4^{th}$ translation step with $3$-words latency,
%% there are $7$ words in the stack of encoder and $4$ words have been 
%% translated by decoder.
%% And we redefine the Eq.~\ref{eq:simieq} as follows:

Then we have a newly defined hidden state sequence 
$\vecz^{(t)}= (z^{(t)}_1,...,z^{(t)}_n)$ at decoding step $t$:
%$z^{(t)}_i$ is as follows:
\begin{equation}
z^{(t)}_i = \textstyle\sum_{j=1}^n \alpha^{(t)}_{ij} \;  P_{W_\text{V}}(x_j)
\label{eq:weightedcontextwitht}
\end{equation}
When a new source word is received,
all previous source words need to adjust their representations.
%% every word which is prior to the new word $g(t)$ on the source side 
%% needs to adjust its' existing representation to a new 
%% representation in order to absorb the new word's information.
%% In words, $z^{(4)}_2$ is different from $z^{(3)}_2$ since 
%% there is one extra word which has been feed into source side.
%The above self-attention layer only allows each word to attend to its , which 
%% generates equivalent representations to the incremental scenario since every word is 
%% blind to the latter words.
%% When we stack more prefix-to-prefix self-attention blocks, the earlier source words are still immune to 
%% the later source words' information. In this way, we simulate the incremental environment
%% when the full source sentence are fed once during training time.

% However, there is still another problem for encoder's context representation generation.


\iffalse
\subsubsection{Context Caching}

The way Transformer generating context representation is different 
from RNN-based framework, especially uni-directional RNN-based models.
In uni-directional RNN-based model, since each word's hidden 
representation only depends on previous state, 
when there is an new word which is append to the source sentence, 
all the representation from prefix words are unchanged.
However, this is different in Transformer due to the self-attention mechanism.

As we observe from the definitions of $\alpha_{ij}$ and $e_{ij}$, when there is another 
word that has been fed into encoder, the translation time step 
increments from $t$ to $t+1$. 
Every word which is prior to the new word $k+t+1$ on the source side 
needs to adjust its' existing representation to a new 
representation in order to absorb the new word's information.
Therefore, different from conventional Transformer, our framework has 
a list of incremental source side context information instead of 
only one tensor $\vech$ in previous section to represent the entire source side.
Our source side context is defined as follows:

\begin{equation*}
\mathbb{L} = [\vech_{[:k]}, \vech_{[:k+1]},...,\vech_{[:n-k]}]
\label{eq:contextlist}
\end{equation*}
where $n$ is the total length of source sentence, and $\vech_{[:k+i]}$ 
represents the context representation of the first $(k+i)^{th}$ words.
Note that $\vech_{[:n-k]}$ equals to $\vech$ in previous section.

On the other hand, for the source-target attention on decoder side, 
at translation step $t$, the decoder only can observe the $t^{th}$ context 
in $\mathbb{L}$.
\fi











==> simul-acl copy 2/exps.tex <==
% !TEX root = main.tex

% \begin{figure*}[!t]%[t]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=7cm]{figs/for_TACL/Fig1a_de2en_AP_dev.pdf}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=7cm]{figs/for_TACL/Fig1b_en2de_AP_dev.pdf}
% \end{subfigure}%
% \captionof{figure}{BLEU scores and AP comparisons with \namecite{gu+:2017} for different wait-$k$ models on German-to-English (left figure) and English-to-German (right figure). \textcolor{colorC0}{$\bigstar$\ding{73}} are greedy decoding and beam-search (beam-size 11) results with Transformer model. Line plots \textcolor{colorC0}{\scriptsize$\blacksquare$} and \textcolor{colorC1}{$\bullet$} are our results with Transformer and RNN models with different wait-$k$. 
% Point-pairs are the results of simultaneous
% greedy decoding and beam-search (beam-size 5)
% respectively with models \cite{gu+:2017} trained with various delay targets:
% $\bigstar$\ding{73}:Wait-Until-End, %$\bigwhitestar
%  \textcolor{PaleGreen}{{$\blacktriangleleft$}$\lhd $}:CW=8,
%  \textcolor{PaleGreen}{$\blacktriangle$$\vartriangle$}:CW=5,
%  \textcolor{PaleGreen}{{$\blacklozenge$}$\diamondsuit$}:CW=2,
%  \textcolor{red}{{$\blacktriangleright$}$\rhd$}:AP=0.3,
%  \textcolor{red}{$\blacktriangledown${$\triangledown$}}:AP=0.5,
%  \textcolor{red}{$\blacksquare$$\square$}:AP=0.7.}
% \label{fig:bleuAP_en2de_test}
% \end{figure*}



% \begin{figure*}[!t]%[t]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=7cm]{figs/for_TACL/Fig2a_de2en_AL_dev.pdf}
% \end{subfigure}%
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=7cm]{figs/for_TACL/Fig2b_en2de_AL_dev.pdf}
% \end{subfigure}%
% \captionof{figure}{BLEU scores for wait-$k$ models on EN2DE test set with latency measured by AL. \textcolor{colorC0}{$\bigstar$\ding{73}} and  \textcolor{colorC1}{$\bigstar$\ding{73}} are greedy decoding and beam-search baselines for Transformer and RNN model respectively.}
% \label{fig:bleuAL_en2de_test}
% \end{figure*}


\begin{figure*}
\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_de2en_AL_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_de2en_CW_test.pdf}
\end{tabular}\\[-0.4cm]
\captionof{figure}{Translation quality against latency metrics (AL and CW) on German-to-English simultaneous translation,
  showing wait-$k$ % (for $k$=1, 3, 5, 7, 9) 
  and test-time wait-$k$ results, full-sentence baselines, and our adaptation of \namecite{gu+:2017}
 (\textcolor{red}{{$\blacktriangleright$}}:CW=2;
  \textcolor{red}{$\blacktriangledown$}:CW=5;
  \textcolor{red}{$\blacksquare$}:CW=8),
  all based on the same Transformer.
%%   BLEU score and AP comparisons with \namecite{gu+:2017} for different wait-$k$ models on German-to-English (left) and English-to-German (right). \textcolor{colorC1}{$\bigstar$\ding{73}} are full-sentence baselines with RNNs (greedy decoding and beam-search with beam-size 11, resp.). Line plots \textcolor{colorC1}{$\bullet$} and \textcolor{colorC1}{$\circ$} are our  wait-$k$ policy's greedy and tail beam search results with RNNs. 
%% Point-pairs are the results from \namecite{gu+:2017} %of simultaneous
%% using greedy decoding and beam-search (beam-size 5)
%% %respectively
%% with models  trained with various delay targets:
\textcolor{colorC0}{$\bigstar$\ding{73}}:full-sentence (greedy and beam-search).%$\bigwhitestar
 %% \textcolor{PaleGreen}{{$\blacktriangleleft$}$\lhd $}:CW=8,
 %% \textcolor{PaleGreen}{$\blacktriangle$$\vartriangle$}:CW=5,
 %% \textcolor{PaleGreen}{{$\blacklozenge$}$\diamondsuit$}:CW=2,
 %% \textcolor{red}{$\blacktriangleright$}:AP=0.3,
 %% \textcolor{red}{$\blacktriangledown$}:AP=0.5,
% and models trained with AP=0.7 achieve a test-time AP around 0..
}
\label{fig:APCW_de2en}
\smallskip

\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2de_AL_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2de_CW_test.pdf}
\end{tabular}\\[-0.4cm]
\captionof{figure}{
  Translation quality against latency metrics on English-to-German simultaneous translation.
%  \namecite{gu+:2017}:
%  \textcolor{red}{{$\blacktriangleright$}}:CW=2;
%  \textcolor{red}{$\blacktriangledown$}:CW=5;
%  \textcolor{red}{$\blacksquare$}:CW=8.
%%   BLEU scores  for wait-$k$ models on German-to-English and English-to-German with latency measured by AL. \textcolor{colorC0}{$\bigstar$\ding{73}} and  \textcolor{colorC1}{$\bigstar$\ding{73}} are greedy decoding and beam-search baselines for Transformer and RNN models respectively. \
%% Similarly, \textcolor{colorC0}{\scriptsize$\blacksquare$} and \textcolor{colorC1}{$\bullet$} are decoded using greedy strategy, while \textcolor{colorC0}{\scriptsize$\square$} and \textcolor{colorC1}{$\circ$} are decoded with tail beam search.
%% \textcolor{red}{$\blacktriangledown$}:AP=0.5 and
%% \textcolor{red}{$\blacksquare$}:AP=0.7 are the same points from Fig.~\ref{fig:bleuAP_en2de_test}.
}
\label{fig:APCW_en2de}


\smallskip

\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_zh2en_AL_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_zh2en_CW_test.pdf}
\end{tabular}\\[-0.4cm]
\captionof{figure}{
  Translation quality against latency on Chinese-to-English simultaneous translation.
%  \namecite{gu+:2017}:
%  \textcolor{red}{{$\blacktriangleright$}}:CW=2;
%  \textcolor{red}{$\blacktriangledown$}:CW=5;
%  \textcolor{red}{$\blacksquare$}:CW=8.
    %???.{$\bigstar$\ding{73}} and  \textcolor{colorC0}{$\bigstar$\ding{73}} are greedy decoding and beam-search baselines.
}
\label{fig:APCW_zh2en}

\smallskip
%\end{figure*}


%\begin{figure*}
\begin{tabular}{cc}
\centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2zh_AL_test.pdf} & \centering
  \includegraphics[width=7.cm]{figs/for_acl/Fig_acl_en2zh_CW_test.pdf}
\end{tabular}\\[-0.4cm]
\captionof{figure}{
  Translation quality against latency  on English-to-Chinese, with encoder catchup (see Appendix~\ref{sec:catchup}). 
  %with one extra word every even step. %English-to-Chinese. % simultaneous translation.
% \namecite{gu+:2017}:
%  \textcolor{red}{{$\blacktriangleright$}}:CW=2;
%  \textcolor{red}{$\blacktriangledown$}:CW=5;
%  \textcolor{red}{$\blacksquare$}:CW=8.x`
%% BLEU scores and AL comparisons with different wait-$k$ models on Chinese-to-English (left) and English-to-Chinese (right)
%% translations on dev set. Note that we use 4-ref BLEU for Chinese-to-English but 1-ref BLEU for English-to-Chinese since the multiple references are only available on English side.
%% %\textcolor{colorC0}{$\bigstar$\ding{73}} are greedy decoding and beam-search baselines.
}
\label{fig:APCW_en2zh}
\end{figure*}



% !TEX root = main.tex
%% This section first presents the accuracy and latency of our proposed wait-$k$ model. 
%% Then, we demonstrate that our catchup model reduces the latency even further with
%% a little sacrifice of accuracy.
%% We analyse some examples from the dev set and 
%% recent news at the end.
% Following the works from~\namecite{Cho+:16,Gu+:2017}, we also use Average Proportion (AP)
% to measure the latency between different systems. 
% Formally, AP is defined as follows:

% \begin{equation*}
% AP = \frac{1}{|X|\;|Y|} \sum_{\tau} p(\tau) 
% \label{eq:AP}
% \end{equation*}
% where $p(\tau)$ measures the number of source words been waited when decoding the 
% $i^{th}$ on target side.

\vspace{-0.2cm}
\subsection{Datasets and Systems Settings}

We evaluate our work on four simultaneous translation directions:
%The performance of our models are demonstrated on both 
German$\leftrightarrow$English and Chinese$\leftrightarrow$English.
% translation tasks. 
For the training data, we use the parallel corpora available from WMT15\footnote{\!\!\!\scriptsize\url{http://www.statmt.org/wmt15/translation-task.html}}
for German$\leftrightarrow$English (4.5M sentence pairs) and 
NIST corpus for Chinese$\leftrightarrow$English (2M sentence pairs).
We first apply BPE~\cite{sennrich+:2015} on all texts in order 
to reduce the vocabulary sizes. % for both source and target sides.
%% We then exclude sentences pairs whose length are longer than 50 and 256 words
%% for English-to-German and Chinese-to-English respectively.
For German$\leftrightarrow$English evaluation, 
we use newstest-2013 (dev) as our dev set and newstest-2015 (test) as our test set,
with 3,000 and 2,169 sentence pairs, respectively.
For Chinese$\leftrightarrow$English evaluation,
we use NIST 2006 and 
NIST 2008 as our dev and test sets.
They contain 616 and 691 Chinese sentences, each with 4 English references.
When translating from Chinese to English, we report 4-reference BLEU scores,
and in the reverse direction, we use the second among the four English references as the source text,
and report 1-reference BLEU scores.
%% In the catchup experiments, we use the decoding catchup frequency of $c=0.25$
%% %pattern $1-1-1-2$
%% which is derived from the dev set tgt/src length ratio of 1.25.
%% %from source side to target side. 
%% %The length ratio of 1.25 is from training corpus.
%% For \deen translation task,
%% we do not need catch since the tgt/src ratio is almost 1.

% The performance of our models are demonstrated on NIST Chinese-to-English translation
% corpus which consists of two million translation pairs between Chinese and English 
% sentences. 
% We first apply BPE~\cite{sennrich+:2015} on both sides in order 
% to reduce the vocabulary for both Chinese and English down to
% 18K and 10K respectively.
% We then exclude the sentences pairs whose length are longer than $256$ words
% on source or target sides.
% We use NIST 06 (616 sentence pairs) and NIST 08 (691 sentence pairs) as our 
% development and testing set.

% In the following experiments, we report 1-reference, 3-reference and 
% 4-reference BLEU scores to compare different models.
% Note that the human reference translations are obtained from non-simultaneous scenarios.
%and reference %human performance.

Our implementation is adapted from PyTorch-based OpenNMT \cite{klein+:2017}.
Our Transformer is essentially the same as the base model from % the base model's parameter settings in 
the original paper \cite{vaswani+:2017}.


%% \begin{table}
%% \centering
%% \resizebox{0.48\textwidth}{!}{
%% \begin{tabular}{ | c |c |c |c |c |c |}
%% \hline
%% \color{red} \detoen & $k$=3 & $k$=4 & $k$=5 & $k$=6 & Gu et al.  \\
%% \hline
%% CW  &  1.35 & 1.43 & 1.54 & 1.65 & 3.85  \\
%% \hline
%% BLEU & 18.54 & 19.78 & 20.53 & 21.23 & 20.07 \\
%% \hline
%% \hline
%% \color{red}\entode & $k$=3 & $k$=4 & $k$=5 & $k$=6 & Gu et al.  \\
%% \hline
%% CW & 1.13 & 1.22& 1.33 & 1.48 & 3.36  \\
%% \hline
%% BLEU & 15.40 & 16.41 & 17.24 & 17.56 & 15.93  \\
%% \hline
%% \end{tabular} 
%% }
%% \caption{Compare with \cite{gu+:2017} on dev set with CW and BLEU score. At similar or higher BLEU levels, our models enjoy much lower CWs.}
%% \label{tb:comparecw}
%% \end{table}







\if
%\subsection{Background: Latency Metrics (AP, CW)}

Before presenting our experiments, we first explain below the two standard latency metrics for simultaneous translation. %: AP and CW.
Consecutive Wait (CW)  \cite{gu+:2017} measures the average lengths of conseuctive wait segments
(the best case is 1 for our wait-1 and the worst case is $|\vecx|$ for full-sentence MT).
%%  (CW) \cite{gu+:2017} is the number of source words
%% waited between two target words. %Using our notation,
For a policy $g(\cdot)$, the per-step CW at step $t$ is
\(
\CW_g(t) = g(t) - g(t-1).
\)
The CW of a sentence-pair $(\vecx, \vecy)$ is the average CW over all consecutive wait segments:
\[
\resizebox{.48\textwidth}{!}{
  $\CW_g(\vecx,\vecy) = \displaystyle\frac{\sum_{t=1}^{|\vecy|} \CW_g(t)}{\sum_{t=1}^{|\vecy|} \mathbbm{1}_{\CW_g(t) > 0}} = \frac{|\vecx|}{\sum_{t=1}^{|\vecy|} \mathbbm{1}_{\CW_g(t) > 0}}$
  }
\]
\vspace{-0.3cm}
%% defines the consecutive waits while 
%% translating each target word. It describes the length of silence 
%% between two translated adjacent words.
%% For each READ or WRITRE action, we have the CW definition as follows:

%% \begin{equation*}
%% c_t=\left\{\begin{matrix}
%%  c_{t-1} + 1& a_t \; \text{is READ}  & \\ 
%%  0& \;\;a_t \; \text{is WRITE}  & 
%% \end{matrix}\right.
%% \label{eq:CW}
%% \end{equation*}
%% where $a_t$ is the action at $t^{th}$ time step and $c_t$ is the number of 
%% waited words between two adjacent translated words.
%The drawback of CW is its insensitivity to the actual lagging behind as discussed in the previous Section;
%for example, catchup has no effect on CW.
Another latency measurement, Average Proportion (AP) \cite{Cho+:16} measures
%focuses on the global latency 
%which is defined as follows:
the proportion of the area above a policy path in Fig.~\ref{fig:idea}:
\vspace{-0.2cm}
\begin{equation}
\AP_g(\vecx,\vecy) = \frac{1}{|\vecx|\;|\vecy|} \textstyle\sum_{t=1}^{|\vecy|} g(t) 
\label{eq:AP}
\end{equation}
\fi


\vspace{-0.3cm}
\subsection{Quality and Latency of Wait-$k$ Model}
\vspace{-0.1cm}

\begin{table}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ | c |c |c |c |c |c |c | }
\hline
\diagbox{\!Train}{\! Test} & $k$=1 & $k$=3 & $k$=5 & $k$=7 & $k$=9 & $k$=$\infty$ \\
%\diagbox{$k$}{$k'$} & 1 & 3 & 5 & 7 & 9 & $\infty$ \\ \hline
%decode-$k$ & \multirow{2}{*}{1} & \multirow{2}{*}{3} & \multirow{2}{*}{5} & \multirow{2}{*}{7} & \multirow{2}{*}{9} & \multirow{2}{*}{$\infty$} \\
%\cline{1-1}
%train-$k$ &&&&&&\\
\hline
$k'$=1 & {\em 34.1} & 33.3 & 31.8 & 31.2 & 30.0 & 15.4 \\ \hline
$k'$=3 & {\bf 34.7} & 36.7 & {\em 37.1} & 36.7 & 36.7 & 18.3 \\ \hline
$k'$=5 & 30.7 & 36.7 & 37.8 & 38.4 & {\em 38.6} & 22.4 \\ \hline
$k'$=7 & 31.0 & {\bf 37.0} & {\bf 39.4} & {\em 40.0} & 39.8 & 23.7 \\ \hline
$k'$=9 & 26.4 & 35.6 & 39.1 & {\bf 40.1} & {\bf {\em 41.0}} & 28.6 \\ \hline
$k'$=$\infty$ & 21.8 & 30.2 & 36.0 & 38.9 & 39.9 &  {\bf {\em 43.2}}\\ \hline

%$k'$=1 & {\em 34.3} & 31.5 & 31.2 & 31.1 & 30.4 & 19.2 \\ \hline
%$k'$=3 & {\bf 34.9} & 36.2 & 37.2 & {\em 37.7} & 37.3 & 19.5 \\ \hline
%$k'$=5 & 30.4 & {\bf 36.8} & {\bf 38.8} & 38.9 & {\em 39.0} & 24.3 \\ \hline
%$k'$=7 & 30.6 & 36.6 & 38.6 & {\em 39.4} & 39.1 & 23.1 \\ \hline
%$k'$=9 & 27.4 & 34.7 & 38.5 & {\bf 39.9} & {\em 40.6} & 27.4 \\ \hline
%$k'$=$\infty$ & 26.2 & 32.7 & 36.9 & 39.3 & {\bf 41.0} &  {\bf {\em 43.7}}\\ \hline


%%%%%%% last:43.72/46.88
% \diagbox{$k$}{$k'$} & 1 & 3 & 5 & 7 & 9 & $\inf$ \\ \hline
% 1 & 34.3 & 31.5 & 31.2 & 31.1 & 30.4 & 19.2 \\ \hline
% 3 & 34.8 & 36.2 & 37.2 & 37.7 & 37.3 & 19.5 \\ \hline
% 5 & 30.4 & 36.8 & 38.8 & 38.9 & 39.0 & 24.3 \\ \hline
% 7 & 30.6 & 36.6 & 38.6 & 39.4 & 39.1 & 23.1 \\ \hline
% 9 & 27.4 & 34.7 & 38.5 & 39.9 & 40.6 & 27.4 \\ \hline
% $\inf$ & 26.2 & 32.7 & 36.9 & 39.3 & 41.0 &  \\ \hline
\end{tabular} 
}
\caption{wait-$k$ policy  in training and test
  (4-ref BLEU, \zhtoen dev set). The bottom row is ``test-time wait-$k$''.
Bold: best in a column; italic: best in a row.}
\label{tb:combo}
\vspace{-.3cm}
\end{table}

%As a first experiment,
Tab.~\ref{tb:combo} shows the results
of a model trained with wait-$k'$
but decoded with wait-$k$ (where $\infty$ means full-sentence).
Our wait-$k$ is the diagonal,
and the last row is the ``test-time wait-$k$'' decoding.
%(using full-sentence model).
Also, the best results of wait-$k$ decoding is often
from a model trained with a slightly larger $k'$.

%Fig.~\ref{fig:bleuWaitk_dev1} shows the accuracy and latency comparison between ``wait-$k$''
%and catchup model with 1-reference and 4-reference BLEU measurement. 
%We also show the baseline performance in each figure.
%From the number of waited words point of view,
%there is a bigger accuracy gap between ``wait-$k$'' and catchup model at each $k$ step.


% For Fig.~\ref{fig:bleuAP_dev1} and Fig.~\ref{fig:bleuAL_dev1}, we compare the accuracy and different latency measurements for both wait-$k$ and catchup models on development set.
% As it is shown, we note that the wait-4 catchup model has similar latency
% with wait-1 model. This demonstrates that our catchup model indeed improves the latency
% especially for the long sentences.
% Our test set data comparison is shown in Table~\ref{tb:waitktest}. 
% Note that our ``wait-2'' has smaller AP than ``wait-1'' model.


%\begin{figure}%[t]
%\centering
%\begin{minipage}[t]{0.48\textwidth}
%\centering
%\includegraphics[width=7cm]{figs/bleu/bleu_waitk_dev_4refs.pdf}
%\end{minipage}
%\begin{minipage}[t]{0.48\textwidth}
%\includegraphics[width=7cm]{figs/bleu/bleu_waitk_dev_ref2.pdf}
%\end{minipage}
%\captionof{figure}{Accuracy for ``wait-$k$'' and catchup models with 1-ref and 4-ref BLEU.
%Latency is measured by number delayed words.}
%\label{fig:bleuWaitk_dev1}
%\vspace{0cm}
%\end{figure}


% \begin{figure}[!t]%[t]
% \centering
% % \hspace{-0.8cm}
% % \begin{minipage}[t]{0.48\textwidth}
% % \centering
% % \includegraphics[width=7cm]{figs/bleu/bleu_AP_dev_4refs.pdf}
% % \end{minipage}
% % \begin{minipage}[t]{0.48\textwidth}
% \includegraphics[width=7cm]{figs/bleu/bleu_AP_dev_ref2.pdf}
% % \end{minipage}
% \captionof{figure}{BLEU scores for wait-$k$ with Transformer (and its catchup version) and wait-$k$ with RNN model on ZH2EN dev set with 1-ref BLEU.
% Latency is measured by AP.}
% \label{fig:bleuAP_dev1}
% \end{figure}

% \begin{figure*}[!t]%[t]
% \centering
% % \hspace{-0.8cm}
% % \begin{minipage}[t]{0.48\textwidth}
% % \centering
% % \includegraphics[width=7cm]{figs/bleu/bleu_AL_dev_4refs.pdf}
% % \end{minipage}
% % \begin{minipage}[t]{0.48\textwidth}
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=7cm]{figs/for_TACL/Fig3a_zh2en_AL_dev.pdf}
% \end{subfigure}
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=7cm]{figs/for_TACL/Fig3b_en2zh_AL_dev.pdf}
% \end{subfigure}
% % \includegraphics[width=7cm]{figs/bleu/bleu_AL_dev_ref2.pdf}
% % \end{minipage}
% \captionof{figure}{BLEU scores for wait-$k$ with Transformer (and its catchup version) and wait-$k$ with RNN model on ZH2EN dev set with 1-ref BLEU.
% Latency is measured by AL.}
% \label{fig:bleuAL_dev1}
% \end{figure*}
% %``B\`ush\'i z\v{o}ngt\v{o}ng z\`ai M\`os\-{i}k\={e}''

% \begin{figure*}[!t]%[t]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=7cm]{figs/for_TACL/Fig3a_zh2en_AL_dev.pdf}
% \end{subfigure}%
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=7cm]{figs/for_TACL/Fig3b_en2zh_AL_dev.pdf}
% \end{subfigure}%
% \captionof{figure}{
% BLEU scores and AL comparisons with different wait-$k$ models on Chinese-to-English (left figure) and English-to-Chinese (right figure)
% translations on dev set. Note we use 4-ref BLEU for Chinese-to-English but 1-ref BLEU for English-to-Chinese since the multiple references are only available on English side.}
% \label{fig:bleuAL_dev1}
% \end{figure*}

% \begin{table*}
% \centering
% % \setlength{\tabcolsep}{2pt}
% \resizebox{15cm}{!}{%
% \begin{tabular}{|c | c |c |c |c |c |c |c |c |c |c |c|c|c|c|}
% \hline
% & & \em{k} & 1 &2 &3 &4 &5 &6 &7 &8 &9 &10 & $\infty^{\dagger}$ &$\infty^{\ddagger}$ \\
% \hline
% \multirow{4}{*}{Transformer}& \multirow{4}{*}{wait-\em{k}} & AP& 0.63 & 0.61 & 0.68 & 0.70 & 0.74 & 0.76 & 0.79 & 0.80 & 0.82 & 0.84 & 1 & 1\\
% \cline{3-15}
% && AL & 3.68 & 2.96 & 5.03 & 5.35 & 6.76 & 7.27 & 8.61 & 9.03 & 9.87 & 11.0 & 28.73 & 28.73\\
% \cline{3-15}
% && 1-ref BLEU & 13.31 & 13.46 & 15.28 & 15.33 & 16.93 & 16.74 & 16.84 & 17.14 & 17.18 & 18.00 & 19.03 & 20.29\\
% \cline{3-15}
% && 4-ref BLEU & 25.73 & 25.24 & 29.36 & 29.20 & 30.73 & 30.86 & 31.66 & 32.03 & 32.69 & 32.95 & 36.29 & 38.34\\
% \hline
% \multirow{4}{*}{RNN}& \multirow{4}{*}{wait-\em{k}} & AP& 0.63 & 0.61 & 0.68 & 0.70 & 0.74 & 0.76 & 0.79 & 0.80 & 0.82 & 0.84 & 1 & 1\\
% \cline{3-15}
% && AL & 3.68 & 2.96 & 5.03 & 5.35 & 6.76 & 7.27 & 8.61 & 9.03 & 9.87 & 11.0 & 28.73 & 28.73\\
% \cline{3-15}
% && 1-ref BLEU & 13.31 & 13.46 & 15.28 & 15.33 & 16.93 & 16.74 & 16.84 & 17.14 & 17.18 & 18.00 & 19.03 & 20.29\\
% \cline{3-15}
% && 4-ref BLEU & 25.73 & 25.24 & 29.36 & 29.20 & 30.73 & 30.86 & 31.66 & 32.03 & 32.69 & 32.95 & 36.29 & 38.34\\
% \hline
% \hline
% \multirow{4}{*}{Transformer}&\multirow{4}{*}{\chn{+catchup}} & AP& 0.50 & 0.55 & 0.60 & 0.62 & 0.68 & 0.72 & 0.73 & 0.76 & 0.79 & 0.81 & 1 &1\\
% \cline{3-15}
% && AL & 0.80 & 1.26 & 1.76 & 2.34 & 4.31 & 5.43 & 5.99 & 6.95 & 8.27 & 9.36 & 28.73 & 28.73\\
% \cline{3-15}
% && 1-ref BLEU & 10.12 & 11.90 & 12.95 & 13.40 & 14.47 & 15.69 & 15.88 & 16.73 & 16.63 & 17.09& 19.03 & 20.29\\
% \cline{3-15}
% && 4-ref BLEU & 18.55 & 22.03 & 24.09 & 25.23 & 27.37 & 29.49 & 29.72 & 30.97 & 31.25 & 32.24& 36.29& 38.34\\
% \hline
% \end{tabular} 
% }
% \caption{Our ``wait-{\em{k}}'' and ``catchup'' model's performance with different number of waited words (first row)and AP in
% one-reference and four-reference BLEU on test set.
% $\infty^{\dagger}$ means baseline with greedy search. $\infty^{\ddagger}$ represents the baseline with beam search when beam is 11.}
% \label{tb:waitktest}
% \end{table*}

\newcolumntype{M}{>{\em}c}


%% \begin{table*}
%% \centering
%% % \setlength{\tabcolsep}{2pt}
%% \resizebox{16cm}{!}{%

%% \begin{tabular}{ | c |c |c|M |c|M |c |M |c |M |c|M|c|M|}
%% %%%%%%%%%%%%%%%%%%%%% removed 12/31/2018 %%%%%%%%%%%%%%%%%%%%% 

%% % \hline
%% % \color{red}last zh2en test & \em{k} & 1 &2 &3 &4 &5 &6 &7 &8 &9 &10 & $\infty^{\dagger}$ &$\infty^{\ddagger}$ \\
%% % \hline
%% % \multirow{4}{*}{\shortstack{Transformer\\ wait-\em{k}}} & AP& 0.53 & 0.58 & 0.61 & 0.64  & 0.66 & 0.76 & 0.79 & 0.80 & 0.82 & 0.84 & 1 & 1\\
%% % \cline{2-14}
%% % & AL & 0.17 & 1.67 & 2.10 &3.02  &3.60 & 7.27 & 8.61 & 9.03 & 9.87 & 11.0 & 28.73 & 28.73\\
%% % \cline{2-14}
%% % & 1-ref BLEU & 11.56 & 12.56 & 13.38 &15.05 & 15.35 & 16.74 & 16.84 & 17.14 & 17.18 & 18.00 & 19.03 & 20.29\\
%% % \cline{2-14}
%% % & 4-ref BLEU & 22.28 &24.19 & 25.92 & 28.41 & 28.80 & 30.86 & 31.66 & 32.03 & 32.69 & 32.95 & 36.29 & 38.34\\
%% % \hline
%% % \hline
%% % \multirow{4}{*}{\shortstack{Transformer\\wait-\em{k}\\\chn{+catchup}}} & AP& 0.54 & 0.60 & 0.62 & 0.65 & 0.68 & 0.72 & 0.73 & 0.76 & 0.79 & 0.81 & 1 &1\\
%% % \cline{2-14}
%% % & AL & 0.60 &  2.37 &  2.68 &  3.40 &  4.16 & 5.43 & 5.99 & 6.95 & 8.27 & 9.36 & 28.73 & 28.73\\
%% % \cline{2-14}
%% % & 1-ref BLEU & 10.24 & 10.96 & 12.50 & 14.24 & 14.85 & 15.69 & 15.88 & 16.73 & 16.63 & 17.09& 19.03 & 20.29\\
%% % \cline{2-14}
%% % & 4-ref BLEU & 19.95 & 21.87 &24.52 & 26.31 & 27.53 & 29.49 & 29.72 & 30.97 & 31.25 & 32.24& 36.29& 38.34\\
%% \hline
%% \color{red}\detoen test & \em{k} & \multicolumn{2}{c|}{1} &\multicolumn{2}{c|}{3} &\multicolumn{2}{c|}{5} &\multicolumn{2}{c|}{7} &\multicolumn{2}{c|}{9}& \multicolumn{2}{c|}{$\infty$} \\
%% \hline
%% \multirow{3}{*}{\shortstack{Transformer\\ wait-\em{k}}} & AP& 0.59 & 0.58 & 0.65 & 0.64 & 0.70 & 0.70 & 0.75 & 0.75 & 0.79 & 0.79& \multicolumn{2}{c|}{1}\\
%% \cline{2-14}
%% & AL & 1.4 & 1.2 & 3.2 & 3.1 & 5.0 & 4.9 & 6.7 & 6.7 & 8.4 & 8.4 & \multicolumn{2}{c|}{28.6}\\
%% \cline{2-14}
%% & 1-ref BLEU & 19.38 & 19.36  & 24.07 & 24.05  & 26.38 & 26.31  & 27.63 & 27.68  & 28.39 & 28.52 & 29.92 & 30.69 \\
%% \hline
%% \multirow{3}{*}{\shortstack{RNN\\wait-\em{k}}} & AP & 0.56 & 0.55 & 0.63 & 0.62 & 0.69 & 0.68 & 0.74 & 0.73 & 0.78 & 0.77 &  \multicolumn{2}{c|}{1}\\
%% \cline{2-14}
%% & AL & 0.67 & 0.26 & 2.9 & 2.5 & 5.1 & 4.7 & 7.0 & 6.7 & 8.9 & 8.7 & \multicolumn{2}{c|}{28.6}\\
%% \cline{2-14}
%% & 1-ref BLEU & 12.59 & 12.47 & 17.32 & 17.31 & 20.39 & 20.32 & 21.55 & 21.61  & 22.69 & 22.87 & 23.19 & 24.42 \\
%% \hline
%% \hline
%% \color{red}\entode test & \em{k} & \multicolumn{2}{c|}{1} &\multicolumn{2}{c|}{3} &\multicolumn{2}{c|}{5} &\multicolumn{2}{c|}{7} &\multicolumn{2}{c|}{9}& \multicolumn{2}{c|}{$\infty$} \\
%% \hline
%% \multirow{3}{*}{\shortstack{Transformer\\ wait-\em{k} }} & AP&  0.57 & 0.57 & 0.64 & 0.63 & 0.70 & 0.70 & 0.76 & 0.76 & 0.80 & 0.80 & \multicolumn{2}{c|}{1}\\
%% \cline{2-14}
%% & AL & 1.6 & 1.5 & 3.3 & 3.2 & 5.2 & 5.2 & 7.0 & 7.0 & 8.8 & 8.8 & \multicolumn{2}{c|}{26.6} \\
%% \cline{2-14}
%% & 1-ref BLEU & 16.73 & 17.13 & 21.97 & 22.33 & 24.52 & 24.82 & 26.0 & 26.13 & 26.65 & 26.79 & 26.63 & 27.44 \\
%% \hline
%% \multirow{3}{*}{\shortstack{RNN\\wait-\em{k} }} & AP & 0.58 & 0.56 & 0.64 & 0.63 & 0.71 & 0.70 & 0.76 & 0.75 & 0.81 & 0.80 & \multicolumn{2}{c|}{1}\\
%% \cline{2-14}
%% & AL & 1.7 & 1.4 & 3.6 & 3.3 & 5.4 & 5.1 & 7.2 & 6.9 & 9.2 & 8.9 & \multicolumn{2}{c|}{26.6}\\
%% \cline{2-14}
%% & 1-ref BLEU &  11.94 & 12.57 & 16.1 & 16.79 & 17.88 & 18.72 & 18.49 & 19.44 & 18.45 & 19.58 & 19.76 & 20.82\\
%% \hline
%% %%%%%%%%%%%%%%%%%%%%% removed 12/31/2018 %%%%%%%%%%%%%%%%%%%%% 
%% % zh2en_test
%% % \begin{tabular}{ | c |c |c |c |c |c |c |c |c |c |c|c|c|c|}
%% \hline
%% \hline
%% \color{red}\zhtoen test & \em{k} & \multicolumn{2}{c|}{1} &\multicolumn{2}{c|}{3} &\multicolumn{2}{c|}{5} &\multicolumn{2}{c|}{7} &\multicolumn{2}{c|}{9}& \multicolumn{2}{c|}{$\infty$} \\
%% \hline
%% \multirow{3}{*}{\shortstack{Transformer\\ wait-\em{k}}} & AP& 0.60 & \em{0.59} & 0.67 & \em{0.67} & 0.73 & \em{0.73} & 0.77 & \em{0.78} & 0.82 & \em{0.82} &  \multicolumn{2}{c|}{1}\\
%% \cline{2-14}
%% & AL & 2.9 & 2.7 & 5.0 & 5.0 & 6.8 & 6.9 & 8.3 & 8.5 & 10.3 & 10.5 &  \multicolumn{2}{c|}{28.7} \\
%% \cline{2-14}
%% % & 1-ref BLEU & 14.41 & 14.41 & 15.88 & 16.0 & 16.98 & 17.3 & 16.9 & 17.41 & 17.95 & 18.29 & 19.03 & 20.29\\
%% % \cline{2-14}
%% & 4-ref BLEU & 25.79 & 26.02 & 28.94 & 29.45 & 31.14 & 31.62 & 31.74 & 32.55 & 33.46 & 34.39 & 36.29 & 38.34\\
%% \hline
%% \multirow{3}{*}{\shortstack{Transformer\\wait-\em{k}\\\color{blue} + \chn{decoder catchup}}} & AP&  0.53 & 0.52 & 0.61 & 0.6 & 0.67 & 0.66 & 0.73 & 0.72 & 0.79 & 0.78 &\multicolumn{2}{c|}{1}\\
%% \cline{2-14}
%% & AL & 0.54 & 0.29 & 2.6 & 2.3 & 4.1 & 3.8 & 6.3 & 5.9 & 8.7 & 8.2 &  \multicolumn{2}{c|}{28.7}\\
%% \cline{2-14}
%% % & 1-ref BLEU & 11.64 & 11.55 & 13.93 & 13.87 & 14.92 & 14.81 & 16.67 & 16.46 & 17.38 & 17.05 & 19.03 & 20.29\\
%% % \cline{2-14}
%% & 4-ref BLEU & 19.95 & 20.32 & 24.52 & 24.85 & 27.53 & 27.66 & 30.56 & 30.51 & 31.19 & 31.29 & 36.29 & 38.34\\
%% \hline
%% \hline
%% \color{red}\entozh test & \em{k} & \multicolumn{2}{c|}{1} &\multicolumn{2}{c|}{3} &\multicolumn{2}{c|}{5} &\multicolumn{2}{c|}{7} &\multicolumn{2}{c|}{9}& \multicolumn{2}{c|}{$\infty$} \\
%% \hline
%% \multirow{3}{*}{\shortstack{Transformer\\ wait-\em{k} \\ \color{blue}+ \chn{encoder catchup}}} & AP& 0.52 & 0.53 & 0.59 & 0.59 & 0.64 & 0.65 & 0.69 & 0.69 & 0.73 & 0.73 & \multicolumn{2}{c|}{1}\\
%% \cline{2-14}
%% & AL & 0.39 & 0.56 & 2.6 & 2.7 & 4.5 & 4.6 & 6.3 & 6.3 & 8.1 & 8.1 & \multicolumn{2}{c|}{38.3} \\
%% \cline{2-14}
%% & 1-ref BLEU & 9.37 & 9.41 & 12.62 & 12.61 & 14.4 & 14.56 & 15.67 & 16.39 & 16.22 & 16.99 & 18.65 & 19.56\\
%% \hline



%% %% \hline
%% %% \multirow{4}{*}{RNN wait-\em{k}} & AP& 0.58 & 0.62 & 0.65 & 0.68 & 0.7 & 0.73 & 0.76 & 0.78 & 0.80 & 0.81 & 1 &1\\
%% %% \cline{2-14}
%% %% & AL & 1.97 & 2.79 & 3.49 & 4.45 & 5.05 & 5.97 & 6.88 & 7.67 & 8.55 & 9.28 & 28.73 & 28.73\\
%% %% \cline{2-14}
%% %% & 1-ref BLEU & 11.14 & 12.18 & 13.06 & 13.27 & 13.96 & 14.35 & 14.28 & 14.42 & 14.98 & 14.42 & 15.08 & 16.40\\
%% %% \cline{2-14}
%% %% & 4-ref BLEU & 21.37 & 23.48 & 24.27 & 24.75 & 26.12 & 26.33 & 26.53 & 26.93 & 27.96 & 27.39 & 28.22& 31.85\\
%% %% \hline
%% \end{tabular} 
%% }
%% \caption{Performances of wait-$k$ with Transformer, its catchup version, and wait-$k$ with RNN models with various $k$ 
%% % (the number of waited words) %(first row) 
%% %and AP in
%% %1-ref and 4-ref BLEU scores 
%% on the \deen and \zhen test sets.
%% For each $k$, the numbers on left side are from greedy decoding,
%% and right, italic font numbers are from tail beam search.
%% $\infty$ represents baseline with results from greedy and beam search.}
%% \label{tb:waitktest}
%% \end{table*}


Figs.~\ref{fig:APCW_de2en}--\ref{fig:APCW_en2zh}
plot translation quality (in BLEU) against latency (in AL and CW) for full-sentence baselines, 
our wait-$k$, test-time wait-$k$ (using full-sentence models),
and our adaptation of \namecite{gu+:2017} from RNN to Transformer\footnote{
However, it is worth noting that, despite our best efforts, we  failed to reproduce their work on their original RNN, %(with BLEU gaps as big as 10 points),
regardless of using their code or our own.
That being said, our successful implementation of their work on Transformer
is also a notable contribution of this work.
By contrast, it is very easy to make wait-$k$ work on either RNN or Transformer.}
on the same Transformer baseline.
In all these figures, we observe that, as $k$ increases, 
(a) wait-$k$ improves in BLEU score and worsens in latency, and
(b) the gap between test-time wait-$k$ and wait-$k$ shrinks.
Eventually, both wait-$k$ and test-time wait-$k$ approaches the full-sentence baseline
as $k\goesto\infty$.
These results are consistent with our intuitions.


We next compare our results with our adaptation of \namecite{gu+:2017}'s two-staged full-sentence model + reinforcement learning on Transformer.
We can see that while on BLEU-vs-AL plots, their models perform similarly to our test-time wait-$k$ for \detoen and \zhtoen, and
slightly better than our test-time wait-$k$ for \entozh,
%\footnote{Due to time constraints, we could not finish replicating Gu et al.~for \entode,
%which will be done in the final version.}
  which is reasonable as both use a full-sentence model at the very core.
However, on BLEU-vs-CW plots, their models have much worse CWs, which is also consistent with results in their paper (Gu, p.c.).
This is because their R/W model prefers consecutive segments of READs and WRITEs (e.g., their model often produces R R R R R W W W W R R R W W W W R ...) while our wait-$k$ translates concurrently with the input
(the initial segment has length $k$, and all others have length 1, thus a much lower CW).
We also found their training to be extremely brittle due to the use of RL
whereas our work is very robust.
%% In Fig.~\ref{fig:bleuAP_en2de_test}, we compare the BLEU 
%% score and AP with the model from \cite{gu+:2017} on dev 
%% set for English-to-German and German-to-English tasks. 
%% The results indicate that our RNN-based model outperforms the 
%% model from \namecite{gu+:2017} in both translation directions 
%% and our simultaneous Transformer achieves much better performance.
%% In Fig.~\ref{fig:bleuAL_en2de_test}, we also compare the 
%% BLEU score together with AL between
%% RNN and Transformer-based models.
%% We also include AL values of one model of \namecite{gu+:2017} in each direction based
%% on the decoded action sequences the authors shared with us (Gu, p.c.).


%% The performance between Chinese and English % translation
%% are shown in Fig.~\ref{fig:bleuAL_dev1}.
%% The difference between wait-$k$ and wait-$k$ with decoder catchup are 
%% compared on the left figure for Chinese-to-English translation.
%% For the direction of English-to-Chinese, we only show 
%% wait-$k$ with encoder catchup since source side is much longer
%% than target side.

%% CW (consecutive wait) measures the average source segment length, 
%% and we also compare CW in Table~\ref{tb:comparecw}.
%% As analysed in Sec.~\ref{sec:al},
%% our wait-$k$ has AL close to 1.
%% With similar or better BLEU scores,
%% our CWs are much lower than those from \namecite{gu+:2017},
%% which indicates better user experience. % since our model reduces no output periods a lot.

%% More comprehensive comparisons on the test sets are shown
%% in Table~\ref{tb:waitktest}.
%% We show both greedy and tail beam search performances
%% in the table.

%src:他 还 说 现在 正在 为 这 一 访问 作 出 安排 。
%hyp:he also said that he is making preparations for this visit .
%ref:he also said that arrangements are currently being made for this trip .
%bleu:66.3615480569



%src:古巴 是 第一 个 与 新 中国 建交 的 拉美 国家 。
%hyp:cuba is the first country to establish diplomatic relations with new china .
%ref:cuba was the first latin american country to establish diplomatic relations with new china .
%bleu:72.9836014355


%\subsection{Comparison with \namecite{gu+:2017}}

\begin{figure*}

\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{.7pt}
\centering
\begin{tabu}{ c | c c c c c c c c c c c c c c c c c c c     l  }
\rowfont{\small}
  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12  & 13 & 14 & 15 & 16 & 17 & 18 & 19  \\
       & doch & w\"{a}hrend & man & \color{purple}sich & im & kongre- & ss &  nicht & auf & ein & \!\!\!vorgehen & \color{blue}einigen & \color{red}kann & , & warten & mehrere & bs. & nicht & l\"{a}nger \\
\rowfont{\small}
  & but & while & they\,  & -self & in  & \multicolumn{2}{c}{congress} & not & on & one & action & \color{blue}agree & \color{red}can & , & wait & several  & states & no & longer \\
  \hline
  $k$=3  &     &       &  & but & , & while & congress & \color{red}has & not & \,\color{blue}agreed & on & a & course & of & action & , & several & states & no & longer wait \\
 %\hline
% $k$=\small$\infty$ & \multicolumn{19}{c}{} & but \!,\! while \!...\\
\end{tabu}
}
\caption{German-to-English example in the dev set with anticipation.
  The main verb in the embedded clause, ``einigen'' (agree), is correctly predicted 3 words ahead of time (with ``sich'' providing a strong hint),
  while the aux.~verb ``kann'' (can) is predicted as ``has''.
  The baseline translation is ``but , while congressional action can not be agreed , several states are no longer waiting''.
  bs.: bunndesstaaten. % (states).
  %``kongress" is split due to BPE.
}
\label{fig:congress}
\smallskip

\resizebox{.9\textwidth}{!}{%
\setlength{\tabcolsep}{1pt}
\centering
\begin{tabu}{ c | c c c c c c c c c c c c l l  }
\rowfont{\small}
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12    \\[-0.1cm]
  \rowfont{\small}
& \chn{t\=a} &\chn{h\'ai} & \chn{shu\=o} & \chn{xi\`anz\`ai} & \chn{zh\`engz\`ai} & \chn{w\`ei} & \chn{zh\`e} & \chn{y\=\i} & \chn{f\v{a}ngw\`en} & \color{purple}\chn{zu\`o} & \chn{ch\=u} & \color{blue}\chn{\=anp\'ai} \\

  & 他 & 还&  说 &现在& 正在& 为 &这 &一 &访问 &\color{purple}作 &出  &\color{blue}安排\\ % 。古巴 &是 &第一 &个 &   与 &新 & 中国 &建交 &     的 &拉美 &  国家 \\ %& 将 & \color{blue}于 & \color{blue}\chn{2008} & \color{blue}年 & 在 & 北京 & 举行  \\

 \rowfont{\small}
 & he & also & said & now  & (\chn{prog.})$^\diamond$ & for & this & one & visit & \color{purple}make & out & \!\!\!\!\color{blue}arrangement\!\!\!\!\\  
 \hline
 $k$=1 & & he & also& said & that & he & is & now & \color{purple}making & \color{blue}preparations & for  & this  & visit \\
 $k$=3 &  & & & he &  also & said & that & he & is & \color{purple}making & \color{blue}preparations & for  & this  visit\\
 \iffalse
 $k$=3$^\dagger$ &  & & & he &  also & said & \ \underline{that  he} & is & now & \color{blue}working  & \underline{for   this} & visit\\[0.05cm]
 \fi
  %\hline
 %\chn{+catchup} &  & & & the & olympic & games  & \chn{will be} & held &in  beijing  \color{blue}in  \color{blue}2008     \\
 \hline
% Baseline$^\dagger$ & \multicolumn{12}{l}{} & he added that arrangements   \\%cuba is the first latin american country to \\
 %                                  &  \multicolumn{12}{l}{} &are being made for this visit  \\[0.1cm] %establish diplomatic relations with new china\\ % the olympic games will be held in beijing {\color{blue}in 2008}\\
$k$=$\infty$ & \multicolumn{12}{l}{} & he also said that arrangements  \\%the olympic games will be held in beijing {\color{blue}in 2008}
& \multicolumn{12}{l}{} & are being made for this visit 
\end{tabu} 
}
\caption{Chinese-to-English example in the dev set with anticipation.
  Both wait-1 and wait-3 policies yield perfect translations,
  with ``making preparations'' predicted well ahead of time.
  $^\diamond$: progressive aspect marker.
  \iffalse
  $^\dagger$: +catchup,
  which produces slightly worse output, and finishes ahead of the source sentence.
  \fi
}

\iffalse %%%%%%%%%%%%%%%%%%
\bigskip

\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{.3pt}
\centering
\begin{tabu}{ c | c c c c c c c c c c c c c c c c c c c c c c c    l  }
\rowfont{\small}
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12   & 13 & 14 & 15 & 16 & \!\!\!\!17 & 18 & 19 & 20 & 21 & 22 & 23 \\[-0.1cm]
  \rowfont{\small}
 & \chn{B\`ush\'\i} & \chn{h\'ai} & \!\chn{bi\=aosh\`\i}\!\! & , & \color{brown}\chn{y\`{\i}ng} & \chn{\bajisitan} & \!\!\!\chn{h\'e} & \!\!\!\chn{\yindu} & \chn{zh\`engf\v{u}} & \chn{de} & \!\!\color{blue}\chn{y\=aoq\v{\i}ng}\!\! & , & \chn{t\=a} & \chn{ji\=ang} & \chn{y\'u} & \chn{3 yu\`e} & \!\!\!\chn{f\`en} & \chn{du\`\i} & \chn{\bajisitan} & \chn{h\'e} & \!\!\chn{\yindu} & \!\color{purple}\chn{j\`{\i}nx\'{\i}ng} & \,\color{red}\chn{f\v{a}ngw\`en}\!\!\!\!\\

  \rowfont{\small}
 & 布什 & 还 & 表示 & , & \color{brown}应& \!\!\! 巴基斯坦 \!\!\! &和 & 印度 & 政府 &的 & \color{blue}邀请 & , & 他 & 将 & 于 & 3月 & \!\!\!\!份& 对 & \!\!巴基斯坦\!\! & 和 & 印度 & \color{purple}进行 & \color{red}访问\\

\rowfont{\small}
 & Bush & also & said & , & \color{brown}at & Pakistan & \& & India & govt & 's & \color{blue}invite &, & he & will & in & \multicolumn{2}{c}{March} & to & Pakistan & \& & India & \color{purple}do & \color{red}visit\\
  \hline  
$k$=1 & & \!\! bush \ & also & said & that & at & the & \!\! \color{blue}invit.\!\! & of & \!\!\! the\ \ & pak. & \!\! \&\, & ind. & govts & , & he & \!\! will\, & \color{red}visit & \color{purple}pak. & \color{purple}\& & \color{purple}ind. & in & mar.\\ 
  $k$=3 & & & & \!\! bush \ & also & said & that & at & the & \!\! \color{blue}invit.\!\! & of & \!\!\! the\ \ & pak. & \& & ind. & govts & , & he & will & \color{purple}pay & a & \color{red}state & \color{red}visit & to  pak.~\& ind.~in  mar.\\
  \iffalse
  $k$=3$^\dagger$ & & & & \!\! bush \ & also & said & \!\!\!\underline{that  at} & the & \!\! \color{blue}invit.\!\! & of & \!\!\! \underline{the pak.} & \& & ind. & govts & \underline{, he} & will & \color{purple}pay & a & \underline{\color{red}state \color{red}visit} & to  & pak. & \& & \underline{ind.~in} &  mar.\\ [0.1cm]
  \fi
% \hline
%$k$=\small$\infty$ & \multicolumn{23}{l}{} & bush also said that  ...
\end{tabu} 
}
\caption{Another Chinese-to-English example in the dev set. Again, both wait-1 and wait-3 correctly predicted
  ``invitation'' because the Chinese construction ``{\em y\`ing} NP {\em de y\=aoq\v{\i}ng}'' means ``at the invitation of NP''.
  Futhermore, both predict ``visit'' (6 words ahead of time in wait-1),
  and wait-1 even predicts ``pakistan and india''.
  The baseline full-sentence translation is identical to that of our wait-1 policy.
  Abbreviations: invit.: invitation; pak.: pakistani/pakistan; ind.: indian/india; govts: governments; mar.: march.; \&: and.
  \iffalse
  $^\dagger$: +catchup, which produces the identical
  translation but predicts more ahead of time.
  \fi
}

\fi

 \smallskip

%\resizebox{16cm}{!}{%
%\setlength{\tabcolsep}{2pt}
%\centering
%\begin{tabular}{ c | c c c c c c c c c c c l l  }
% & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11    \\
% Chinese & 古巴 &是 &第一 &个 &   与 &新 & 中国 &建交 &     的 &拉美 &  国家 \\ %& 将 & \color{blue}于 & \color{blue}\chn{2008} & \color{blue}年 & 在 & 北京 & 举行  \\
% Pinyin & \chn{G\v{u}b\={a}} &\chn{sh\`{i}} & \chn{d\`iy\=\i} & \chn{g\`e} & \chn{y\v{u}} & \chn{x\={\i}n} & \chn{Zh\=onggu\'o} & \chn{ji\`anji\=ao} & \chn{de} & \chn{L\=am\v{e}i} & \chn{gu\'oji\=a}\\ 
% Gloss & Cuba & is & first & -  & with & new & China & est.~dipl.~ties & - & Lat.~Am. & country\\  
% \hline
% Wait-3 &  & & & cuba &  is & the & first & country & to & establish & diplomatic & relations  with  new  china\\
%  %\hline
% %\chn{+catchup} &  & & & the & olympic & games  & \chn{will be} & held &in  beijing  \color{blue}in  \color{blue}2008     \\
% \hline
% Baseline$^\dagger$ & \multicolumn{11}{l}{} &  cuba is the first latin american country to \\
%                                  &  \multicolumn{11}{l}{} & establish diplomatic relations with new china\\ % the olympic games will be held in beijing {\color{blue}in 2008}\\
%Baseline$^\ddagger$ & \multicolumn{11}{l}{} &  \\%the olympic games will be held in beijing {\color{blue}in 2008}
%\end{tabular} 
%}
%\caption{TBD}
%\caption{Our ``wait-3'' model  Baseline$^\dagger$ represents greedy decoding and Baseline$^\ddagger$ represents decoding with beam size 11.}
%\label{tb:olympic}
%\smallskip

%\begin{figure*}
\resizebox{0.9\textwidth}{!}{%
\setlength{\tabcolsep}{1pt}
\centering
\begin{tabu}{ c | c c c c c c c c c c c l }
\rowfont{\small}
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 &   \\[-0.1cm]
  \rowfont{\small}
 &\chn{jiāng} & \chn{zémín} & \color{purple}\chn{duì} & \color{purple}\chn{bùshí} & \color{purple}\chn{zǒngtǒng} & \color{colorC1}\chn{lái} & \color{colorC1}\chn{huá} & \color{cyan}\chn{fǎngwèn} & \color{blue}\chn{biǎoshì} & \color{brown}\chn{rèliè} & \color{brown}\chn{huānyíng}\\
 & 江 & 泽民 & \color{purple}对 & \color{purple}布什 & \color{purple}总统 & \color{colorC1}来 & \color{colorC1}华 & \color{cyan}访问 & \color{blue}表示 & \color{brown}热烈 & \color{brown}欢迎\\ [-0.1cm]
 \rowfont{\small}
 & jiang & zeming & \color{purple}to & \color{purple}bush & \color{purple}president & \color{colorC1}come-to & \color{colorC1}china & \color{cyan}visit & \color{blue}express & \color{brown}warm & \color{brown}welcome \\ 
 \hline
 %\rowfont{\small}
 $k$=3 &&&&jiang & zemin & \color{blue}expressed & \color{brown}welcome & \color{purple}to & \color{purple}president & \color{purple}bush & \color{purple}'s & \color{cyan}visit \color{colorC1}to china \\
\hline
 $k$=3$^\dagger$ &&&& jiang & zemin & \color{red}meets & \color{purple}president & \color{purple}bush & \color{colorC1}in & \color{colorC1}china & 's & bid to \color{cyan}visit \color{colorC1}china \\
% \hline
%$k$=$\infty$ & \multicolumn{12}{l}{} & he also said that arrangements  \\%the olympic games will be held in beijing {\color{blue}in 2008}
%& \multicolumn{12}{l}{} & are being made for this visit 
\end{tabu} 
}
\caption{Chinese-to-English example from online news. 
Our wait-3 model correctly
anticipates both ``{\color{blue}expressed}" and ``{\color{brown}welcome}'' (though missing ``{\color{brown}warm}''),
and moves the PP (``{\color{purple}to} ... {\color{cyan}visit} {\color{colorC1}to china}") to the very end which is fluent in the English word order.
$^\dagger$: test-time wait-$k$
produces nonsense translation.
}
  \smallskip
  
\resizebox{0.9\textwidth}{!}{
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabu}{c | c c c c c c c c c c l l }
\rowfont{\small}
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\[-0.1cm]
 \rowfont{\small}
 & \meiguo & \dangju & \dui & \shate & \jiezhe & \shizong & \yi & \an &\color{cyan}\gandao &  \color{blue}\danyou \\
(a) & 美国 &  当局 &对 &沙特 &记者 &失踪& 一& 案
 & \color{cyan}感到 &\color{blue}担忧\\
\rowfont{\small}
 \footnotesize & US & authorities & to & Saudi & reporter & \color{purple}missing & a & case & \color{cyan}feel & \color{blue}concern\\
 \hline
 $k$=3 & & & & the & us & authorities & \color{cyan}are & \color{blue}very  & \color{blue}concerned & about & the  saudi  reporter  's  missing  case\\
 \iffalse
 $k$=3$^\dagger$ & & & & the & us & authorities & \underline{\color{cyan}are \color{blue}very}  & \color{blue}concerned & about & the &  saudi  reporter  's  missing  case\\[0.1cm]
 \fi
%\hline
%$k$=\small$\infty$ & \multicolumn{10}{c}{} & us authorities concerned over \\
%& \multicolumn{10}{c}{} &  saudi journalists missing\\
\hline
 $k$=3$^\dagger$ & & & & the & us & authorities & \color{red}have & \color{red}dis-  & \color{red}appeared & from & saudi reporters \\
\hline
\rowfont{\small}
     &         &           &               &         &       &    &     &        &     & \color
     {red}\buman\\
(b) & 美国 &  当局 &对 &沙特 &记者 &失踪& 一& 案 & \color{cyan}感到 &\color{red}\bf 不满\\
 \hline
 $k$=3 & & & & the & us & authorities & \color{cyan}are & \color{blue}very  & \color{blue}concerned & about & the  saudi  reporter  's  missing  case\\
 $k$=5 & & & & & & the & us & \!\!\! authorities \!\!\!\!\! & \color{cyan}have & \color{cyan}expressed & {\color{red}\bf dissatisfaction}  with the incident \\
 & \multicolumn{10}{c}{} &   of saudi arabia 's missing reporters\\
%\hline
%$k$=\small$\infty$ & \multicolumn{10}{c}{} & us authorities dis- satisfied with \\
%& \multicolumn{10}{c}{} &   saudi reporters ' missing case\\
\hline
\iffalse
$k$=5$^\dagger$ & & & & & &us & \!\!\!\!\!\! authorities \!\!\!\!\!\! & ' & case & of & saudi  reporters being \\
&\multicolumn{10}{c}{} & dis- satisfied with missing 
\fi
\end{tabu}
}
\caption{(a) Chinese-to-English example from more recent news, clearly outside of 
  our data. Both the verb ``\gandao'' (``feel'') and the predicative ``\danyou'' (``concerned'') are correctly anticipated, probably hinted by ``missing''.
  \iffalse
  $^\dagger$: +catchup.
  \fi
(b) If we change the latter to \buman (``dissatisfied''),
the wait-3 result remains the same (which is wrong) while wait-5
%is just conservative enough to translate
translates conservatively without anticipation.
$^\dagger$: test-time wait-$k$ 
%which does not anticipate, and 
produces nonsense translation.
}
\label{fig:reporter}
\end{figure*}


\begin{figure*}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1pt}
\centering
\begin{tabu}{ c | c c c c c c c c c c c c c c c c c c c c c c c l }
\rowfont{\small}
%  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18  \\[-0.1cm]
  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 &14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23  \\[-0.1cm]
 & it & was & learned & that & this & is & \color{purple}the & \color{purple}largest & \color{colorC1}fire & \color{colorC1}accident & \color{cyan}in & \color{cyan}the & \color{cyan}medical & \color{cyan}and& \color{cyan}health & \color{cyan}system& \color{brown}nationwide & \color{blue}since & \color{blue}the & \color{blue}founding & \color{blue}of \color{blue}& \color{blue}new & \color{blue}china \\
 \hline
 %\multirow{1}{*}{$k$=5} 
 \begin{tabu}{c}
 \rowfont{\small}\\ \rowfont{\small}\\[-0.1cm]$k$=3 \\[-0.1cm] \rowfont{\small}\\ 
 \hline
 \rowfont{\small}\\ $k$=3$^\dagger$ \\[-0.1cm]  \rowfont{\small}\\
 \end{tabu}
 & 
 \begin{tabu}{c}
 \rowfont{\small}~1~\\ \rowfont{\small}\\ [-0.1cm]\\[-0.1cm]\rowfont{\small}\\\hline
 \end{tabu}
 & 
 \begin{tabu}{c}
 \rowfont{\small}~~~2~~~\\ \rowfont{\small}\\ [-0.1cm]\\[-0.1cm]\rowfont{\small}\\\hline
 \end{tabu}
 & 
 \begin{tabu}{c}
 \rowfont{\small}~~~~~~3~~~~~~~\\ \rowfont{\small}\\ [-0.1cm]\\[-0.1cm]\rowfont{\small}\\\hline
 \end{tabu}
 &
 %\multirow{1}{*}{
 \multicolumn{21}{l}{
 \begin{tabu}{c c c c c c c c c c c c c c c c c l}
 \rowfont{\small}
 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20\\[-0.1cm]
 \rowfont{\small}
  \chn{jù} & \chn{liǎojiě} & \chn{,} & \chn{zhè} & \chn{shì} & \color{PaleGreen}\chn{zhōngguó} & \color{red}\chn{jìn} & \color{red}\chn{jǐ} & \color{red}\chn{nián} & \color{red}\chn{lái} & \chn{fāshēng} & \chn{de} & \color{purple}\chn{zuì} & \color{purple}\chn{dà} & \color{purple}\chn{yī} & \color{purple}\chn{qǐ} &\color{cyan}\chn{yīliáo} & \chn{\color{cyan}wèishēng xìtǒng \color{colorC1}~huǒzāi shìgù} \\
  据 & 了解 & , & 这 & 是 & \color{PaleGreen}中国 & \color{red}近 & \color{red}几 & \color{red}年 & \color{red}来 & 发生 & 的 & \color{purple}最 & \color{purple}大 & \color{purple}一 & \color{purple}起 & \color{cyan}医疗 &\color{cyan}~~卫生 ~~系统 \color{colorC1}~火灾  事故 \\[-0.1cm]
\rowfont{\small}
  to & known & ,& this & is & \color{PaleGreen}China & \color{red}recent & \color{red}few & \color{red}years & \color{red}since & happen & - & \color{purple}most & \color{purple}big & \color{purple}one & \color{purple}case & \color{cyan}medical & \color{cyan}~~~health  ~~system \color{colorC1}~~fire accident \\
  \hline
 \rowfont{\small}
  \chn{yīnwèi} & \chn{tā} & \chn{shì} & \chn{,} & \chn{zhègè} & \chn{,} & \chn{shì} & \color{purple}\chn{zùi} & \color{purple}\chn{dà} & \chn{de} & \color{colorC1}\chn{huǒzāi} & \color{colorC1}\chn{shìgù} & \chn{,} & \color{blue}\chn{zhè} & \color{blue}\chn{shì} & \color{blue}\chn{xīn} & \color{blue}\chn{zhōngguó} & \color{blue}\chn{chénglì} \chn{yǐlái} \\
  因为 & 它 & 是 & , & 这个 & , & 是 & \color{purple}最 & \color{purple}大 & 的 & \color{colorC1}火灾 & \color{colorC1}事故 & , & \color{blue}这 & \color{blue}是 & \color{blue}新 &\color{blue}中国 &\color{blue}~成立 以来 \\[-0.1cm]
  \rowfont{\small}
  because & it & is & , & this & , & is & \color{purple}most & \color{purple}big & - & \color{colorC1}fire & \color{colorC1}accident &,& \color{blue}this & \color{blue}is & \color{blue}new & \color{blue}China &\color{blue}funding since\\
 
 \end{tabu}
 }\\
 \hline
% \hline\hline
% \rowfont{\small}
%   & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18  \\[-0.1cm]

% \rowfont{\small}
%  \multirow{3}{*}{$k$=3} & &&&\chn{jù} & \chn{liǎojiě} & \chn{,} & \chn{zhè} & \chn{shì} & \chn{zhōngguó} & \color{red}\chn{jìn} & \color{red}\chn{jǐ} & \color{red}\chn{nián} & \color{red}\chn{lái} & \chn{fāshēng} & \chn{de} & \chn{zuì} & \chn{dà} & \chn{yī} & ~\chn{qǐ}~ $\cdots$ ~\chn{huǒzāi}  \chn{shìgù} \\
%   &&&& 据 & 了解 & , & 这 & 是 & 中国 & \color{red}近 & \color{red}几 & \color{red}年 & \color{red}来 & 发生 & 的 & 最 & 大 & 一 & 起 $\cdots$ 火灾  事故 \\[-0.1cm]
%  \rowfont{\small}
%   &&&& to & known & ,& this & is & China & \color{red}recent & \color{red}few & \color{red}years & \color{red}since & happen & - & most & big & one & case $\cdots$ fire accident \\
% %%%%$k$=$\infty$ & 据 & 了解 & , & 这 & 是 & 新 & 中国 & 成立 & 以来 & , & 全国 & $\cdots$ & 发生 & 的 & 最 & 大 & 的 & 火灾 & 事故 \\
% %%%% $k$=5 & &&&&&据悉 & , & 这 & 是 & 今年 & 以来 & 中国 & 发生 & 的 & 最 & 大 & 一 & 起 & $\cdots$ 火灾 事故	\\
%  \hline
%  \rowfont{\small}
%   \multirow{3}{*}{$k$=3$^\dagger$} &&&& \chn{yīnwèi} & \chn{tā} & \chn{shì} & \chn{,} & \chn{zhègè} & \chn{,} & \chn{shì} & \chn{zùi} & \chn{dà} & \chn{de} & \chn{huǒzāi} & \chn{shìgù} & \chn{,} & \color{blue}\chn{zhè} & \color{blue}\chn{shì} & \color{blue}\chn{xīn} \chn{zhōngguó} \chn{chénglì} \chn{yǐlái} \\
%   &&&& 因为 & 它 & 是 & , & 这个 & , & 是 & 最 & 大 & 的 & 火灾 & 事故 & , & \color{blue}这 & \color{blue}是 & \color{blue}~新 ~中国 ~~成立 以来 \\[-0.1cm]
%   \rowfont{\small}
%   &&&& because & it & is & , & this & , & is & most & big & - & fire & accident &,& \color{blue}this & \color{blue}is & \color{blue}new ~China ~~funding since\\
%  \hline
% %%%%$k$=$\infty$ & 据 & 了解 & , & 这 & 是 & 新 & 中国 & 成立 & 以来 & , & 全国 & $\cdots$ & 发生 & 的 & 最 & 大 & 的 & 火灾 & 事故 \\
% %%%%\hline
\end{tabu} 
}
\caption{English-to-Chinese example in the dev set with incorrect anticipation due to mandatory long-distance reorderings. The English sentence-final  clause {\color{blue}``since the founding of new china''} is incorrectly predicted in Chinese as {\color{red}``近 几 年 来''(``in recent years'')}. %Even wait-5 and wait-7 cannot predict it; in fact, 
%Only a wait-till-end policy works here, because the Chinese word order dictates that the translation of this sentence-final English clause be placed %before ``发生''(``happen")
%very early in Chinese. 
Test-time wait-3 produces  translation in the English word order, which
sounds odd in Chinese,
and misses two other quantifiers ({\color{cyan}``in the medical and health system''} and {\color{brown}``nationwide''}), though without prediction errors.
%which is expected, since it uses the full-sentence translation model.
The full-sentence translation, 
``据 了解，这 是 {\color{blue}{新 中国 成立 以来}} ，{\color{brown}全国} {\color{cyan}医疗 卫生 系统} 发生 的 {\color{purple}最 大 的 一 起} {\color{colorC1}火 灾 事故}'', is perfect.}
\label{fig:fire}
\end{figure*}

\vspace{-0.2cm}

\subsection{Human Evaluation on Anticipation}
\vspace{-0.1cm}

\begin{table}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ | l |r |r |r |r |r |r |}
\hline
\multirow{2}{*}{} & $k$=3 & $k$=5 & $k$=7 & $k$=3 & $k$=5 & $k$=7 \\
\cline{2-7}
& \multicolumn{3}{c|}{\color{red} \zhtoen} & \multicolumn{3}{c|}{\color{red} \entozh} \\
\hline
sent-level \% & 33 & 21 & 9 & 52 & 27 & 17 \\
\hline
word-level \% & 2.5 & 1.5 & 0.6 & 5.8 & 3.4 & 1.4 \\
%\hline
\hfill accuracy & 55.4 & 56.3 & 66.7 &  18.6 & 20.9 & 22.2 \\
\hline
 & \multicolumn{3}{c|}{\color{red} \detoen} & \multicolumn{3}{c|}{\color{red} \entode} \\
\hline
sent-level \% & 44 & 27 & 8 & 28 & 2 & 0 \\
\hline
word-level \% & 4.5 & 1.5 & 0.6 & 1.4 & 0.1 & 0.0 \\
%\hline
\hfill accuracy & 26.0 & 56.0 & 60.0 & 10.7 & 50.0 & n/a \\
\hline
\end{tabular} 
}
\caption{Human evaluation for all four directions (100 examples each from dev sets). We report sentence- and word-level anticipation rates, and
   the word-level anticipation accuracy (among anticipated words).}
\label{tb:human}
\vspace{-.3cm}
\end{table}


Tab.~\ref{tb:human} shows human evaluations on anticipation rates and  accuracy on all four directions, using 100 examples in each language pair from the dev sets.
As expected, we can see that, with increasing $k$,
the anticipation rates decrease (at both sentence and word levels),
and the anticipation accuracy improves.
Moreover, the anticipation rates are very different among the four directions,
with
\[
\text{\entozh \;  $>$ \; \detoen \; $>$ \; \zhtoen \;  $>$ \; \entode}
\]
Interestingly, this order is exactly the same
with the order of the BLEU-score gaps between our wait-9 and full-sentence models:
\[
\small
\text{\entozh: 2.7 $>$  \detoen: 1.1 $>$ \zhtoen: 1.6$^\dagger >$  \entode: 0.3}
\]
($^\dagger$: difference in 4-ref BLEUs, which in our experience reduces by about half in 1-ref BLEUs).
We argue that this order roughly characterizes the relative
difficulty of {\em simultaneous} translation in these directions.
In our data, we found \entozh to be particularly difficult due to the mandatory long-distance reorderings
of English sentence-final temporal clauses (such as ``in recent years'') to much earlier positions in Chinese;
see Fig.~\ref{fig:fire} for an example.
It is also well-known that \detoen is  more challenging in simultaneous translation than \entode since SOV$\rightarrow$SVO involves prediction of the verb,
while SVO$\rightarrow$SOV generally does not need prediction in our wait-$k$ with a reasonable $k$,
because V is often shorter than O.
For example, human evaluation found only 1.4\%, 0.1\%, and 0\% word anticipations in \entode for $k$=3, 5 and 7, %respectively,
and 4.5\%, 1.5\%, and 0.6\% for \detoen.




\vspace{-0.2cm}

\subsection{Examples and Discussion}
\vspace{-0.1cm}



We showcase some examples in \detoen and \zhtoen
from the dev sets and online news in Figs.~\ref{fig:congress} to~\ref{fig:reporter}.
%which are generated from our proposed model and 
%baseline framework for demonstrating the effectiveness of our system from 
%% For all these figures,
%% we show the encoding step number and source language (and pinyin when 
%% translate from Chinese) with its gloss in the upper side. 
%% We show different generation results with different wait-$k$ models and baselines
%% in the lower part of these tables.
%% Note that baseline method which starts generating words after the entire source 
%% sentence are encoded in the last row while our model only wait $k$ encoding steps.
In all these examples except Fig.~\ref{fig:reporter}(b),
our wait-$k$ models can generally anticipate correctly,
often producing translations as good as the full-sentence baseline.
In Fig.~\ref{fig:reporter}(b), when we change the last word,
the wait-3 translation remains unchanged (correct for (a) but wrong for (b)),
but wait-5 is more conservative and produces the correct translation without anticipation.





%%%%%%%%%%%%%%%%%%%%%

%% \begin{table*}

%% %% \resizebox{\textwidth}{!}{
%% %% \centering
%% %% \setlength{\tabcolsep}{2pt}
%% %% \begin{tabu}{c | c c c c c c c c c c l l }
%% %%  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
%% %%   \rowfont{\small}
%% %% & \meiguo & \zongtong & \bushi &\zai &\mosike & \yu & \eluosi &\zongtong &\pujing &  \huitan \\
%% %%  & 美国 & 总统 & 布什 & 在 & 莫斯科 & 与 & 俄罗斯  & 总统 & 普京 & 会谈\\
%% %%  \rowfont{\small}
%% %% & US & pres. & Bush & in & Moscow & with & Russian & pres. & Putin & \color{blue}talk\\
%% %%  \hline
%% %% $k$=3 & & & & us & pres. & bush & \color{blue}met  & with & russian & pres. & putin  in  moscow\\
%% %% $k$=3$^\dagger$ & & & & us & pres. & bush & \underline{\color{blue}met   with} & russian & pres. & putin  & in  moscow\\
%% %% \hline
%% %% $k$=\small$\infty$ & \multicolumn{10}{c}{} & us president bush {\color{blue}holds talks} with\\
%% %% & \multicolumn{10}{c}{} &  russian president putin in moscow\\
%% %% \end{tabu}
%% %% }
%% %% \caption{A Chinese-to-English example in the news domain outside of 
%% %% our data, similar to our running example.$^\dagger$: +catchup.}

%% %% \smallskip

%% \resizebox{\textwidth}{!}{
%% \centering
%% \setlength{\tabcolsep}{2pt}
%% \begin{tabu}{c | c c c c c c c c c c l l }
%%  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
%%  \rowfont{\small}
%%  & \meiguo & \dangju & \dui & \shate & \jiezhe & \shizong & \yi & \an &\color{cyan}\gandao &  \color{blue}\danyou \\
%% (a) & 美国 &  当局 &对 &沙特 &记者 &失踪& 一& 案
%%  & \color{cyan}感到 &\color{blue}担忧\\
%% \rowfont{\small}
%%  \footnotesize & US & authorities & to & Saudi & reporter & \color{purple}missing & a & case & \color{cyan}feel & \color{blue}concern\\
%%  \hline
%% $k$=3 & & & & the & us & authorities & \color{cyan}are & \color{blue}very  & \color{blue}concerned & about & the  saudi  reporter  's  missing  case\\
%% $k$=3$^\dagger$ & & & & the & us & authorities & \underline{\color{cyan}are \color{blue}very}  & \color{blue}concerned & about & the &  saudi  reporter  's  missing  case\\[0.1cm]
%% \hline
%% $k$=\small$\infty$ & \multicolumn{10}{c}{} & us authorities concerned over \\
%% & \multicolumn{10}{c}{} &  saudi journalists missing\\
%% \hline
%% \hline
%% \rowfont{\small}
%%      &         &           &               &         &       &    &     &        &     & \color
%%      {red}\buman\\
%% (b) & 美国 &  当局 &对 &沙特 &记者 &失踪& 一& 案 & \color{cyan}感到 &\color{red}\bf 不满\\
%%  \hline
%%  $k$=3 & & & & the & us & authorities & \color{cyan}are & \color{blue}very  & \color{blue}concerned & about & the  saudi  reporter  's  missing  case\\
%%  $k$=5 & & & & & & the & us & authorities & \color{cyan}have & \color{cyan}expressed & {\color{red}\bf dissatisfaction}  with the incident of\\
%%  & \multicolumn{10}{c}{} &   saudi arabia 's missing reporters\\
%% \hline
%% $k$=\small$\infty$ & \multicolumn{10}{c}{} & us authorities dis- satisfied with \\
%% & \multicolumn{10}{c}{} &   saudi reporters ' missing case\\
%% \end{tabu}
%% }
%% \caption{(a) A sentence from more recent news, clearly outside of 
%% our data. Both the verb ``\gandao'' (``feel'') and the predicative ``\danyou'' (``concerned'') are anticipated.
%% $^\dagger$: +catchup.
%% (b) If we change the predicative to \buman (``dissatisfied''),
%% the wait-3 result remains the same, which is wrong, while wait-5
%% is just conservative enough to translate 
%% without anticipation.
%% }


%% \end{table*}

%%  \begin{table*}
%%  \resizebox{16cm}{!}{%
%%  \setlength{\tabcolsep}{2pt}
%%  \centering
%%  \begin{tabular}{ c | c c c c c c c c l  }
%%   & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 &    \\
%%   Chinese & 奥运会 & 将 & \color{blue}于 & \color{blue}\chn{2008} & \color{blue}年 & 在 & 北京 & 举行  \\
%%   Pinyin & \chn{\`Aoy\`unhu\`{i}} & \chn{ ji\={a}ng} & \color{blue}\chn{y\'u} & \color{blue}\chn{2008} & \color{blue}\chn{ni\'an} & \chn{z\`ai} & \chn{B\v{e}ij\={\i}ng} & \chn{j\v{u}x\'ing} & \\ 
%%   Gloss & Olympics & will & \color{blue}in & \color{blue}2008 & \color{blue}year & in & Beijing & hold \\  
%%   \hline
%%   Wait-3 &  & & & the & olympic & games  &will& be & held in  beijing  \color{blue}in  \color{blue}2008     \\
%%    %\hline
%%  % \chn{+catchup} &  & & & the & olympic & games  & \chn{will be} & held &in  beijing  \color{blue}in  \color{blue}2008     \\
%%  % \hline
%%  % Baseline$^\dagger$ & \multicolumn{8}{l}{} &  the olympic games will be held in beijing {\color{blue}in 2008}\\
%% %  Baseline$^\ddagger$ & \multicolumn{8}{l}{} &  the olympic games will be held in beijing {\color{blue}in 2008}
%%  \end{tabular} 
%%  }
%%  \caption{Our ``wait-3'' model moves the adverbial (``in 2008 year'') to the end, producing  translation fluent in the English word order which is identical 
%%  to the full-sentence baseline.}
%%  \label{tb:olympic}
%%  \smallskip
%%  \end{table*}

%%  \begin{table*}
%%  \resizebox{16cm}{!}{%
%%  \setlength{\tabcolsep}{1.2pt}
%%  \centering
%%  \begin{tabular}{ c | c c c c c c c c c c c l }
%%   & 1&2&3&4&5&6&7&8&9&10&11&  \\
%%   Chinese & \color{chocolate}中东 & \color{chocolate}地区 & \color{blue}因为 & \color{blue}局势& \color{blue}动荡 & 所以 & 爆发 & 了 
%%   & 一 &系列& 冲突 & \\
%%   Pinyin & \color{chocolate}\chn{zh\={o}ngd\={o}ng} & \color{chocolate}\chn{d\`iq\={u}} & \color{blue}\chn{y\={\i}nw\'ei} & \color{blue}\chn{j\'ush\`i} & \color{blue}\chn{d\`ongd\`ang} & \chn{s\v{u}oy\v{\i}} & \chn{b\`aof\={a}} & \chn{le} 
%%   & \chn{y\'i} &\chn{x\`ili\`e}& \chn{ch\={o}ngt\={u}} & \\ 
%%   Gloss & \color{chocolate}mideast & \color{chocolate}area & \color{blue}because & \color{blue}situation & \color{blue}turbulent & so & break & - & a & series & conflicts\\  
%%   \hline
%%   Wait-3 &  & & & \color{blue}because & \color{blue}of & \color{blue}the  &
%%   \color{blue}tur- & \color{blue}bul- & \color{blue}ence
%%   &\color{chocolate}in & \color{chocolate} the  & {\color{chocolate}middle east ,} a series of conflicts have occurred  \\
%%    %\hline
%% %  \chn{+catchup} &  & & & \color{blue}because & \color{blue}of & \color{blue}the  &
%% %  \chn{\color{blue}tur-  \color{blue}bul-} & \color{blue}ence & \color{blue}situation
%% %  &\color{chocolate}in & \chn{\color{chocolate} the middle}  & {\color{chocolate} east ,} a series of conflicts broke out  \\
%%    \hline
%%   \multirow{2}{*}{Baseline$^\dagger$} & \multicolumn{11}{l}{} & a series of conflicts broke out {\color{chocolate} in the middle east} \\
%%                                                 & \multicolumn{11}{l}{} &  \color{blue}because of  turbulent situation \\
%% %  \multirow{2}{*}{Baseline$^\ddagger$} & \multicolumn{11}{l}{} & a series of conflicts broke out {\color{blue} due to turbulence } \\
%% %                                                & \multicolumn{11}{l}{} &  \color{chocolate}in the middle east region \\
%%  \end{tabular} 
%%  }
%%  \caption{Our ``wait-3''  can also move the reason clause (``because of the ...'') to the beginning of the sentence and the location clause (``in the middle east'') to the middle of sentence.}
%%  \label{tb:war}
%%  \end{table*}
%% %% \smallskip


%% \resizebox{16cm}{!}{%
%% \setlength{\tabcolsep}{2pt}
%% \centering
%% \begin{tabular}{ c |c c c c c c c c  l  }
%%  & 1&2&3&4&5&6&7&8& \\
%%  Chines & 江 & 泽民 & 对 & 布什 & 的& 发言 & 表示 & \color{blue}遗憾 &  \\ 
%%  Pinyin & \chn{ji\={a}ng} & \chn{z\'em\'in} & \chn{d\`ui} & \chn{b\`ush\'i} & \chn{de} & \chn{f\={a}y\'an} & \chn{bi\v{a}osh\`i} & \color{blue}\chn{y\'ih\`an} &  \\ 
%%  Gloss & jiang & zemin & to & bush & 's & speech & express & \color{blue}regret \\  
%%  \hline
%%  Wait-3 &  & & & jiang & zemin & expressed & his & \color{red}{appreciation} & for  bush 's speech \\
%%  Wait-5 &  & & & & & jiang & zemin & expressed & {\color{blue}{regret}} over bush 's speech  \\
%%  \hline
%%  {Baseline$^\dagger$} & \multicolumn{8}{l}{} & jiang zemin expressed {\color{blue}regret} over bush 's speech\\ 
%% {Baseline$^\ddagger$} & \multicolumn{8}{l}{} & jiang zemin expressed {\color{blue}regret} over bush 's speech\\ 
%% \end{tabular} 
%% }
%% \caption{Different outputs between ``wait-3'' and ``wait-5'' models. When ``wait-3'' model decodes the $5^{th}$ target word, the encoder  can only see the first 7 words
%%   while ``wait-5'' model at that point can already see the entire source sentence.
%%   This is why ``wait-5'' model correctly predicts ``regret'' while ``wait-3'' model incorrectly predicts ``appreciation''. % based on training experience.
%%   Baseline$^\dagger$ and Baseline$^\ddagger$ represent greedy and beam search decoding (beam size 11) results, resp.}
%% \label{tb:w3vsw5}
%% \end{table*}




% the first line is Chinese inputs which are represented by pinyin for easier reference to non-Chinese speaker. 
% The second line is the ``gloss'' which is the word-by-word translation.
% Our ``wait-3'' system's outputs are in the third line of the table 
% with $3$ words behind the inputs.
% Baseline method which starts generating words after the entire source 
% sentence are encoded in the last row.



\iffalse
Table~\ref{tb:olympic} demonstrates that our system could move
the prepositional phrase to the end of the sentence depend on the situation.
For the case in Table~\ref{tb:olympic}, the year information is the $3^{th}$ word on source side,
while the first decoding step only can see the first three words.
Then the decoder move the time information to the end of the sentence.
Table~\ref{tb:war} shows that our model also can move reason clause to 
the beginning of the 
sentence and location clause to the middle of sentence.





Table~\ref{tb:w3vsw5} shows another comparison between ``wait-3'' and ``wait-5'' models.
During decoding time, ``wait-3'' can not observe any sentimental information at $5^{th}$
decoding time since the sentimental information ``\chn{y\'ih\`an}'' ("regret")
only shows up at the end of sentence.
Therefore, the ``wait-3'' model makes the prediction of ``appreciation'' based on training 
experience. 
For ``wait-5'' model which can observe the sentimental information at the $5^{th}$ decoding
step, the model can correctly predict the word ``regret''.

We also make further analysis about the probability difference between these two words:
``wait-3'' model predict ``appreciation'' with probability of $18.2\%$ while the word ``regret'' 
ranks at the $20^{th}$ with the probability of $0.0047\%$.
For the ``wait-5'' model, after the model observed the sentimental 
information ``\chn{y\'ih\`an}'' (means regret) from the source side,
the word ``appreciation'' was degraded to $21^{th}$ place with a confident of $0.0026\%$
and the model promotes ``regret'' to the first place with confident of $24.2\%$
% which is higher probability than the 
which is higher probability than the 
word ``appreciation'' in ``wait-3'' model.

\fi




%\subsection{Limitations of Our Work}





Fig.~\ref{fig:fire} demonstrates a major limitation of our fixed wait-$k$ policies,
that is, sometimes it is just impossible to predict correctly and
you have to wait for more source words. In this example,
due to the required long-distance reordering between English and Chinese
(the sentence-final English clause has to be placed very early in Chinese),
any wait-$k$ model would not work, and a good policy should wait till the very end.


%% This example demonstrates another major limitation in almost all simultaneous translation work including ours,
%% which are usually trained on non-simultaneous parallel text such as newswire in our experiments.
%% These data often includes unnecessary long-distance reorderings which could be eliminated
%% by paraphrasing, as is often done by human interpreters.



% \begin{table*}
% \setlength{\tabcolsep}{2pt}
% \centering
% \resizebox{16cm}{!}{%
% \begin{tabular}{ c |c c c c c c c c c l  }
%  & 1&2&3&4&5&6&7&8& \\
%  Chinese & \chn{ji\={a}ng} & \chn{z\'em\'in} & \chn{d\`ui} & \chn{b\`ush\'i} & \chn{de} & \chn{f\={a}y\'an} & \chn{bi\v{a}osh\`i} & \chn{y\'ih\`an} &  \\ 
%  Gloss & jiang & zemin & to & bush & 's & speech & express & regret \\  
%  \hline
%  Wait-3 &  & & & jiang & zemin & expressed & his & \color{red}{appreciation} & for & bush 's speech \\
%  Wait-5 &  & & & & & jiang & zemin & expressed & {\color{blue}{regret}} & over bush 's speech  \\
%  \hline
%   \multirow{2}{*}{Baseline} & \multicolumn{9}{l}{} & jiang zemin expressed {\color{blue}regret}\\ 
% & \multicolumn{9}{l}{} &  over the us president 's remarks\\
% \end{tabular} 
% }
% \caption{Outputs difference between ``wait-3'' and ``wait-5'' words models. When ``wait-3'' model decodes to the $5^{th}$ word, the encoder only can see the first $7$ words while ``wait-5'' model can see the entire source sentence. This is the reason why ``wait-5'' model made a correct prediction of ``regret'' while ``wait-3'' model predicted ``welcome'' based on training experience.}
% \label{tb:w3vsw5}
% \end{table*}


% \begin{table*}
% \setlength{\tabcolsep}{1.2pt}
% \centering
% \resizebox{16cm}{!}{%
% \begin{tabular}{ c | c c c c c c c c l }
%  & 1&2&3&4&5&6&7&8&  \\
%  Chinese & \chn{j\`inni\'anl\'ai} & \chn{zh\={o}nggu\'o} & \chn{zh\`engf\v{u}} &  \chn{y\`izh\'i} & \chn{zh\`il\`i} & \chn{y\'u} & \chn{xi\={a}och\'u} & \chn{p\'ink\`un} & \\ 
%  Gloss & recently & chinese & govt. &  always & dedicate & to & remove & poverty &\\  
%  \hline
%  Wait-3 &  &  & & \color{blue}in & \color{blue}recent & \color{blue}years & , &the & chinese  government  has  been  working  hard  to  eliminate  poverty  \\
%   %\hline
%  \chn{+catchup} &  &  & & \color{blue}in & \color{blue}recent & \color{blue}years  & \chn{, the} & chinese & government  has  been  working  hard  to  eliminate  poverty  \\
%  % Baseline & the & chinese & government & has & been & working & hard & to & eliminate & poverty & in & recent & years & &   \\
%  \hline
%  \multirow{2}{*}{Baseline} & \multicolumn{8}{l}{} &  the chinese government has been working hard to eliminate \\
%                                                & \multicolumn{8}{l}{} & poverty \color{blue}{in recent years}\\
% \end{tabular} 
% }
% \caption{Comparison between ``wait-3'' model and baseline (greedy). Our proposed model moves the prepositional phrase (``in recent years'') to the beginning of the sentence to reduce latency with better accuracy.}
% \label{tb:ppprefix}
% \end{table*}

% \definecolor{chocolate(traditional)}{rgb}{0.48, 0.25, 0.0}
% \definecolor{chocolate}{rgb}{0.48, 0.25, 0.0}
% \definecolor{bole}{rgb}{0.47, 0.27, 0.23}












% \begin{table*}
% \resizebox{16cm}{!}{%
% \setlength{\tabcolsep}{2pt}
% \centering
% \begin{tabular}{ c | c c c c c c c c l  }
%  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 &    \\
%  Chinese & 奥运会 & 将 & \color{blue}于 & \color{blue}\chn{2008} & \color{blue}年 & 在 & 北京 & 举行  \\
%  Pinyin & \chn{\`Aoy\`unhu\`{i}} & \chn{ ji\={a}ng} & \color{blue}\chn{y\'u} & \color{blue}\chn{2008} & \color{blue}\chn{ni\'an} & \chn{z\`ai} & \chn{B\v{e}ij\={\i}ng} & \chn{j\v{u}x\'ing} & \\ 
%  Gloss & Olympics & will & \color{blue}in & \color{blue}2008 & \color{blue}year & in & Beijing & hold \\  
%  \hline
%  Wait-3 &  & & & the & olympic & games  &will& be & held in  beijing  \color{blue}in  \color{blue}2008     \\
%   %\hline
%  \chn{+catchup} &  & & & the & olympic & games  & \chn{will be} & held &in  beijing  \color{blue}in  \color{blue}2008     \\
%  \hline
%  Baseline & \multicolumn{8}{l}{} &  the olympic games will be held in beijing {\color{blue}in 2008}
% \end{tabular} 
% }
% \caption{Our ``wait-3'' model moves the adverbial (``in 2008'') to the end, which is fluent in the English word order, and produces a translation identical 
% to the non-simultaneous baseline.}
% \label{tb:olympic}
% \end{table*}




% \begin{table*}
% \resizebox{16cm}{!}{%
% \setlength{\tabcolsep}{1.2pt}
% \centering
% \begin{tabular}{ c | c c c c c c c c c c c l }
%  & 1&2&3&4&5&6&7&8&9&10&11&  \\
%  Chinese & \color{chocolate}中东 & \color{chocolate}地区 & \color{blue}因为 & \color{blue}局势& \color{blue}动荡 & 所以 & 爆发 & 了 
%  & 一 &系列& 冲突 & \\
%  Pinyin & \color{chocolate}\chn{zh\={o}ngd\={o}ng} & \color{chocolate}\chn{d\`iq\={u}} & \color{blue}\chn{y\={\i}nw\'ei} & \color{blue}\chn{j\'ush\`i} & \color{blue}\chn{d\`ongd\`ang} & \chn{s\v{u}oy\v{\i}} & \chn{b\`aof\={a}} & \chn{le} 
%  & \chn{y\'i} &\chn{x\`ili\`e}& \chn{ch\={o}ngt\={u}} & \\ 
%  Gloss & \color{chocolate}mideast & \color{chocolate}area & \color{blue}because & \color{blue}situation & \color{blue}turbulent & so & break & - & a & series & conflicts\\  
%  \hline
%  Wait-3 &  & & & \color{blue}because & \color{blue}of & \color{blue}the  &
%  \color{blue}tur- & \color{blue}bul- & \color{blue}ence
%  &\color{chocolate}in & \color{chocolate} the  & {\color{chocolate}middle east ,} a series of conflicts have occurred  \\
%   %\hline
%  \chn{+catchup} &  & & & \color{blue}because & \color{blue}of & \color{blue}the  &
%  \chn{\color{blue}tur-  \color{blue}bul-} & \color{blue}ence & \color{blue}situation
%  &\color{chocolate}in & \chn{\color{chocolate} the middle}  & {\color{chocolate} east ,} a series of conflicts broke out  \\

%  % Baseline & the & chinese & govt. & has & been & working & hard & to & eliminate & poverty & in & recent & years & &   \\
%  \hline
%  \multirow{2}{*}{Baseline} & \multicolumn{11}{l}{} &  {\color{chocolate}the middle east region} has a series of conflicts \\
%                                                & \multicolumn{11}{l}{} &  \color{blue}because of the turbulent situation \\
% \end{tabular} 
% }
% \caption{Our ``wait-3'' also can move the reason clause (``because the situation ...'') to the beginning of the sentence.}
% \label{tb:war}
% \end{table*}


% \begin{table*}
% \resizebox{16cm}{!}{%
% \setlength{\tabcolsep}{2pt}
% \centering
% \begin{tabular}{ c |c c c c c c c c c l  }
%  & 1&2&3&4&5&6&7&8& \\
%  Chines & 江 & 泽民 & 对 & 布什 & 的& 发言 & 表示 & \color{blue}遗憾 &  \\ 
%  Pinyin & \chn{ji\={a}ng} & \chn{z\'em\'in} & \chn{d\`ui} & \chn{b\`ush\'i} & \chn{de} & \chn{f\={a}y\'an} & \chn{bi\v{a}osh\`i} & \color{blue}\chn{y\'ih\`an} &  \\ 
%  Gloss & jiang & zemin & to & bush & 's & speech & express & \color{blue}regret \\  
%  \hline
%  Wait-3 &  & & & jiang & zemin & expressed & his & \color{red}{appreciation} & for & bush 's speech \\
%  Wait-5 &  & & & & & jiang & zemin & expressed & {\color{blue}{regret}} & over bush 's speech  \\
%  \hline
%   \multirow{2}{*}{Baseline} & \multicolumn{9}{l}{} & jiang zemin expressed {\color{blue}regret}\\ 
% & \multicolumn{9}{l}{} &  over bush 's remarks\\
% \end{tabular} 
% }
% \caption{Outputs difference between ``wait-3'' and ``wait-5'' words models. When ``wait-3'' model decodes to the $5^{th}$ word, the encoder only can see the first $7$ words while ``wait-5'' model can see the entire source sentence. This is the reason why ``wait-5'' model made a correct prediction of ``regret'' while ``wait-3'' model predicted ``welcome'' based on training experience.}
% \label{tb:w3vsw5}
% \end{table*}




==> simul-acl copy 2/intro.tex <==
% !TEX root = main.tex


%We study
Simultaneous translation %which aims to eventually automate 
%the automatic form of
%has the potential
aims to automate simultaneous interpretation,
%There are 
%Between the two modes of human interpretation,
%consecutive and simultaneous.
%Consecutive interpretation
%is common in press conferences and one-on-one meetings,
%where
%While consecutive interpretation waits until 
%starts
%to translate when 
%the speaker pauses (usually at sentence boundaries) to initiate translation,
%and thus doubling the time needed,
%and therefore the time needed (at least) doubles.
%if it takes $T$ second to finish a conversation in one language,
%it will take at least $2T$ seconds to finish it via consecutive interpretation.
%simultaneous interpretation  %, by contrast,
%interprets while the speaker is speaking,
%and preferably
%starts translation within seconds after the speaker starts speaking,
%and finishes within seconds after the speaker finishes.
which translates concurrently with the source-language speech,
with a delay of only a few seconds.
%Therefore the time needed is only $T+\delta$.
This {\em additive} latency %of $\delta$ 
%which is 
%often less than 3 seconds in practice,
is much more desirable than the {\em multiplicative} 2$\times$ slowdown
in consecutive interpretation.

%This multiplicative overhead of 2x is undesirable,


\begin{figure}%[t]
\centering
\includegraphics[width=7.8cm]{figs/waitk.pdf}
\captionof{figure}{Our wait-$k$  model 
emits target word $y_t$ given source-side prefix $x_1 ...\, x_{t+k-1}$,
often before seeing the corresponding source word
(here $k$=2, outputing $y_3$=``met'' before $x_7$={\small ``\huiwu''}). % is available. %  corresponding to $y_t$.
%% Here $k$ is 2, and the model learns to predict %the English verb
%% ``meets'' given the Chinese prefix
%% {\em ``\bushi \zongtong \zai \mosike''} (``Bush President at Moscow''),
%% long before the Chinese verb  %equivalent of ``meet'' (
%% \huiwu (``meet'') %)
%% arrives at the very end.
Without anticipation, a 5-word wait is needed (dashed arrows). See also~Fig.~\ref{fig:idea2}.
}
\label{fig:idea}\vspace{-0.3cm}
\end{figure}
\begin{figure*}

\resizebox{\textwidth}{!}{
%\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabu}{l | l l l l l l l l l l l l   l }
% & 1 & 2 & & 3 & & 4 & & 5 & & 6 & & 7 &  \\
  \rowfont{\small}
& \textbf{\textit{B\`ush\'\i}}\, & \textbf{\textit{z\v{o}ngt\v{o}ng}} &\textbf{\textit{z\`ai}}  & \textbf\textit{M\`os\={\i}k\=e} & \transparent{0.5}\color{gray}\yu   &\transparent{0.5}\color{gray}\pujing &  \transparent{0.5}\color{blue}\huiwu \\
 &  \bf布什\, & \bf总统 &\bf在& \bf莫斯科 & \transparent{0.5}与 & \transparent{0.5}普京 & \transparent{0.5}\color{blue}会晤\\
 \rowfont{\small}
 & \bf Bush & \bf president& \bf in & \bf Moscow & \transparent{0.5}with/and & \transparent{0.5}Putin & \transparent{0.5}\color{blue}meet\\
\hline
(a) simultaneous: our wait-2  & \multicolumn{2}{c}{\small\em\color{red} ...wait 2 words...} &  pres.  & bush & \bf \color{blue}met &    \color{gray}with  &  
\color{gray}putin& \multicolumn{2}{l}{\color{gray}  in  moscow}\\
\hline
(b) non-simultaneous baseline & \multicolumn{7}{c}{\small\em\color{red} ..... wait whole sentence ......} & \multicolumn{2}{l}{pres. bush {\color{blue}met} with putin in moscow}\\
(c) simultaneous: test-time wait-2 & \multicolumn{2}{c}{\small\em\color{red} ...wait 2 words...} &  pres.  & bush & in & moscow &    and  &  \multicolumn{2}{l}{pol- ite meeting}\\
\hline
\hline
 &  布什\, & 总统 & &\qquad 在& 莫斯科 &与 &普京 & \color{blue}会晤\\
(d) simultaneous: non-predictive    & \multicolumn{2}{c}{\small\em\color{red} ...wait 2 words...} &  pres. bush\!\!\!\!\!\!\!\!\!\!\!\! & \multicolumn{5}{c}{{\em\color{red} \qquad ..... wait 5 words ......}} & {\color{blue}met}  with  putin   in  moscow\\
 \end{tabu}
}
\caption{Another view of  Fig.~\ref{fig:idea}, highlighting the prediction of  English {\color{blue}``met''}
  corresponding to the sentence-final Chinese verb {\color{blue}\huiwu}. % (``meet'') is at the end. %comes at the very end, just like a German verb.
%The full-sentence (non-simultaneous) translation needs to wait till the end of the Chinese sentence,
(a) Our wait-$k$ policy (here $k=2$) translates concurrently with the source sentence, but always $k$ words behind. % after the first $k$ source words,
It correclty predicts the English verb given just the first 4 Chinese words (in bold),
%\bushi \zongtong \zai \mosike (
lit.~``Bush president in Moscow'',
%This is 
because it is trained in a prefix-to-prefix fashion (Sec.~\ref{sec:pred}), and the training data contains many prefix-pairs in the form of (X \zai Y ...,  X met ...).
(c) The test-time wait-$k$ decoding (Sec.~\ref{sec:waitk}) using the full-sentence model in (b) can not anticipate 
and produces nonsense translation.
(d) A simultaneous translator without anticipation such as \namecite{gu+:2017}
has to wait 5 words. % for \huiwu. % is received.
%where X is an official and Y is a location.
%and we train our model in a prefix-to-prefix way to force it to output ``met'' given the 4-word Chinese prefix.
\label{fig:idea2}
}
\end{figure*}


%Simultaneous translation aims to automate
With this appealing property,
simultaneous interpretation
%has been gradually replacing consecutive interpretation
%ever since the famous Nuremburg Trials \cite{nuremberg:1946,palazchenko:1997},
%and
%and
has been widely used in many scenarios including
multilateral organizations (UN/EU),
and international summits (APEC/G-20). %, and conferences.
%bilateral/multilateral negotiations.
%and legal proceedings.
However, due to the concurrent comprehension %(in the source language)
and production in two languages, %(in the target language),
it is  extremely challenging and exhausting  for humans:
% there are reportedly only a few thousand 
the number of qualified
simultaneous interpreters worldwide is very limited,
%\footnote{
%The International Association of Conference Interpreters (AIIC),
%the only global association of conference interpreters,  3,000 professionals
and each can only last for about 15-30 minutes in one turn,
whose error rates grow exponentially after just minutes of interpreting \cite{moser+:1998}.
Moreover, %it has been shown that
limited memory forces
human interpreters to routinely omit source content \cite{hehe+:2016}.
%and the best of them can only retain about 60\% of the source material.
Therefore, there is %a huge demand for simultaneous interpretation but not nearly enough supply,
%leaving
a critical need to % automate this task by
develop simultaneous machine translation techniques
to reduce the burden of human interpreters %\cite{un:1957} 
and make it % this service
more accessible and affordable.


Unfortunately, simultaneous translation is also notoriously difficult for machines,
 due in large part to the diverging word order between the source and target languages.
For example, think about simultaneously translating an SOV %or verb-final
language such as Japanese or German to an SVO language such as English or Chinese:\footnote{
Technically, German is SOV+V2 in main clauses,
and SOV in embedded clauses; Mandarin is a mix of SVO+SOV.}
you have to wait until the source language verb.
As a result, %virtually all
existing so-called ``real-time'' translation systems resort to conventional full-sentence translation,
causing an undesirable latency of at least one sentence. % delay on the target-side, which is more akin to consecutive translation.
%and rendering the user out of sync with the speaker.
Some researchers, on the other hand,
have noticed the importance of verbs in SOV$\goesto$SVO translation
\cite{grissom+:2016}, and
have attempted to reduce latency by explicitly predicting the sentence-final German \cite{grissom+:2014} or English verbs \cite{matsubarayx+:2019},
which is limited to this particular case,
or unseen syntactic constituents \cite{oda+:2015,he+:2015},
which requires incremental parsing on the source sentence.
Some researchers propose to translate on an optimized sentence
segment level to get better translation 
accuracy \cite{oda+:2014,fujita+:2013,bangalore+:2012}.
%% Others use reinforcement learning to prefer (rather than enforce) a specific % segment or
%% latency:
More recently, \namecite{gu+:2017}
propose a two-stage model % trained in two stages.
whose base model is a full-sentence model, %, % except that it is unidirectional,
%trained in the conventional way.
On top of that, they use a READ/WRITE (R/W) model to decide, at every step, whether to wait for another source word (READ) or to emit a target word 
using the pretrained base model (WRITE),
and this R/W model is trained by reinforcement learning to prefer (rather than enforce) a specific latency, without updating the base model.
%which  is never met at test time.
All these efforts have the following major limitations:
(a) none of them can achieve any arbitrary given latency such as ``3-word delay'';
(b) their base translation model is still trained on full sentences;
and (c) their systems are complicated, involving many components (such as pretrained model, prediction, and RL) and are difficult to train.


%% Other works use reinforcement learning to decide when to wait and when to translate,
%% but is over-complicated and hard to replicate.
%% More importantly, existing efforts can not achieve any practical latency requirements
%% such as the ``3-second delay'' mentioned above.
%% Overall, not enough attention has been given to the latency (rather than quality) issue for this problem.


We instead present a very simple yet % surprisingly
effective solution,
%to this problem.
designing a novel prefix-to-prefix framework that predicts target words using only prefixes of the source sentence.
Within this framework, we study a special case, the ``wait-$k$'' policy, 
%which is trained to translate %concurrently with the input sentence, just always
whose translation is always $k$ words behind the input.
Consider the Chinese-to-English example in Figs.~\ref{fig:idea}--\ref{fig:idea2}, where the translation of the sentence-final Chinese verb \huiwu (``meet'')
needs to be emitted earlier to avoid a long delay.
Our wait-2 model correctly anticipates the English verb given only the first 4 Chinese words (which provide enough clue for this prediction
given many similar prefixes in the training data).
We make the following contributions:
\begin{itemize}
    \setlength\itemsep{.1em}
\item Our prefix-to-prefix framework is tailored to simultaneous translation
and trained from scratch without using full-sentence models.
\item It
  %This framework
  seamlessly integrates implicit anticipation and translation in a single model
  that directly predicts {\em target} words without explictly hallucinating {\em source} ones.
  %% Unlike previous efforts which explicit predict source words,
  %% our work directly predicts target words.
\item As a special case, we present a  ``wait-$k$'' policy %for simultaneous translation
  %trained to generate the target sentence concurrently with the source sentence, but always $k$ words behind,
  %for any given $k$. % the source input.
%\item
  %This strategy  therefore
  that can satisfy any latency requirements.
%% \item Unlike previous works with explicit prediction of source words,
%%   our model directly predicts target words, and seamlessly integrates anticipation and translation in a single model.
\item This strategy %only involves minor changes to the existing sequence-to-sequence framework,
  %and
  can be  applied to most sequence-to-sequence models with relatively minor changes.
  Due to space constraints, we only present its performance 
  the Transformer \cite{vaswani+:2017},
  though our initial experiments on RNNs \cite{bahdanau+:2014} showed equally strong results (see our November 2018 arXiv version {\footnotesize \url{https://arxiv.org/abs/1810.08398v3}}).
  %It is also much  faster to train than previous ones. % and can scale up to larger corpora.
  \iffalse
\item We also propose a new metric of latency called ``Averaged Lagging'', which addresses deficiencies of previous metrics.
  %\item This framework can be implemented on any sequence-to-sequence architecture, and we demonstrate two such cases: RNNs and Transformer.
  \fi
\item Experiments show our strategy achieves low latency and reasonable BLEU scores (compared to full-sentence translation baselines) %  with very low latency
   % both Chinese-to-English and English-to-German simultaneous translation.
  on 4 directions: \zhen and \deen. %Chinese$\leftrightarrow$English and German$\leftrightarrow$English. % simultaneous translation.
\end{itemize}


==> simul-acl copy 2/method.tex <==
% !TEX root = main.tex

We first briefly review %the sequence-to-sequence architecture 
standard (full-sentence) neural  translation to %system to
set up the notations. 

Regardless of the particular design of different seq-to-seq models,
%we first encode the entire source sentence and pass 
%the encoded representations to the decoder to generate in the target language. 
%Generally speaking,
the encoder always takes the input 
sequence $\vecx = (x_1,...,x_n)$ %of $n$ elements 
where each $x_i \in \mathbb{R}^{d_x}$ is a word embedding of $d_x$ dimensions,
and produces a new sequence of hidden states $\vech =f(\vecx) = (h_1,...,h_n)$. %where $h_i = f(\vecx)$.
The encoding function $f$ can be implemented by RNN or Transformer. %-based model.

On the other hand, a (greedy) decoder 
predicts %the probability of 
the next output word $y_t$
given the source sequence (actually its representation \vech) 
and previously generated words, denoted $\vecy_{<t}=(y_1,...,y_{t-1})$.
%Consequently, during greedy search, at time step $i$,
%the decoder picks the word with highest
%probability score as $y_i$.
The decoder %will continue generating more words until
stops when it emits \eos,
%At the end %When decoding finishes,
and the final hypothesis $\vecy = (y_1,...,\eos)$ %where $y_n$ is $\eos$, with
has probability %the model score:
\begin{equation}
p(\vecy \mid \vecx) = \textstyle\prod_{t=1}^{|\vecy|}  p(y_t \mid \vecx,\, \vecy_{<t})
\label{eq:gensentscore}
\end{equation}
%where $\vecy_{<t}$ denotes the prefix $(y_1,...,y_{(t-1)})$. 
At training time, we maximize the conditional probability of each ground-truth target sentence $\vecy^\star$ given input \vecx
over the whole training data $D$, or equivalently minimizing the following loss:
\begin{equation}
\ell(D) = - \textstyle\sum_{(\vecx,\vecy^\star)\in D} \log p(\vecy^\star \mid \vecx) %\sum_{t=1}^{|\vecy^\star|}  \log p(y_t \mid \vecx,\, \vecy^\star_{<t})
\label{eq:train}
\end{equation}




==> simul-acl copy 2/pred.tex <==
% !TEX root = main.tex


\begin{figure}%[t]
\centering
\includegraphics[width=7.8cm]{figs/pref2pref.pdf}
\captionof{figure}{Seq-to-seq vs.~our prefix-to-prefix frameworks (showing wait-2 as an example).
}
\label{fig:p2p}
\end{figure}


In full-sentence translation (Sec.~\ref{sec:method}), 
each $y_i$ %in Eq.~\ref{eq:gensentscore}
is predicted using the entire source sentence~$\vecx$.
But in simultaneous translation,
we need to translate concurrently with the (growing) source sentence,
%% i.e.,
%% only prefixes of  $\vecx$ are available, %and %where we need immediate translation outputs before the entire source sentence finishes, 
so we design a new prefix-to-prefix architecture
to (be trained to) predict using a source prefix.

\subsection{Prefix-to-Prefix Architecture} %and Wait-$k$}

% we need to design a different way of generating predictions.
%we propose a
%% In our prefix-to-prefix framwork,
%% the decoder starts producing 
%% target words when the encoder only sees an ever growing prefix of the source sentence.
%% %\footnote{
%%   %We mean prefix by prefix of the word sequence,
%% %By ``prefix'' we mean prefix of the sequence of words.}
%% For example, given a source sentence $\vecx$, 
%% we use $\vecx_{\leq{t}}$ to denote the prefix of source sentence
%% $(x_1,...,x_{t})$, i.e., the first $t$ {\em words} of $\vecx$.


\begin{definition}
Let $g(t)$ be a {\bf monotonic non-decreasing} function of $t$
that denotes the number of source words processed by the encoder when deciding the target word $y_t$.
\end{definition}
For example, in Figs.~\ref{fig:idea}--\ref{fig:idea2}, $g(3)=4$,
i.e., a 4-word Chinese prefix is used to predict $y_3$=``met''.
We use the source prefix %$\vecx_{\leq{g(t)}} =
$(x_1,...,x_{g(t)})$ rather than the whole $\vecx$
%and the  target prefix $\vecy_{<t}$ 
to predict $y_t$:
\(
p(y_t \mid \vecx_{\leq{g(t)}},\, \vecy_{<t}).
\)
Therefore the decoding probability is: %decoding objective is
%of our prefix-to-prefix are: % framework become: %are as follows:
\begin{equation}
\vspace{-0.1cm}
p_g(\vecy \mid \vecx) = \textstyle\prod_{t=1}^{|\vecy|} p(y_t \mid \vecx_{\leq{g(t)}},\, \vecy_{<t})
\label{eq:ourgoal}
\end{equation}
and given training $D$, the training objective is:
\begin{equation}
\ell_g(D) = - \textstyle\sum_{(\vecx,\,\vecy^\star)\in D} \log p_g(\vecy^\star \mid \vecx)
\label{eq:newtrain}
\end{equation}
%where $g(t)$ is a monotonic function of $t$ which describes the number of source words that have been processed by the encoder at decoding time step t.
%% Then the term $\vecx_{\leq{g(t)}}$  %represents theprocessed source sequence
%% denotes the prefix
%% $(x_1,...,x_{g(t)})$.

Generally speaking, $g(t)$ can be used to represent any arbitrary policy,
and we give two special cases where $g(t)$ is constant:
%\begin{itemize}
%\item
(a) $g(t)=|\vecx|$: baseline full-sentence translation;
%\item
(b) $g(t)=0$: an ``oracle'' that does not rely on any source information.
Note that in any case, $0 \leq g(t)\leq |\vecx|$ for all $t$.
%\end{itemize}
%, which reveal the number of processed word(s)
%on both encoder and decoder.

\iftrue
\begin{definition}%[cut-off step]
We define the {\bf ``cut-off'' step}, $\tau_g(|\vecx|)$,
to be the decoding step when source sentence finishes:
\begin{equation}
\tau_g(|\vecx|) = \min \{t \mid g(t)=|\vecx|\} 
\end{equation}
\end{definition}
\noindent
For example, in Figs.~\ref{fig:idea}--\ref{fig:idea2}, the cut-off step is 6,
i.e., the Chinese sentence finishes right before $y_6$=``in''.
\fi

\smallskip

\noindent
{\bf Training vs.~Test-Time Prefix-to-Prefix.}
While most previous work in simultaneous translation, in particular \namecite{bangalore+:2012} and \namecite{gu+:2017}, might be seen as special cases in this framework,
we note that only their {\em decoders} are prefix-to-prefix, while their training is still full-sentence-based. %seq-to-seq.
In other words, they use a full-sentence translation model to do simultaneous decoding, which is a mismatch between training and testing.
The essence of our idea, however, is to {\em train} the model to predict using source prefixes. % thus unifying training and testing.
Most importantly, %being {\em forced} to predict using a source prefix
this new training implicitly learns anticipation as a by-product, overcoming word-order differences such as SOV$\goesto$SVO.
Using the example in Figs.~\ref{fig:idea}--\ref{fig:idea2},
the anticipation of the English verb is possible because
the training data contains many prefix-pairs in the form of (X \zai Y ...,  X met ...),
thus although the prefix $\vecx_{\le 4}$=``\bushi \zongtong \zai \mosike'' (lit.~``Bush president in Moscow'') does not contain the verb,
it still provides enough clue to predict ``met''. %to predict ``met''.
%(see Figs.~\ref{fig:idea}--\ref{fig:idea2}).

\subsection{Wait-$k$ Policy}
\label{sec:waitk}

\iffalse
\begin{figure}%[t]
\centering
\includegraphics[width=7.8cm]{figs/tailbeam.pdf}
\captionof{figure}{Tail beam search after the entire source sentence is finished.
%  The earlier target words must be greedily generated.
}
\label{fig:tailbs}
\end{figure}
\fi

%Inspired by this,
As a very simple example within the prefix-to-prefix framework,
we present a wait-$k$ policy,
which first wait $k$ source words,
and then translates concurrently with the rest of source sentence, i.e., the output is always $k$ words behind the input. % after the first $k$ source words,
This is inspired by human simultaneous interpreters who generally start translating a few seconds into the speakers' speech,
and finishes a few seconds after the speaker finishes.
For example, if $k=2$, the first target word is predicted using the first 2 source words,
and the second target word using the first 3 source words, etc; see Fig.~\ref{fig:p2p}.
%which adapts the prediction 
%on decoder side into making prediction on the next output word $y_t$
%based on the input prefix $\vecx_{\leq{g(t)}}$ and output prefix $\vecy_{<t}$.
More formally, its $g(t)$ is defined as follows:
\begin{equation}
  \gwaitk(t) =\min\{k+t-1, \, |\vecx|\}
%%   \left\{\begin{matrix} 
%%  k+t-1 & t < |\vecx|-k \\ 
%%  |\vecx|  &  \text{otherwise} %|x|-k \leq t 
%% \end{matrix}\right. 
\label{eq:policy}
\end{equation}
For this policy, the cut-off point $\tau_\gwaitk(|\vecx|)$ is exactly $|\vecx|-k+1$
(see Fig.~\ref{fig:catchup}).
%and for all $t>|\vecx|-k$,
%For all $t\geq |\vecx|-k$,
From this step on,
$\gwaitk(t)$ is fixed to $|\vecx|$, %$\tau_g(|\vecx|)$, %the  source sentence is finished, and
which means the remaining target words (including this step) are generated using the full source sentence,
similar to conventional MT.
We call this part of output, $\vecy_{\geq |\vecx|-k}$, the ``tail'', and
can perform beam search on it (which we call ``tail beam search''),
but all earlier  words %($t<\tau_g(|\vecx|)$)
are generated greedily one by one %and 
%must be generated
%greedily
(see Appendix). %Fig.~\ref{fig:tailbs}). %in a greedy fashion
%due to simultaneity requirements.
%because they are generated one word at a time.
\iffalse
A general prefix-to-prefix policy
such as the {\em decoder} of \namecite{gu+:2017},
however, can use beam search whenever $g(t)=g(t-1)$,
i.e., predicting more than one word using the {\em same} input prefix. % (e.g., the tail in wait-$k$).
\fi

\smallskip
\noindent
    {\bf Test-Time Wait-$k$.}
    As an example of test-time prefix-to-prefix in the above subsection,
    we present a very simple ``test-time wait-$k$'' method, i.e.,
    using a full-sentence model but decoding it with a wait-$k$ policy (see also Fig.~\ref{fig:idea2}(c)).
    %In fact,
    Our experiments show that this method, without the anticipation capability, performs much worse than our genuine wait-$k$
    when $k$ is small, but gradually catches up, and eventually both methods approach the full-sentence baseline ($k=\infty$).

%% This is different from \namecite{gu+:2017} who
%% output several words at a time and can perform beam search before the tail.


%% where $k$ represents the word-level 
%% latency which means that 
%% the target side is always $k$ word(s) behind the source side.


%% \if
%% To have a simple overview of our proposed ``wait-$k$'' process,
%% we only need to adapt the prediction on decoder side into making 
%% prediction on the next output word $y_t$
%% % based on the whole input sequence \vecx and the output prefix $\vecy_{<i}$,
%% % we now train a ``wait-$k$'' model to predict $y_i$ 
%% based on the input prefix $\vecx_{<{(t+k)}}$ and output prefix $\vecy_{<t}$.
%% We use $\vecx_{<{(t+k)}}$ to represent the processed source sequence
%% $(x_1,...,x_{(t+k-1)})$ and $k$ to represent the word-level 
%% %translation
%% latency which means that 
%% the target side is always $k$ word(s) behind the source side.
%% %Our decoding time step $t$ starts from 1 and $(t+k-1)$ always capped with $|\vecx|$.
%% Then we have the following wait-$k$ model: %decoding strategy:
%% \begin{equation}
%% \vspace{-0.1cm}
%% p_k(\vecy \mid \vecx) = \textstyle\prod_{t=1}^{|\vecy|} p(y_t \mid \vecx_{<(t+k)},\, \vecy_{<t})
%% \label{eq:ourgoal1}
%% \end{equation}

%% To have a more general definition which can be applied to any arbitrary 
%% policy, we replace the above $(t+k)$ with $g(t)$ to describes the number of source words that have been processed by the encoder at decoding time step $t$:
%% \begin{equation}
%% g(t) = \left\{\begin{matrix} 
%%  k+t-1 & t < |x|-k \\ 
%%  |x|  &  \text{otherwise} %|x|-k \leq t 
%% \end{matrix}\right. 
%% \label{eq:policy}
%% \end{equation}
%% then our new decoding and training objective becomes:
%% \begin{equation}
%% \vspace{-0.1cm}
%% p_g(\vecy \mid \vecx) = \textstyle\prod_{t=1}^{|\vecy|} p(y_t \mid \vecx_{\leq{g(t)}},\, \vecy_{<t})
%% \label{eq:ourgoal}
%% \end{equation}
%% and 
%% \begin{equation}
%% \ell_k(D) = - \textstyle\sum_{(\vecx,\vecy^\star)\in D} \log p_g(\vecy^\star \mid \vecx) %\sum_{t=1}^{|\vecy^\star|}  \log p(y_t \mid \vecx_{\leq{g(t)}},\, \vecy^\star_{<t})
%% %% =======
%% %% \begin{equation}\scriptstyle{
%% %% \ell_k(D) = - \!\!\!\! \displaystyle{\sum_{(\vecx,\vecy^\star)\in D}} \sum_{t=1}^{|\vecy^\star|}  \log p(y_t \mid \vecx_{\leq{g(t)}},\, \vecy^\star_{<t})}
%% %% >>>>>>> ae7bb9d9b39ed69753da93532a3c3755da2ed013
%% \label{eq:newtrain}
%% \end{equation}
%% where $\vecx_{\leq{g(t)}}$  %represents theprocessed source sequence
%% denotes the prefix
%% $(x_1,...,x_{g(t)})$.

%% % based on the input prefix $\vecx_{\leq{g(t)}}$ and output prefix $\vecy_{<t}$.
%% % We use $k$ to represent the word-level translation latency which means that 
%% % decoder is always $k$ word(s) behind the encoder.
%% % The decoder translation step is defined with $t$.
%% % Note that $\vecx_{\leq{g(t)}}$ represents the source sequence $(x_1,...,x_{g(t)})$ and $g(t)$
%% % is always capped with $|\vecx|$.
%% % Here the output stream \vecy is always $k$ words behind the input stream \vecx.
%% % In other words, the training objective becomes:
%% % \begin{equation}
%% % \vspace{-0.1cm}
%% % \score_{k}(\vecx,\vecy) = \textstyle\sum_{t=1}^{|\vecy|} \log p(y_t \mid \vecx_{\leq{g(t)}},\, \vecy_{<t})
%% % \label{eq:ourgoal}
%% % \end{equation}
%% % where $g(t)$ describes the number of source words that have been processed by encoder at decoding time step $t$:
%% % \begin{equation}
%% % g(t) = \left\{\begin{matrix} 
%% %  k+t-1 & 1 \leq t < |x|-k \\ 
%% %  |x|  & |x|-k \leq t 
%% % \end{matrix}\right. 
%% % \label{eq:policy}
%% % \end{equation}
%% \fi

%% Eq.~\ref{eq:policy} describes the number of words that are observed 
%% by decoder from source side.
%% As shown in Fig.~\ref{fig:p2p},
%% when our model decodes the first word,
%% there are $k$ words are observed at encoder.
%% Since the second decoder step, 
%% every later step will observe one more word on source side.
%% After time step $|x|-k$, encoder receives the entire source sentence
%% and the number of observed words stops increasing.

%% The above decoding strategy in Eq.~\ref{eq:ourgoal} is different from Eq.~\ref{eq:gensentscore} and defines an encoding-decoding policy which first waits $k$ words on the source side, then starts to decode the first translated word
%% on target. Thenceforth the decoder will generate a new target word 
%% every time another source word is fed into the encoder.  
% We formally define our ``wait-$k$'' policy as follows:

% \begin{equation}
% p(\tau) = \left\{\begin{matrix}
% k & \tau = 1\\ 
%  p(\tau-1)+1& 2 \leq \tau \leq |x|-k \\ 
%  |x|& |x|-k < \tau 
% \end{matrix}\right. 
% \label{eq:policy}
% \end{equation}
% where $\tau$ represents the decoder time step and $k$ is the number of words that our
% decoder waits.




\iffalse
%The rest of this section introduces
In Sec.~\ref{sec:detail} we will describe two 
%simultaneous Neural Machine Translation frameworks
implementations of this policy %simple framework,
using RNN and Transformer as the underlying model, respectively. %-based implementations.
%We first talk about our RNN-based approach then introduce our Transformer-based 
%model with more details.
\fi


==> simul-acl copy 2/related.tex <==
% !TEX root = main.tex

The work of \namecite{gu+:2017} is different from ours in four (4) key aspects:
(a) by design, their model does not anticipate;
(b) their model can not achieve any specified latency metric at test time while our wait-$k$ model is guaranteed to have a $k$-word latency; % (even though encouraged at training time);
(c) their model is a combination of two models, using a full-sentence base model to translate, thus a mismatch between training and testing,
while our work is a genuine simultaneous model,
and
(d) their training is also two-staged, using RL to update the R/W model, while we train from scratch.

In a parallel work, % released after our paper,
\namecite{press+smith:2018} propose an ``eager translation" model which also outputs target-side words before the whole input sentence is fed in, 
but there are several crucial differences:
(a) their work still aims to translate full sentences using beam search, and is therefore, as the authors admit, ``not a simultaneous translation model'';
(b) their work does not anticipate future words; and
(c) they use word alignments to learn the reordering and achieve it 
in decoding by emitting the $\epsilon$ token, while our work integrates reordering into a single wait-$k$ prediction model that is agnostic of, yet capable of, reordering.


In another recent work, \namecite{ashkan+:2018}
adds a prediction action to the work of \namecite{gu+:2017}.
Unlike \namecite{grissom+:2014} who predict the source verb which might come after several words, %maybe several words into the future,
they instead predict the {\em immediate} next source words, which we argue is not as useful  in SOV-to-SVO translation.
%% however, like \namecite{gu+:2017},
%% its translation model is  is {\em not} trained to predict
%This is different from our anticipation in three aspects: its encoder/decoder is still trained using full sentences.
\footnote{
Their codebase on Github is not runnable,
and their baseline %(based on \namecite{gu+:2017}'s code)
 is inconsistent with \namecite{gu+:2017} which we compared to,
so we did not include their results for comparison.
}
In any case, we are the first to predict directly {\em on the target side}, thus
integrating anticipation in a single translation model.


\namecite{jaitly+:2016} propose an online neural transducer for speech recognition
that is conditioned on prefixes. This problem does not have reorderings
and thus no anticipation is needed.

